Riemannian block SPD coupling manifold and its application to optimal transport

In this work, we study the optimal transport (OT) problem between symmetric positive definite (SPD) matrix-valued measures. We formulate the above as a generalized optimal transport problem where the cost, the marginals, and the coupling are represented as block matrices and each component block is a SPD matrix. The summation of row blocks and column blocks in the coupling matrix are constrained by the given block-SPD marginals. We endow the set of such block-coupling matrices with a novel Riemannian manifold structure. This allows to exploit the versatile Riemannian optimization framework to solve generic SPD matrix-valued OT problems. We illustrate the usefulness of the proposed approach in several applications.

==> icml/icml_manuscript.tex <==




% \begin{abstract}
% % Optimal transport (OT) has seen its popularity in various fields of applications. We start by observing that the discrete OT problem can be equivalently solved with respect to a block matrix-valued coupling with uniform diagonal marginals. This leads us to consider a generalized matrix-valued OT problem setup, where the cost and/or the marginals are symmetric positive definite (SPD) matrix-valued. 

% % We propose a novel Riemannian manifold for the matrix version of general doubly stochastic constraint set, which we call the block SPD coupling manifold. Specifically, we consider blocks of SPD matrices, where summation of row blocks and column blocks are constrained. Developing a manifold structure on the constraint allows to make Riemannian optimization framework to be exploited to solve such problems. The framework is generic to solve any linear and non-linear OT problem without specific regularization. This includes projected matrix-valued OT, matrix-valued domain adaptation and barycentric projection, matrix-valued Wasserstein barycenter, Gromov-Wasserstein OT, and distance averaging.
 
% Optimal transport (OT) has seen its popularity in various fields of applications. We start by observing that the OT problem can be viewed as an instance of a general symmetric positive definite (SPD) matrix-valued OT problem, where the cost, the marginals, and the coupling are represented as block matrices and each component block is a SPD matrix. The summation of row blocks and column blocks in the coupling matrix are constrained by the given block-SPD marginals. We endow the set of such block-coupling matrices with a novel Riemannian manifold structure. This allows to exploit the versatile Riemannian optimization framework to solve generic SPD matrix-valued OT problems. We illustrate the usefulness of the proposed approach in several applications.

% % tensor field mass interpolation, Wasserstein-barycenter learning, 
% % %Gromov-Wasserstein distance averaging, 
% % and domain adaptation tasks.  
% \end{abstract}


\section{Introduction}
Optimal transport offers a systematic approach to compare probability distributions by finding a transport plan (coupling) that minimizes the cost of transporting mass from one distribution to another. Optimal transport has been successfully applied in a wide range of fields, such as computer graphics \citep{solomon2015convolutional,solomon2014earth}, graph representation learning \citep{chen2020graph,petric2019got}, text classification \cite{yurochkin2019hierarchical}, and domain adaptation \citep{courty2016optimal,courty2014domain}, to name a few.

% There exists a number of efficient solvers for classic optimal transport problem \citep{cuturi2013sinkhorn,ferradans2014regularized,genevay2016stochastic,peyre2019computational}. Particularly, by adding an entropy regularization, the OT problem can be solved efficiently via Sinkhorn algorithm \citep{sinkhorn1964relationship} and is known to achieve faster convergence \citep{cuturi2013sinkhorn} and improved sample complexity \cite{genevay2019sample}. 

Despite the popularity of OT, existing OT formulations are mostly limited to {transporting scalar-valued mass.} 
%scalar-valued costs and marginals. 
% which we find it to be an instance of a general OT problem with matrix-valued cost. 
% while sometimes a vector-valued and (positive semidefinite) matrix-valued costs are able to capture more information \cite{lopez2021vector}. 
Applications such as diffusion tensor imaging \cite{le2001diffusion}, image set classification~\cite{huang2015log,harandi2014manifold}, 
anisotropic diffusion \cite{weickert1998anisotropic}, involve symmetric positive definite (SPD) matrix-valued distributions. 
In brain imaging particularly, where the local diffusion of water molecules are encoded in a SPD matrix \cite{assaf2008diffusion}, being able to compare fields of such SPD matrices is crucial. This, however, requires a nontrivial generalization of existing optimal transport framework with careful construction of cost and transport plan. 

% Hence a generalization to matrix-valued OT is needed. \alertPJ{I think we need to change/improve this as SPD/matrix valued data points is not our focus. Our focus is SPD-valued marginals. SPD/matrix valued data can have scalar-valued marginals. Maybe we can take inspiration from the motivation from existing works. } 

In the quantum mechanics setting, existing works~\citep{jiang2012distances,carlen2014analog,chen2017matrix,chen2018vector} have explored geodesic formulation of the Wasserstein distance between vector and matrix-valued densities. In \citep{ning2013thesis,ning2014matrix}, the Monge-Kantorovich optimal mass transport problem has been studied for comparing matrix-valued power spectra measures. Recently, \citet{peyre2016quantum} proposed to solve an unbalanced optimal transport problem for SPD-valued distributions of unequal masses. 

%In \cite{jiang2012distances,carlen2014analog,chen2017matrix,chen2018vector}, a geodesic formulation of the Wasserstein distance between vector and matrix-valued densities is given, inspired by quantum mechanics. 
%General Matrix-valued OT formulations are developed in \cite{ning2014matrix, ning2013thesis}. 
%\citet{peyre2016quantum} for SPD-valued OT problems and show the usefulness in various applications. It should be emphasized all of the above works rely on \emph{unbalanced} OT formulations.

% where one considers a trace-constrained relaxation for balancing the trace of the marginals \cite{ning2014matrix} and the other \cite{peyre2016quantum} applies a quantum relative entropy regularization to solve an {unbalanced} OT problem (i.e., the transport plan only approximately satisfy the coupling constraint).  


% \alertPJ{This paragaph should be expanded. No need to give dynamic vs static classification}
% \alertAH{The dynamic vs static are discussed in many papers we are referencing. This helps better compare our work to the others because our formulation is static and balanced.}


% \alertAH{When $F(\bGamma)$ is linear, such as in \eqref{reformulated_mw}, one can solve an unbalanced relaxation of the problem with quantum Sinkhorn algorithm \cite{peyre2016quantum}. However, optimization of \eqref{mot_define} in its generic form is challenging, particularly in the balanced setting. }

% \alertBM{The manifold motivation is missing. Why not cvx and why Riemannian.}

In this paper, we propose a general framework for solving the balanced OT problem between SPD-valued distributions, where the cost and the coupling are represented as block SPD matrices. We discuss a Riemannian manifold structure for the set of such block coupling matrices, and we are able to use the Riemannian optimization framework \cite{absil2009optimization, boumal2020intromanifolds} to solve various generalized OT problems. Specifically, our {contributions} as follows. 


% \alertPJ{Here, we could add a comment on the block-SPD nature of coupling (and maybe even cost function). After this description, we can discuss Riemannian manifold structure and optimization. Perhaps very similar to abstract flow. We can state Barycenter learning and GW generalization for SPD-valued measures in the contribution points rather than this paragraph.}

% This generalizes the matrix coupling manifold for scalar-valued densities \cite{shi2021coupling,mishra2021manifold}. 
% which proves its versatility in various non-classic scalar-valued optimal transport problems, such as Gromov-Wasserstein OT \cite{memoli2011gromov,peyre2016gromov}, Co-OT \cite{redko2020co}, regularized OT \cite{ferradans2014regularized}.   
\begin{enumerate}
    \item We introduce the general SPD matrix-valued balanced OT problem for block SPD marginals. We study the metric properties of the proposed formulation and discuss its relationship with the $2$-Wasserstein distance.
    %In the particular case when the SPD marginals are lifted versions of probability measures, the proposed formulation leads to a well-defined distance metric and that it generalizes the classic $2$-Wasserstein distance.
    
    \item We propose a novel manifold structure for the set of block matrix coupling matrices, which generalizes the manifold structures studied in \cite{douik2019manifold,shi2021coupling,mishra2021manifold,mishra2019riemannian}. We discuss optimization-related ingredients like Riemannian metric, Riemannian gradient, Hessian, and retraction.
    
    \item We extend our SPD-valued balanced OT formulation to block SPD Wasserstein barycenter and Gromov-Wasserstein OT.
    
    \item We empirically illustrate the benefit of the proposed framework in domain adaptation, tensor-valued shape interpolation, and displacement interpolation between tensor fields.
\end{enumerate}




\paragraph{Organizations.} 
We start with a brief review of optimal transport and Riemannian optimization in Section \ref{preliminary_sect}. In Section \ref{matrix_generalized_ot_sect}, we introduce the generalized SPD matrix-valued OT problem. Section \ref{manifold_geometry_sect} derives the necessary Riemannian optimization ingredients. Section \ref{sec:applications} develops two extensions to the matrix-valued OT problem. In Section \ref{Experiment_sect}, we test the proposed framework in various applications. In the appendix sections, we provide the proofs and show additional experiments. 



%\alertAH{preliminary as part of introduction?}

\section{Preliminaries}
\label{preliminary_sect}

\subsection{Optimal transport}
\label{ot_preliminary_sect}

Consider two discrete measures supported on $\sR^d$, $\mu = \sum_{i = 1}^m p_i \delta_{\bx_i}$, $\nu = \sum_{j = 1}^n q_j \delta_{\by_j}$, where $\bx_i, \by_j \in \sR^d$. The weights $\bp \in \Sigma_m, \bq \in \Sigma_n$ are in probability simplex, i.e., $\sum_i p_i = \sum_j q_j = 1$, for $p_i, q_j \geq 0$ and $\delta_\bx$ is the Dirac at $\bx$. The $2$-Wasserstein distance between $\mu, \nu$ is given by solving the Monge-Kantorovich optimal transport problem: 
% \alertPJ{Here source/target terminology and symbols $\bx_i$ and $\by_i$ are not defined.}
\begin{equation}
\label{W22}
    {\mathrm W}_2^2(\bp,\bq) = \min_{\bgamma \in \Pi(\bp,\bq)} \sum_{i,j} \|\bx_i-\by_j\|^2 \gamma_{i,j},
\end{equation}
where $\Pi(\bp,\bq) \coloneqq \{\bgamma \in \sR^{m \times n} : \bgamma \geq 0, \bgamma \bone = \bp, \bgamma^\top \bone = \bq  \}$ is the space of joint distribution between the source and
the target marginals. An optimal solution of (\ref{W22}) is referred to as an optimal transport plan (or coupling).  %the set of couplings with marginals $\bp$ and $\bq$. 
Recently, \citet{cuturi2013sinkhorn} proposed the Sinkhorn-Knopp  algorithm~\citep{sinkhorn1964relationship,knight2008sinkhorn} for entropy-regularized OT formulation. For a recent survey of OT literature and related machine learning applications, please refer to~\citep{peyre2019computational}. 

%Although \eqref{W22} can be solved via linear programming, the computational cost scales poorly with dimension $d$. In \citep{cuturi2013sinkhorn}, an entropy regularization is added to largely reduce the computational cost while pushing the solution away from the boundary. 
% Define the entropy of the coupling as $h(\bgamma) = - \sum_{i,j} \gamma_{i,j} \log(\gamma_{i,j}) + \gamma_{i,j}$. The entropy-regularized problem is 
% \begin{equation}
% \label{W22_reg}
%         _{\bgamma \in \Pi(\bp,\bq)} \sum_{i,j} \|\bx_i-\by_j\|^2 \gamma_{i,j} - \epsilon \, h(\bgamma).
% \end{equation}
%The solution to the regularized problem is unique and can be efficiently solved via the Sinkhorn-Knopp algorithm, originally designed for matrix balancing \citep{sinkhorn1964relationship}. 
% \alertPJ{This can be shortened to save space if required.}


% \paragraph{Matrix OT} brief literature review

% \alertAH{Already give a review in intro. No need to do it again because we do not rely on their formulation.}

\subsection{Riemannian optimization}%geometry and optimization}
A matrix manifold $\M$ is a smooth subset of the ambient vector space $\gV$ with local bijectivity to the Euclidean space. A Riemannian manifold is a manifold endowed with a Riemannian metric (a smooth, symmetric positive definite inner product structure $\langle \cdot, \cdot\rangle_x$) on every tangent space $T_x\M$. The induced norm on the tangent space is thus $\| u\|_x = \sqrt{\langle u,u \rangle_x}$. 
% {\color{red} Optimization of an objective function over a smooth Riemannian manifold $\M$ has gained attraction lately \citep{absil2009optimization, boumal2020intromanifolds}. Conceptually, the Riemannian optimization framework treats a constrained optimization problem as an unconstrained optimization problem over the constraint manifold. Consequently, all the standard unconstrained optimization methods such as steepest descent, conjugate gradient, and trust-region have their Riemannian variants \citep{boumal2020intromanifolds}. } \alertAH{Can this be removed or merged somehow?}

The orthogonal projection operation for an embedded matrix manifold ${\rm P}_{x}: \gV \xrightarrow{} T_x\M$ is a projection that is orthogonal with respect to the Riemannian metric $\langle \cdot, \cdot \rangle_x$. Retraction is a smooth map from tangent space to the manifold
% , which allows iterates to move on the manifold along some direction on the tangent space.
That is, for any $x \in \M$, retraction $R_x: T_x\M \xrightarrow{} \M$ such that 1) $R_x(0) = x$ and 2) $\D R_x(0)[u] = u$, where $\D f(x)[u]$ is the derivative of a function at $x$ along direction $u$. 

The Riemannian gradient of a function $F:\M \xrightarrow{} \sR$ at $x$, denoted as $\grad F(x)$ generalizes the notion of the Euclidean gradient, which is defined as the unique tangent vector satisfying $\langle \grad F(x) , u \rangle_x = \D F(x)[u] = \langle \nabla F(x) ,u\rangle_2$ for any $u \in T_x\M$. $\nabla F(x)$ is the Euclidean gradient and $\langle \cdot, \cdot\rangle_2$ denotes the Euclidean inner product. To minimize the function, Riemannian gradient descent \citep{absil2009optimization} and other first-order solvers apply retraction to update the iterates along the direction of negative Riemannian gradient while staying on the manifold, i.e., $x_{t+1} = R_{x_t}(-\eta \, \grad F(x_t))$, where $\eta$ is the step size. 
Similarly, the Riemannian Hessian $\hess F(x) : T_x\M \xrightarrow{} T_x\M$ is defined as the covariant derivative of Riemannian gradient. Popular second-order methods, such as trust regions and cubic regularized Newton's methods have been adapted to Riemannian optimization \citep{absil2007trust,agarwal2018adaptive}. 
% \alertPJ{This can be shortened to save space if required.}







% \subsection{Optimal transport and Riemannian geometry}
% Many work has constructed manifold geometry for either the coupling or the marginals. The set of (strictly positive) histograms form the so-called multinomial manifold with the Fisher information Riemannian metric \cite{sun2015heterogeneous}. This has later been generalized to simplex of SPD matrices where each simplex element is a SPD matrix \cite{mishra2019riemannian}. In \cite{douik2019manifold,shi2021coupling}, they construct a coupling manifold for the set of positive doubly stochastic couplings, further generalizing the multinomial manifold. All these works can be regarded as special cases of our proposed block SPD coupling manifold.






%\section{{\Manname}}
\section{Block SPD optimal transport}
\label{matrix_generalized_ot_sect}
%\alertPJ{Consider the same setting as in Section \ref{ot_preliminary_sect}.} 
%Let $\bp \in \Sigma_m$ and $\bq \in \Sigma_n$ be the given marginal distributions with supports given by the sets $\{\bx_i\}_{i=1}^m \in \sR^d$ and $\{\by_j\}_{j=1}^n \sR^d$, respectively. 

Consider the same setting as in Section \ref{ot_preliminary_sect}, with two given measures $\mu = \sum_{i = 1}^m p_i \delta_{\bx_i}$, $\nu = \sum_{j = 1}^n q_j \delta_{\by_j}$ and the marginals $\bp \in \Sigma_m$ and $\bq \in \Sigma_n$.

We consider \textit{lifting} the given probability measures to a space of matrix-valued measures where an associated \textit{mass} is represented as a positive semi-definite matrix. To this end, we convert the marginals $\bp$ and $\bq$ to block matrices $\bP$ and $\bQ$, where $\bP \coloneqq \{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$. Here, $[\cdot]_{m \times n}$ denotes a collection of $mn$ matrices organized as a block matrix and $\bI$ represents the identity matrix. 
The cost of transporting a positive semi-definite (matrix) mass $\bA$ from position $\bx_i$ to $\by_j$ is parameterized by a (given) positive semi-definite matrix $\bC_{i,j}$ and is computed as $\trace(\bC_{i,j}\bA)$. Under this setting, we propose a {block SPD matrix valued OT} problem as 
\begin{equation}
    {\rm MW}^2(\bP, \bQ) \coloneqq \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}), \label{reformulated_mw}
\end{equation}
where $\bGamma = [\bGamma_{i,j}]_{m \times n}$ is a block-matrix coupling of size $m \times n$ and the set of such couplings are defined as $\bPi(m,n,d,\bP, \bQ) \coloneqq \{ [\bGamma_{i,j}]_{m \times n} : \bGamma_{i,j} \in \sS_{+}^d, \sum_j \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} = \bQ_j, \forall i \in [m], j \in [n] \}$. Here $\sS_{+}^d$ is used to denote the set of $d\times d$ positive semi-definite matrices and $\trace(\cdot)$ is the matrix trace. With a slight abuse of notation, let ${\rm MW}(\bp, \bq)\coloneqq {\rm MW}(\bP, \bQ)$ with $\bP,\bQ$ defined above. Below we compare the generalized distance ${\rm MW}(\bp, \bq)$ to ${\rm W}_2(\bp, \bq)$ and analyze its metric properties. 


\paragraph{Relationship with ${\rm W}_2(\bp, \bq)$.} 
The $2$-Wasserstein distance ${\mathrm W}_2(\bp,\bq)$ considers the transportation cost of a unit mass from $\bx_i$ to $\by_j$ as $\|\bx_i-\by_j\|^2$, which can be rewritten as $\trace{((\bx_i -\by_j)(\bx_i - \by_j)^\top)}$. Hence, if we consider the cost for the proposed OT problem (\ref{reformulated_mw}) as $\bC_{i,j} = (\bx_i -\by_j)(\bx_i - \by_j)^\top$, then ${\rm MW}(\bp, \bq) = {\mathrm W}_2(\bp,\bq)$ where the optimal block-matrix coupling is $\bGamma^* = \bgamma^* \otimes \bI$ where $\bgamma^*$ is the optimal coupling for ${\rm W}_2(\bp, \bq)$ and $\otimes$ is the Kronecker product.


\paragraph{Metric properties of ${\rm MW}(\bp, \bq)$.} 
% For given marginals $\bp\in\Sigma_m$ and $\bq\in\Sigma_n$, let the corresponding block SPD marginals $\bP$ and $\bQ$ be defined as $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$. 
In the following proposition, we formalize the conditions under which ${\rm MW}(\bp, \bq)$ is a valid distance metric.
\begin{proposition}
\label{mw_distance_prop}
Suppose the marginals $\bp, \bq \in \Sigma_n$ have the same support and the costs $\{\bC_{i,j}\}_{i,j=1}^n$ satisfy
\begin{enumerate}
    \item $\bC_{i,j}=\bC_{j,i}$ and
    \item $\bC_{i,j}\succ\bzero$ for $i\neq j$ and $\bC_{i,j}=\bzero$ for $i=j$,
%    \item $\bC_{i,j}=\bzero$ if and only if $i=j$
    \item $\forall (i,j,k)\in [n]^3,$ and $ \bA\succeq \bzero,$ $\sqrt{\trace( \bC_{i,j} \bA)} \leq \sqrt{\trace( \bC_{i,k} \bA)} + \sqrt{\trace(  \bC_{j,k}  \bA)}$.
\end{enumerate}
Then, ${\rm MW}(\bp, \bq)$ is a metric between the marginals $\bp$ and~$\bq$. 
\end{proposition}

We remark that the conditions on $\bC_{i,j}$ in Proposition \ref{mw_distance_prop} generalize the conditions required for ${\rm W}_2(\bp, \bq)$ in \eqref{W22} to be a metric. See for example \citep[Proposition 2.2]{peyre2019computational}. In Appendix \ref{cost_choice_appendix}, we discuss some particular constructions of the cost that satisfy the conditions.



%\paragraph{Generalized block matrix-valued optimal transport.}
The previous discussion on ${\rm MW}(\bp, \bq)$ motivates the generalized SPD matrix valued OT problem \eqref{reformulated_mw} where the marginals are arbitrary positive semi-definite matrix mass. That is, $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i \in \sS_{+}^d\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bP_i \in \sS_{+}^d\}$ and $\bP$ and $\bQ$ have the same total mass. Without loss of generality, we assume $\sum_i \bP_i = \sum_j \bQ_j = \bI$. The problem is well-defined provided that the corresponding coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ is non-empty. This is discussed in Section \ref{manifold_geometry_sect}.

% The generalized OT problem has been considered for tensor field processing \cite{peyre2016quantum}, image color interpolation . 



% \alertPJ{\paragraph{Relationship with existing matrix OT problems.} A few works }
% \alertAH{Not sure how? I have somehow discuss this in introduction.}

In the next section, we analyze the coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ and show that it can be endowed with a manifold structure. This allows to exploit the versatile Riemannian optimization framework to solve (\ref{reformulated_mw}) and any more general problem \citep{absil2009optimization}. 

% \alertAH{We emphasize that this formulation departs substantially from the existing work where the solutions rely on entropy regularization.}

% \alertAH{(How to better compare with the existing work?)}

% We analyze $\bPi(m,n,d,\bP, \bQ)$ in this setting in Section~\ref{manifold_geometry_sect}.


% \alertAH{The marginals $\bP$ and $\bQ$ should have the same total mass and without loss of generality, we assume $\sum_i \bP_i = \sum_j \bQ_j = \bI$.} 

% It should be noted that the proposed OT problem \eqref{reformulated_mw} is well-defined for the general setting $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i \in \sS_{+}^d\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bP_i \in \sS_{+}^d\}$ if $\sum_i \bP_i = \sum_j \bQ_j$ and \alertAH{the corresponding block SPD coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ is non-empty. We analyze $\bPi(m,n,d,\bP, \bQ)$ in this setting in Section~\ref{manifold_geometry_sect}.} 

% \alertPJ{In Section~\ref{sec:applications}, we discuss the proposed \alertPJ{matrix-valued} OT (\ref{reformulated_mw}) for domain adaptation application and provide common costs that satisfy the conditions stated in Proposition~\ref{mw_distance_prop}. }

% \begin{proposition}
% \label{mw_distance_prop}
% Given histograms $\bp, \bq \in \Sigma_n$, define the {cost} $\bC_{i,j} = (\bX_i - \bY_j) (\bX_i -\bY_j)^\top \succ \bzero$ for $\bX_i \neq \bY_j$, where $\{ \bX_i \}, \{ \bY_j\} \subset \sR^{d \times s}$. Then,
% ${\rm MW}(\bp, \bq)$ is a metric between the marginals $\bp$ and $\bq$. 
% \end{proposition} %supported on $\sR^{d \times s} (s \geq d)$
%The condition that $s \geq d$ in the above proposition ensures $\bC_{i,j} \succ \bzero$ for $\bX_i \neq \bY_j$. For general positive semi-definite {cost} $\bC_{i,j} \succeq \bzero$ for {$i \neq j$} (as for the vector-valued samples), ${\rm MW}(\bp, \bq)$ is a pseudo-metric where it may happen that ${\rm MW}(\bp, \bq) = 0$ for $\bp \neq \bq$. 

%\subsection{Properties of ${\rm MW}^2(\bP, \bQ)$}






% In the following Section~\ref{manifold_geometry_sect}, we analyze the coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ and show that it can be endowed with a manifold structure. Specifically, we consider the following \alertPJ{set}, 
% %propose the following Riemannian manifold structure, 
% termed as the {\manname}, 
% \begin{equation}\label{eq:manifold_proposed}
% \begin{array}{ll}
%     \M_{m,n}^d(\bP, \bQ) 
%     \coloneqq \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \\
%     \qquad \qquad \qquad \sum_{j} \bGamma_{i,j} = \bP_i, 
%      \sum_i \bGamma_{i,j} =\bQ_j \},
% \end{array}
% \end{equation}
% where we restrict $\bGamma_{i,j} \in \sS_{++}^d$ to be in the set of symmetric positive definite (SPD) matrices. This ensures that the proposed \alertPJ{set} 
% %manifold 
% $\M_{m,n}^d(\bP, \bQ)$ in (\ref{eq:manifold_proposed}) is the interior of the set $\bPi(m,n,d,\bP, \bQ)$.


% We begin by considering an equivalent reformulation of the objective in classic OT problem \eqref{W22} as
% \begin{equation*}
%     \min_{\bGamma \, : \, \bGamma_{i,j} = \gamma_{i,j} \bI, \bgamma \in \Pi(\bp, \bq)} \sum_{i,j} \trace\left((\bx_i-\by_j)(\bx_i-\by_j)^\top \bGamma_{i,j} \right),
% \end{equation*} 
%  \alertPJ{Should we state here $\sS_{+}^d$? Should we state marginals also as scalar times Identity matrix here itself? It will motivate (3) as a more direct generalization of the above - as only the constraints on $\bGamma_{i,j}$ need to be relaxed.}

% Next we define $\bP_i = p_i \bI_d$, $\bQ_j = q_j \bI_d$, and a block matrix coupling set as $\bPi(m,n,d,\bP, \bQ) := \{ \bGamma : \bGamma_{i,j} \in \sS_{+}^d, \sum_j \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} = \bQ_j, \forall i \in [m], j \in [n] \}$, where $\sS_{+}^d$ is the set of $d\times d$ positive semi-definite matrices and $[a] = \{1, ..., a \}, a \geq 1$. It is observed that the constraint set of the classic OT problem is a subset of $\bPi(m,n,d,\bP, \bQ)$ with uniform diagonal block. It, thus, becomes natural to consider a generalized matrix Wasserstein distance with the relaxed constraint set:

% where $\bC_{i,j} = (\bx_i - \by_j)(\bx_i - \by_j)^\top$. It is easy to verify the optimal solution for the classic OT problem \eqref{W22} is a feasible solution for the proposed generalized OT problem \eqref{reformulated_mw}. 

% Such a formulation now motivates us to consider a more general problem as 




% \paragraph{Relationship with existing manifolds.} 
% We note that the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ can be regarded as a generalization to existing manifold structures. For example, when $d =1$ and either $m=1$ or $n=1$, the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ reduces to the multinomial manifold of probability simplex  \citep{sun2015heterogeneous}. When $d=1$ while $m, n \neq 1$, $\M_{m,n}^d(\bP, \bQ)$ becomes the so-called matrix coupling manifold \citep{shi2021coupling}. When $d=1$ while $m, n \neq 1$, but $m = n$ and $\bP$ and $\bQ$ are uniform, $\M_{m,n}^d(\bP, \bQ)$ reduced to the doublystochastic manifold \citep{douik2019manifold}. When $d > 1$ while either $m =1$ or $n =1$, our manifold simplifies to the simplex manifold of SPD matrices \citep{mishra2019riemannian}.







% With such a manifold structure, one can utilize Riemannian optimization to solve any generic problem in the form of 

% \begin{equation}
%     \min_{\bGamma \in \bPi(m,n,d,\bP, \bQ)} F(\bGamma), \label{mot_define}
% \end{equation}
% where $F : \bPi(m,n,d,\bP, \bQ) \xrightarrow{} \sR$ is a block-wise and possibly nonlinear loss function. 




% \paragraph{Relationship of ${\rm MW}^2$ and ${\mathrm W}_2^2$.}
% When the marginals are given by $\bP_i = p_i \bI, \bQ_j = q_j \bI$, the cost matrix is $\bC_{i,j} = (\bx_i -\by_j)(\bx_i - \by_j)^\top$, and we constrain $\bGamma_{i,j} = \gamma_{i,j} \bI$, the matrix generalized Wasserstein distance \eqref{reformulated_mw} is identical to the $2$-Wasserstein distance \eqref{W22}. The formulation in \eqref{reformulated_mw}, therefore, is more general than \eqref{W22}.






% To solve for the block matrix OT problem in \eqref{mot_define}, one can consider  This is mainly due to the fact that the constraint set might be empty for arbitrary SPD-valued marginals, even with $\sum_{i = 1} \bP_i = \sum_{j = 1} \bQ_j$. 

% \alertPJ{We don't have a smooth story here. We should improve it. I too dont have a clear vision as of now.}








\section{{\Manname}}
%\section{Riemannian optimization}
\label{manifold_geometry_sect}

%In this section, we analyze the coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ and show that it can be endowed with a manifold structure. Specifically, 
We propose the following Riemannian manifold structure, 
termed as the {\manname}, 
\begin{equation}\label{eq:manifold_proposed}
\begin{array}{ll}
    \M_{m,n}^d(\bP, \bQ) 
    \coloneqq \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \\[3pt]
    \qquad \qquad \qquad \sum_{j} \bGamma_{i,j} = \bP_i, 
     \sum_i \bGamma_{i,j} =\bQ_j \},
\end{array}
\end{equation}
where $\sum_i \bP_i = \sum_j \bQ_j = \bI$. Particularly, we restrict $\bP_i, \bQ_j,\bGamma_{i,j} \in \sS_{++}^d$, the set of SPD matrices. This ensures that the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ in (\ref{eq:manifold_proposed}) is the interior of the set $\bPi(m,n,d,\bP, \bQ)$.




For arbitrary SPD marginals $\bP, \bQ$, there is no guarantee that the set $\M_{m,n}^d(\bP, \bQ)$ defined in (\ref{eq:manifold_proposed}) is non-empty \citep{ning2014matrix}. Hence, we assume the following.
\begin{assumption}\label{assumption:existence}
The block-SPD marginals $\bP$ and $\bQ$ are chosen such that there exists at least one element in the set $\M_{m,n}^d(\bP, \bQ)$.
\end{assumption}
It should be noted that Assumption \ref{assumption:existence} can be easily satisfied for various types of block-SPD marginals such as uniform or arbitrary positive diagonal marginals. 




\begin{algorithm}[t]
 \caption{Riemannian optimization for solving (\ref{eq:manifold_problem}).}
 \label{Riemannian_optimizer}
 \begin{algorithmic}[1]
 \STATE Initialize a feasible $\bGamma \in \M_{m,n}^d$.
  \WHILE{not converging}
  \STATE Compute Riemannian gradient (and Hessian) at $\bGamma$.
  \STATE Compute the update step $\bxi \in T_{\bGamma} \M_{m,n}^d$.
%   \STATE 
%   \hspace*{0.8em} \textbullet \,\, (RSD) $\bxi = -\eta \, \grad F(\bGamma^{t-1})$. \newline
%          \hspace*{0.8em} \textbullet \,\, (RCG) conjugate direction of $\grad F(\bGamma^{t-1})$. \newline
%          \hspace*{0.8em} \textbullet \,\, (RTR) solving trust region subproblem.
   \STATE Update $\bGamma \leftarrow R_{\bGamma}(\bxi)$.
  \ENDWHILE
%   \STATE \textbf{Output:} $\bGamma$.
 \end{algorithmic} 
\end{algorithm}




\begin{proposition}
\label{smooth_set_prop}
Under Assumption \ref{assumption:existence}, the set $\M^d_{m,n}(\bP, \bQ)$ is smooth, i.e., differentiable.
\end{proposition}

Proposition \ref{smooth_set_prop} implies that we can endow $\M^d_{m,n}(\bP, \bQ)$ with a Riemannian structure (introduced in Section \ref{Riem_opt_sec}). 

%\paragraph{Relationship with existing manifolds.} 
It should be emphasized that the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ can be regarded as a generalization to existing manifold structures. For example, when $d =1$ and either $m=1$ or $n=1$, $\M_{m,n}^d(\bP, \bQ)$ reduces to the multinomial manifold of probability simplex  \citep{sun2015heterogeneous}. When $d=1$ and $m, n \neq 1$, it reduces the so-called doubly stochastic manifold \citep{douik2019manifold} with uniform marginals or the more general matrix coupling manifold \citep{shi2021coupling}. When $d > 1$ and either $m =1$ or $n =1$, our proposed manifold simplifies to the simplex manifold of SPD matrices \citep{mishra2019riemannian}.

% When $d=1$ while $m, n \neq 1$, but $m = n$ and $\bP$ and $\bQ$ are uniform, $\M_{m,n}^d(\bP, \bQ)$ reduces to the doubly stochastic manifold \citep{douik2019manifold}. 



Below, we derive various optimization-related ingredients on $\M_{m,n}^d(\bP, \bQ)$ that allow optimization of an arbitrary differentiable objective function on the manifold. It follows the general treatment proposed by \citep{absil2009optimization}.


% We define the \manname \, as 
% \begin{align*}
%     &\M_{m,n}^d(\bP, \bQ) \\
%     &:= \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \sum_{j} \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} =\bQ_j \},
% \end{align*}
% where we restrict $\bGamma_{i,j} \in \sS_{++}^d$, the set of symmetric positive definite (SPD) matrices. This ensures that $\M_{m,n}^d(\bP, \bQ)$ is the interior of the set $\bPi(m,n,d,\bP, \bQ)$. Without loss of generality, we assume $\sum_i \bP_i = \sum_j \bQ_j = \bI$.

\subsection{Riemannian geometry and optimization on $\M_{m,n}^d$}
\label{Riem_opt_sec}

% \alertPJ{(this subsection should focus on optimization only)}
We consider the general problem
\begin{equation}
    \min_{\bGamma \in \M_{m,n}^d(\bP, \bQ)} F(\bGamma) \label{eq:manifold_problem}
\end{equation}
via the Riemannian optimization framework. It provides a principled class of optimization methods and computational tools for manifolds, both first order and second order, as long as the ingredients such as Riemannian metric, orthogonal projection, retraction, and Riemannian gradient (and Hessian) of a function are defined \citep{absil2009optimization, boumal2014manopt, boumal2020intromanifolds}. Conceptually, the Riemannian optimization framework treats (\ref{eq:manifold_problem}) as an ``unconstrained'' optimization problem over the constraint manifold $\M_{m,n}^d$ (omitted marginals $\bP$, $\bQ$ for clarity).

In Algorithm \ref{Riemannian_optimizer}, we outline the skeletal steps involved in optimization over $\M_{m,n}^d$, where the step $\bxi$ can be computed from different Riemannian methods. In Riemannian steepest descent, $\bxi = -\eta \, \grad F(\bGamma)$, where $\grad F(\bGamma)$ is the Riemannian gradient at $\bGamma$. Also, $\bxi$ is given by the ``conjugate'' direction of $\grad F(\bGamma)$ in the Riemannian conjugate gradient method. And, for the Riemannian trust-region method, $\bxi$ computation involves minimizing a second-order approximation of the objective function in a trust-region ball
\citep{absil2009optimization}. Below, we show the computations of these ingredients.












% \subsection{Riemannian metric}
\paragraph{Riemannian metric.} 
% \alertPJ{Can this be moved up to before Section 4.1?} 
The manifold $\M^d_{m,n}$ is a submanifold of the Cartesian product of $m \times n$ SPD manifold of size $d \times d$, which we denote as $\bigtimes_{m, n} \sS_{++}^d$. The dimension of the manifold $\M^d_{m,n}$ is $(m-1)(n-1)d(d+1)/2$. The {tangent space} characterization of $\M_{m,n}^d$ at $\bGamma$ is given by
\begin{align*}
    &T_\bGamma \M_{m,n}^d \\
    &= \{ [\bU_{i,j}]_{m \times n}: \bU_{i,j} \in \sS^d, \sum_{j} \bU_{i,j} = \bzero, \sum_{i} \bU_{i,j} = \bzero\},
\end{align*}
where $\sS^d$ is the set of $d \times d$ symmetric matrices. We endow each SPD manifold with the affine-invariant Riemannian metric \citep{bhatia2009positive}, which induces a {Riemannian metric} for the product manifold $\M_{m,n}^d$ as
\begin{equation}
    \langle \bU, \bV \rangle_\bGamma = \sum_{i,j} \trace(\bGamma_{i,j}^{-1} \bU_{i,j} \bGamma^{-1}_{i,j} \bV_{i,j}), \label{Riem_metric}
\end{equation}
for any $\bU, \bV \in T_{\bGamma} \M_{m,n}^d$. 

%\GaoC{Better to use $\Gamma_{i,j}$ instead of $\mathbf X_{i,j}$ for notation consistence?}


% \subsection{Orthogonal projection, Riemannian gradient, and Hessian}
\paragraph{Orthogonal projection, Riemannian gradient, and Riemannian Hessian.}
As an embedded submanifold, the orthogonal projection plays a crucial role in deriving the Riemannian gradient (as orthogonal projection of the Euclidean gradient in the ambient space). 

\begin{proposition}
\label{orthogonal_proj}
The orthogonal projection of any $\bS \in \bigtimes_{m, n} \sS^d$ to $T_\bGamma\M_{m,n}^d$ with respect to the Riemannian metric \eqref{Riem_metric} is given by 
\begin{equation*}
     {\rm P}_{\bGamma}(\bS) = \bU, \text{ with } \bU_{i,j} = \bS_{i,j} + \bGamma_{i,j} (\bLambda_i+ \bTheta_j) \bGamma_{i,j},
\end{equation*}
where auxiliary variables $\bLambda_i, \bTheta_j$ are solved from the system of matrix linear equations:
\begin{equation*}
\begin{cases}
    -\sum_i \bS_{i,j} = \sum_{i} \bGamma_{i,j} (\bLambda_i + \bTheta_j) \bGamma_{i,j}, & \forall j \\
    -\sum_j \bS_{i,j} = \sum_{j} \bGamma_{i,j} (\bLambda_i + \bTheta_j) \bGamma_{i,j}, & \forall i.
\end{cases}
\end{equation*}
\end{proposition}


Subsequently, the Riemannian gradient and Hessian are derived as the orthogonal projection of the gradient and Hessian from the ambient space. 

\begin{proposition}
\label{Riem_grad_hess}
The Riemannian gradient and Hessian of $F: \M_{m\times n}^d \xrightarrow{} \sR$ are derived as 
\begin{align*}
    \grad F(\bGamma) &= {\rm P}_\bGamma([\bGamma_{i,j} \{ \nabla F(\bGamma_{i,j}) \}_{\rm S} \bGamma_{i,j}]_{m\times n}),\\
    \hess F(\bGamma)[\bU] &= {\rm P}_\bGamma([\D \grad F(\bGamma_{i,j})[\bU_{i,j}]\\
    &\quad - \{ \bU_{i,j} \bGamma_{i,j}^{-1} \grad F(\bGamma_{i,j}) \}_{\rm S}]_{m\times n}),
\end{align*}
where $\bU \in T_\bGamma\M_{m,n}^d$ and $\nabla F(\bGamma_{i,j})$ is the block partial derivative of $F$ with respect to $\bGamma_{i,j}$. Here, $\D \grad F(\bGamma_{i,j})[\bU_{i,j}]$ denotes the directional derivative of the Riemannian gradient $\grad F$ along $\bU$ and $\{ \bA\}_{\rm S} \coloneqq (\bA + \bA^\top)/2$.
\end{proposition}


% \subsection{Retraction and block matrix balancing algorithm}
% \label{retraction_sinkhorn}

\paragraph{Retraction and block matrix balancing algorithm.}
Retraction of $\M_{m, n}^d$ is given by a composition of two operations. The first operation is to ensure positive definiteness of the blocks in the coupling matrix. In particular, we use the exponential map associated with the affine-invariant metric on the SPD manifold $\sS_{++}^d$ \citep{bhatia2009positive}. The second operation is to ensure that the summation of the row blocks and column blocks respect the block-SPD marginals. Given an initialized block SPD matrix $[\bA_{i,j}]_{m \times n}$, where $\bA_{i,j} \in \sS_{++}^d$, the goal is to find a `closest' block SPD coupling matrix $\bB \in \M_{m,n}^d$. The is achieved by alternatively normalizing the row and column blocks to the corresponding marginals. The procedure is outlined in Algorithm~\ref{bmb_algorithm}. The solution for the row and column normalization factors $\bR_j, \bL_i$, which are SPD matrices, are computed by solving the Riccati equation $\bT \bX \bT = \bY$ for given $\bX, \bY \in \sS_{++}^d$. Here, $\bT$ admits a unique solution \citep{bhatia2009positive,malago2018wasserstein}. Different from the scalar marginals case where the scaling can be expressed as a diagonal matrix, we need to symmetrically normalize each SPD block matrix. Algorithm~\ref{bmb_algorithm} is a generalization of the RAS algorithm for balancing non-negative matrices \cite{sinkhorn1967diagonal}, which is related to the popular Sinkhorn-Knopp algorithm \citep{sinkhorn1964relationship,knight2008sinkhorn}. 

It should be noted that a similar matrix balancing algorithm has been introduced for positive operators \cite{gurvits2004classical,georgiou2015positive}, where the convergence is only established in limited cases. Algorithm~\ref{bmb_algorithm} is different from the quantum Sinkhorn algorithm proposed in \cite{peyre2016quantum} that applies to the {unbalanced} setting. Although we do not provide a theoretical convergence analysis for Algorithm \ref{bmb_algorithm}, we empirically observe quick convergence of this algorithm in various settings (see Appendix \ref{convergence_bmb_retr_appendix}).

% \alertAH{It can be seen that Algorithm~\ref{bmb_algorithm} is a generalization of the popular Sinkhorn-Knopp algorithm \citep{knight2008sinkhorn} which deals with non-negative scalar entries (instead of SPD blocks).}

% \alertAH{RAS algorithm}


% {Here we overload the notation $\sS_{++}^d$ to mean both the set of SPD matrices and SPD manifold with the AI metric.} 
% which is $\bX \exp(\bX^{-1} \bU)$ for any $\bX \in \sS_{++}^d, \bU \in T_\bX\sS_{++}^d$. The $\exp(\cdot)$ denotes matrix exponential.




% \begin{algorithm}[H]
%  \caption{Block matrix balancing algorithm}
%  \label{bmb_algorithm}
%  \begin{algorithmic}[1]
%   \STATE Initialize $\bA_{i,j}^0 = \bA_{i,j}$.
%   \FOR{$t = 1, \ldots, T$}
%   \STATE Find $\bR_j^{t-1}$ such that $\sum_i \bR_j^{t-1} \bA_{i,j}^{t-1} \bR_j^{t-1} = \bQ_j$, $\forall j$.
%   \STATE Update $\bA_{i,j}^{t-1} \xleftarrow{} \bR_j^{t-1} \bA_{i,j}^{t-1} \bR_j^{t-1}$, $\forall j$. 
%   \STATE Find $\bL_i^{t-1}$ such that $\sum_j \bL_i^{t-1} \bA_{i,j}^{t-1} \bL_i^{t-1} = \bP_i$, $\forall i$.
%   \STATE Update $\bA_{i,j}^t \xleftarrow{} \bL_i^{t-1} \bA_{i,j}^{t-1} \bL_i^{t-1}, \forall i$. 
%   \ENDFOR
%  \end{algorithmic} 
% \end{algorithm}


\begin{algorithm}[t]
 \caption{Block matrix balancing algorithm}
 \label{bmb_algorithm}
 \begin{algorithmic}[1]
  \STATE \textbf{Input:} $[\bA_{i,j}]_{m \times n}$, where $\bA_{i,j} \in \sS_{++}^d$.
  \WHILE{not converging}
  \STATE Find $\bR_j \in \sS_{++}^d$ such that $\sum_i \bR_j \bA_{i,j} \bR_j = \bQ_j$, $\forall j$.
  \STATE Update $\bA_{i,j} \xleftarrow{} \bR_j \bA_{i,j} \bR_j$, $\forall j$. 
  \STATE Find $\bL_i \in \sS_{++}^d$ such that $\sum_j \bL_i \bA_{i,j} \bL_i = \bP_i$, $\forall i$.
  \STATE Update $\bA_{i,j} \xleftarrow{} \bL_i \bA_{i,j} \bL_i, \forall i$. 
  \ENDWHILE
  \STATE \textbf{Output:} The balanced matrix $\bB = \bA$.
 \end{algorithmic} 
\end{algorithm}






Based on Algorithm \ref{bmb_algorithm}, we define a retraction $R_\bGamma(\bU)$ at $\bGamma \in  \M_{m, n}^d$ for any $\bU \in T_\bGamma \M_{m,n}^d$ as
\begin{equation}
    R_\bGamma(\bU) = {\rm MBalance} \big([\bGamma_{i,j} {\rm exp}(\bGamma_{i,j}^{-1} \bU_{i,j})]_{m \times n} \big), \label{retr_define}
\end{equation}
where {\rm MBalance} calls the matrix balancing procedure in Algorithm~\ref{bmb_algorithm} and $\exp(\cdot)$ denotes the matrix exponential. The retraction proposed in \eqref{retr_define} is valid (i.e., satisfy the two conditions) for diagonal marginals and empirically we also see the retraction is well-defined for arbitrary block-SPD marginals. See Appendix \ref{convergence_bmb_retr_appendix} for more details. 

% \alertPJ{Is our matrix balancing algorithm similar-to/different-from quantum Sinkhorn algorithm?}



% When each block $\bA_{i,j} \in \sR$ is a positive scalar, i.e. $d = 1$, Sinkhorn's Theorem \cite{sinkhorn1964relationship} proves that the balanced matrix $\bB$ has a standard form $\bB = \bD_1 \bA \bD_2$ for diagonal matrices $\bD_1, \bD_2$. The convergence of the balancing algorithm can be easily established. 

% However, when $d > 1$, proving convergence of Algorithm \ref{bmb_algorithm} is challenging given we need to symmetrically normalize each block. Further, finding the standard form of the balanced block matrix is nontrivial. Nevertheless, we assume a standard form of the resulting block matrix as $\bB_{i,j} = \tilde{\bL}_i \tilde{\bR}_j \bA_{i,j} \tilde{\bR}_j \tilde{\bL}_i$ (or $\tilde{\bR}_j \tilde{\bL}_i \bA_{i,j} \tilde{\bL}_i \tilde{\bR}_j$) $\forall i,j$.

% This assumption is needed to establish a valid retraction based on Algorithm \ref{bmb_algorithm}. 
% Although no theoretical analysis is given, we observe quick empirical convergence of the balancing algorithm, which is illustrated in Figure ..., with randomly generated SPD marginals and block identity initialization.








% \alertAH{The convergence analysis is referred to the Riemannian optimization. However, it seems abrupt to directly move from retraction to convergence for Riemannian optimization.}

\subsection{Convergence and computational complexity}
\label{convergence_complexity_sect}
\paragraph{Convergence of Riemannian optimization.}
Similar to Euclidean optimization, the necessary first-order optimality condition for any differentiable $F$ on $\M_{m,n}^d$ is $\grad F(\bGamma^*) = 0$, i.e., where the Riemannian gradient vanishes. We call such $\bGamma^*$ the stationary point. The Riemannian methods are known to converge to a stationary point \citep{absil2009optimization,boumal2020intromanifolds} under standard assumptions. Additionally, we show the following.


% This suggests that for the matrix-valued OT problem with convex regularization, the global optimal solution can always be guaranteed by Riemannian optimization. 


\begin{theorem}
\label{Prop_Riem_opt_optimal}
Suppose the objective function of the problem $\min_{\bGamma \in \bPi(m,n,d,\bP, \bQ)} F(\bGamma)$ is (strictly) convex and the optimal solution $\bGamma^*$ is positive definite, i.e., it lies in the interior of $\bPi(m,n,d, \bP, \bQ)$. Then, Riemannian optimization (Algorithm~\ref{Riemannian_optimizer}) for (\ref{eq:manifold_problem}) converges to the same global optimal solution $\bGamma^*$. 
% \alertBM{rephrase this properly}
\end{theorem}
% \begin{proof}
% The main idea is to write out the Riemannian gradient at optimality, which we show coincides with the KKT optimality conditions of (\ref{mot_define}). See Appendix \ref{proof_sect} for more details. 
% \end{proof}
Theorem \ref{Prop_Riem_opt_optimal} guarantees the quality of the solution obtained by Riemannian optimization for a class of objective functions which includes the SPD matrix-valued OT problem with convex regularization.


% \subsection{Computational complexity}
\paragraph{Computational complexity.}
The complexity of each iteration of the Riemannian optimization algorithm is dominated by the computations of retraction, the Riemannian gradient, the Riemannian Hessian. These also make use of the orthogonal projection operation. All these operations cost $O(mnd^3)$. It should be noted that the number of parameters to be learned is $mnd^2$.

% \alertAH{We develop (in Appendix \ref{proj_appendix}) a projected variant of problem \eqref{eq:manifold_problem} by simultaneously optimizing a projection matrix and the coupling in a low-dimensional space. Suppose the space is of dimension $r$ (with $r \ll d$). We show the complexity can be reduced to $O(mnr^3 + d^2r)$.}



% The retraction defined in (\ref{retr_define}) costs $O(mnd^3)$. To compute the Riemannian gradient, we need to evaluate the orthogonal projection as in Proposition \ref{orthogonal_proj}, which costs $O(mnd^3)$ for solving the systems of matrix linear equations. For methods which make use of Hessian information, an additional directional derivative of the Riemannian gradient is required which costs $O(mnd^3)$.
















%\section{Block SPD coupling matrix and optimal transport}
%\section{Barycenter learning and Gromov-Wasserstein discrepancy}
\section{Extensions of block SPD optimal transport}
In this section, we discuss extensions of the proposed SPD OT framework to Wasserstein barycenters and the Gromov-Wasserstein setting. 
%\section{Applications \alertAH{(better title needed)}}
\label{sec:applications}
%In this section, we consider the application of 



% \subsection{Matrix generalized Wasserstein distance}

% We first analyze the metric property of the generalized matrix Wasserstein distance introduced in Section \ref{matrix_generalized_ot_sect}:
% \begin{equation}
%     {\rm MW}^2(\bP, \bQ) = \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}). \label{MW_mot_restate}
% \end{equation}
% With a slight abuse of notation, we denote ${\rm MW}(\bp, \bq)$ as the matrix Wasserstein distance between $\bP, \bQ$ where $\bP_i = p_i \bI, \bQ_j = q_j \bI$ for $\bp, \bq$ in probability simplex. 

% We show in the following proposition that ${\rm MW}(\bp, \bq)$ is a valid distance metric between the discrete measures $\bp, \bq$ provided we construct $\bC_{i,j}$ to be strictly positive definite for $i \neq j$.

% \begin{proposition}
% \label{mw_distance_prop}
% Given $\bp, \bq \in \Sigma_n$ and the cost matrix $\bC_{i,j} \succ \bzero$ for $i \neq j$ and $\bC_{i,j} = \bzero$ for $i = j$, ${\rm MW}(\bp, \bq)$ is a metric between histograms $\bp, \bq$.
% \end{proposition}

% For general semidefinite cost matrix $\bC_{i,j} \succeq \bzero$ for $i \neq j$, ${\rm MW}(\bp, \bq)$ is a pseudo metric where it may happen that ${\rm MW}(\bp, \bq) = 0$ for $\bp \neq \bq$. 



% In Section \ref{matrix_generalized_ot_sect}, we show how the matrix Wasserstein distance is generalized from classic Wasserstein distance: 
% \begin{equation*}
%     {\rm MW}^2(\bp, \bq) := \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}), 
% \end{equation*}

% However, because the matrix cost $\bC_{i,j}$ is a rank-1 semi-definite matrix, the generalized matrix Wasserstein distance ${\rm MW}(\bp, \bq)$ fails to be a valid distance as it does not satisfy the definiteness property. Nevertheless, we show that when $\bC_{i,j}$ is strictly positive definite for $i \neq j$, ${\rm MW}(\bp, \bq)$ is a valid distance metric.




% In this section, we develop various applications and extensions that involve optimization with respect to a block doubly stochastic matrix. We show how our proposed unified framework can be applied in all the settings. 







% \subsection{Barycentric projection for Block SPD OT}

% \label{matrix_domain_adaptation}
% \alertPJ{No need of this section, we need to shift the expression to Section 6.4. Note that useful expression for barycentric projection is available only for a few cost functions, e.g., W22 for scalar OT. Hence, we can discuss our  exact expression in Section 6.4 itself. }

% The optimal transport framework has been popularly explored in unsupervised domain adaptation problems \alertPJ{references} as it exploits the geometry of the underlying metric space to provide distances between the source and the target distributions even when the supports of these distributions do not overlap. The barycentric projection expression for the $2$-Wasserstein OT setting (\ref{W22}) is well-known. 
% Here, we discuss the computation of unsupervised mapping (barycenter projection) of source points in the target domain. 

% Given the source samples $\{ \bX_i \}_{i = 1}^m$, and the target $\{ \bY_j \}_{j = 1}^n$, with $\bX_i, \bY_j \in \sR^{d \times s}$. We define a matrix-valued cost as $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$, which can be viewed as a cross-covariance between the samples. 


% \begin{proposition}
% When $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$, ${\rm MW}(\bp, \bq)$ is a distance metric. 
% \end{proposition}




% Domain adaptation first searches for an optimal coupling by solving problem \eqref{MW_mot_restate}. From Theorem \ref{Prop_Riem_opt_optimal}, we can use Riemannian framework developed in Section \ref{manifold_geometry_sect} to optimize the coupling. Then the source samples are projected to align with the target, a process known as \textit{barycentric projection}.


% With the optimal coupling $\bGamma_{i,j}^*$, barycentric projection of the source $\{\bX_i\}$ is computed as
% \begin{equation*}
%     \hat{\bX}_i = \argmin_{\bX_i \in \sR^{d\times s}} \sum_{i,j} \trace \big( (\bX_i - \bY_j)(\bX_i - \bY_j)^\top \bGamma_{i,j}^* \big).
% \end{equation*}
% From the first order condition, we have 
% \begin{equation}
%     \hat{\bX}_i = \bP_i^{-1}(\sum_j \bGamma_{i,j}^* \bY_j), \quad \forall i. \label{barycentric_proj}
% \end{equation}
% The projected samples $\{ \hat{\bX}_i\}$ follow the same distribution as the target samples $\{ \bY_j\}$. When the samples are structured, i.e. symmetric and even semidefinite, barycentric projection can be similarly derived. For symmetric $\bX_i, \bY_j \in \sS_{+}^d$, the projected source samples $\hat{\bX}_i$ are now the symmetric solution to the Lyapunov equation: $\{ \bP_i \hat{\bX}_i \}_{\rm S} = \{\sum_j \bGamma^*_{i,j} \bY_j\}_{\rm S}$.  














\subsection{Block SPD Wasserstein barycenter learning}
\label{block_spd_barycenter}
We consider the problem of computing the Wasserstein barycenter of a set of block SPD matrix-valued measures. 
%Let $\Delta_n(\sS_{++}^d)$ denote $n$ SPD matrices of size $d\times d$, i.e., $\Delta_n(\sS_{++}^d) := \{ \bP = [\bP_i]_{n \times 1} : \sum_i \bP_i = \bI \}$. 
Let $\Delta_n(\sS_{++}^d) \coloneqq \{ \bP = [\bP_i]_{n \times 1} : \bP_i\in\sS_{++}^d, \sum_i \bP_i = \bI \}$ denotes the space of $n\times 1$ block SPD marginals. 
%Let $\{\bP^\ell\}_{\ell=1}^K \in \Delta_{n_\ell}(\sS_{++}^d)$ be the given set of measures. 
Then, the Wasserstein barycenter $\bar{\bP}$ of a set $\{\bP^\ell\}_{\ell=1}^K \in \Delta_{n_\ell}(\sS_{++}^d)$ is computed as follows:
%Given a set of SPD matrix-valued measures, $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$ for $\ell = 1,...,K$, the block SPD Wasserstein barycenter learning problem is to identify
\begin{equation}
    % \gW\gB_\epsilon(\{ \bP^\ell \}, \bomega)
    \bar{\bP}= \argmin_{{\bP} \in \Delta_{n}(\sS_{++}^d)} \sum_{\ell =1}^K \omega_\ell {\rm MW}^2_\epsilon({\bP}, \bP^\ell) , \label{w_barycenter}
\end{equation}
where the given non-negative weights satisfy $\sum_\ell \omega_\ell =1$. 
It should be noted that we employ a regularized version of the proposed block SPD OT problem (\ref{reformulated_mw}) to ensure the differentiability of the objective function near boundary in~\eqref{w_barycenter}. The regularized block SPD OT problem is defined as 
%For the purpose of barycenter learning, we consider a regularized matrix-valued OT problem:
\begin{align}
    &{\rm MW}^2_\epsilon(\bP, \bQ) \nonumber\\
    &:= \min_{\bGamma \in \M_{m,n}^d(\bP, \bQ)} \sum_{i,j} \Big( \trace( \bC_{i,j}\bGamma_{i,j})+ \epsilon \, \Omega(\bGamma_{i,j}) \Big),\label{eqn:regMWOT} 
\end{align}
where $\epsilon>0$ is the regularization parameter and  $\Omega(\cdot)$ is a strictly convex regularization  (e.g., entropic regularization) on the block SPD coupling matrices. 
%As long as the regularization is convex, Theorem \ref{Prop_Riem_opt_optimal} guarantees the optimal solution by Riemannian optimization. 

%\alertBM{$\gW\gB_\epsilon$ is not used anywhere, removing it}

To solve for $\bar{\bP}$ in (\ref{w_barycenter}), we consider Riemannian optimization on $\Delta_n(\sS_{++}^d)$, which has recently been studied in~\citep{mishra2019riemannian}. 
%To solve $\bar{\bP}$ in (\ref{w_barycenter}), we consider Riemannian optimization in the space of $\Delta_n(\sS_{++}^d)$, which has recently been shown to have a Riemannian manifold structure~\citep{mishra2019riemannian}. 
%that allows optimization of a general objective function. 
%To that end, we only need to compute the Euclidean gradient of the barycenter problem \eqref{w_barycenter} with respect to $\bar{\bP}$ (the Riemannian gradient and other optimization-related ingredients for $\Delta_n(\sS_{++}^d)$ follow from the work of \citep{mishra2019riemannian}. 
%The next proposition shows the Euclidean gradient is given by evaluating the projection of Euclidean gradient of ${\rm MW}_\epsilon$ at optimality.
The following result provides an expression for the Euclidean gradient of the objective function in problem~(\ref{w_barycenter}). 
% with the dual variables $\bLambda_i, \bTheta_j, \bPsi_{i,j}$. From the dual problem, we can verify the Euclidean gradient of the barycenter problem \eqref{w_barycenter} with respect to $\bar{\bX}_i$ is $\bLambda_i^*$ (which is unique up to a translation matrix of size $d \times d$), the optimal dual variable. As long as the optimal dual variable $\bLambda_i^*$ can be computed, we can update $\bar{\bX}_i$ via Riemannian gradient descent on the simplex of SPD manifold \cite{mishra2019riemannian}. 
\begin{proposition}
\label{dual_var_solution_prop}
The Euclidean gradient of \eqref{w_barycenter} with respect to ${\bP}_i$, for $i \in [n]$ is
\begin{equation*}
    \sum_{\ell=1}^K \omega_\ell \nabla_{{\bP}_i}{\rm MW}_\epsilon({\bP}, \bP^\ell) = - \sum_{\ell=1}^K \omega_\ell (\bLambda^\ell_i)^*,
\end{equation*}
where $(\bLambda^\ell_i)^*$ is given by evaluating the orthogonal projection ${\rm P}_{(\bGamma^\ell)^*}(\nabla_{(\bGamma^\ell)^*} {\rm MW}_\epsilon)$, where $\nabla_{(\bGamma^\ell_{i,j})^*} {\rm MW}_\epsilon = \bC_{i,j}^\ell + \epsilon \nabla \Omega((\bGamma^\ell_{i,j})^*)$ and $(\bGamma^\ell)^*$ is the optimal coupling for $\bP^\ell$. That is, $(\bLambda^\ell_i)^*$ is the auxiliary variable obtained during the solving of the system of matrix linear equations in Proposition \ref{orthogonal_proj}. %\alertPJ{Some notational issues - will discuss it over call.}
% The optimal dual variables $\bLambda_i^*, \bTheta_j^*$, $\forall i,j$ of the regularized block matrix-valued OT problem $min_{\bGamma \in \M_{m \times n}^d(\bP, \bQ)} \gW_\epsilon(\bP, \bQ)$ is given by evaluating the orthogonal projection ${\rm P}_{\bGamma^*}(\nabla_{\bGamma^*} \gW_\epsilon)$, where $\nabla_{\bGamma^*_{i,j}} \gW_\epsilon = \bC_{i,j} + \epsilon \nabla \Omega(\bGamma_{i,j}^*)$. The $\bLambda_i^*, \bTheta_j^*$ are given by solving the system of matrix linear equations in Proposition \ref{orthogonal_proj}.
\end{proposition}
% This proposition is a direct result from Theorem \ref{Prop_Riem_opt_optimal}, based on which the Euclidean gradient of problem \eqref{w_barycenter} with respect to the barycenter $\bar{\bX}_i$ is given by $\sum_\ell \omega_\ell (\bLambda_i^\ell)^*$.
The complete algorithm for computing the barycenter in \eqref{w_barycenter} is outlined in Algorithm \ref{wb_algorithm} (Appendix \ref{geometry_spd_simplex_appendix}). 

% \alertPJ{Is this algorithm required or can we simply refer to~\citep{mishra2019riemannian}.} 
% \alertAH{Yes it is required. It is for the purpose of general audience.} \alertPJ{If its general audience, we should put it in supplementary unless we need to fill the main paper - as all the steps can be mapped to the general Algorithm 1.}




% \alertBM{Relook at the remark}
% \begin{remark}
% \label{fast_compute_barycenter_rmk}
% When there are only two input marginals $\sum_{i=1}^m \bX_i \delta_{x_i}$ and $\sum_{j=1}^n \bY_j \delta_{y_j}$, and the distance matrix is scalar-valued, i.e., $\bC_{i,j} = d(x_i, y_j) \bI$ for some ground cost metric $d(\cdot, \cdot)$ on $\gX = \gY$, the barycenter computation can be simplified by extending the displacement interpolation \cite{mccann1997convexity} to matrix-valued marginals. See \citep[Section~2.2]{peyre2016quantum} for more information. Note that due to the balanced nature of our proposed formulation, we do not need to adjust the couplings after matching as required in \cite{peyre2016quantum}.
% \end{remark}




%\subsection{Matrix-valued Gromov-Wasserstein optimal transport and distance averaging}
\subsection{Block SPD Gromov-Wasserstein discrepancy}
\label{sec:proposedGW}
The Gromov-Wasserstein (GW) distance~\citep{memoli2011gromov} generalizes the optimal transport to the case where the measures are supported on possibly different metric spaces $\gX$ and $\gY$. 
Let $\bD^x\in\sR^{m\times m}$ and $\bD^y\in\sR^{n\times n}$ represent the similarity (or distance) between elements in metric spaces $\gX$ and $\gY$ respectively. Let $\bp\in \Sigma_m$ and $\bq \in \Sigma_n$ be the marginals corresponding to the elements in $\gX$ and $\gY$, respectively. 
%Let two set of metric-measure pairs be represented by $(\bD^x, \bp)$ and $(\bD^y, \bq)$. Here, $\bp\in \Sigma_m$ and $\bq \in \Sigma_n$ are the measures and  where $\bD^x$ and $\bD^y$ represent distance (or similarity) matrices 
%Suppose we are given two sets of pairs $(\bD^x, \bp), (\bD^y, \bq)$, where $\bD^x, \bD^y$ represent either similarity or distance matrices and $\bp \in \Sigma_m, \bq \in \Sigma_n$ are the given marginals. 
Then, the GW discrepancy between the two distance-marginal pairs $(\bD^x, \bp)$ and $(\bD^y, \bq)$ is defined as 
\begin{equation*}
\label{eqn:GW}
\begin{array}{ll}
{\rm GW} \big( (\bD^x, \bp), ( \bD^y, \bq ) \big)  \\[3pt]
 \coloneqq \min_{\bgamma \in \Pi(\bp, \bq)} \sum_{i,i',j,j'} \L(D^x_{i,i'}, D^y_{j,j'}) \gamma_{i,j} \gamma_{i',j'},
\end{array}
\end{equation*}
where $D_{k,l}$ denotes the $(k,l)$-th element in the matrix $\bD$ and $\L$ is a loss between the distance pairs. Common choices of $\L$ include the $L_2$ distance and the KL divergence. 


% \paragraph{GW for cross-domain quantum optimal transport.} 
We now generalize the GW framework to our setting where the marginals are SPD matrix-valued measures.  
%(i.e., tensor-valued by the terminology in \cite{peyre2016quantum}). 
% This can be used for matching tensor fields supported on different domains. 
Let $(\bD^x, \bP)$ and $(\bD^y, \bQ)$ be two distance-marginal pairs, where the Dirac measures are given by $\sum_i \bP_i \delta_{x_i}$, $\sum_j \bQ_j \delta_{y_j}$ respectively, for $\{x_i\}_{i \in [m]} \subset \gX, \{y_j\}_{j \in [n]} \subset \gY$. The marginals are tensor-valued with $\bP \in \Delta_m(\sS_{++}^d)$, $\bQ \in \Delta_n(\sS_{++}^d)$. 
%Different to setting in \citep{peyre2016quantum}, we consider the general case where $\gX \neq \gY$ while the SPD-valued marginals are assumed to have the same dimension $d$. 
%
% We now generalize the GW distance to different metric spaces having block SPD measures. 
% $\bPsi\coloneqq\{[\bPsi_i]_{m\times 1}:\bPsi_i \in \sS_{+}^d,\sum_i \bPsi_i=\bI\}$ and $\bPhi\coloneqq\{[\bPhi_j]_{n\times 1}:\bPhi_i \in \sS_{+}^d,\sum_j \bPhi_j=\bI\}$. 
%Consider two dirac measures $\bPsi = \sum_i \bPsi_i \delta_{x_i}$ and $\bPhi = \sum_j \bPhi_j \delta_{y_j}$ where $\{x_i\}_{i \in [m]} \in \gX, \{y_j\}_{j \in [n]} \in \gY$ and the measures are tensor-valued, i.e., $\bPsi_i, \bPhi_j \in \sS_{++}^d$. Different to \citep{peyre2016quantum}, we consider the general case where $\gX \neq \gY$ and thus the classic matrix-valued OT cannot apply. 
% In \citep{peyre2016quantum}, the domains are assumed to be identical, i.e., $\gX = \gY$ and thus the classic matrix-valued OT can be applied. Here we consider the general case where $\gX \neq \gY$, with $D^x_{i,i'} = d_\gX(x_i, x_{i'}), D^y_{j, j'} = d_{\gY}(y_j, y_{j'})$ for $i,i'\in [m], j,j' \in [n]$ computed from the ground distance on $\gX, \gY$. 
We define the SPD generalized GW discrepancy as
\begin{equation}\label{scalar_gw_ot}
\begin{array}{lll}
    {\rm MGW} \big( (\bD^x, \bP), ( \bD^y, \bQ ) \big)  \coloneqq \\[3pt]
   \min\limits_{\bGamma \in \M^d_{m \times n}} \sum\limits_{{i,i',} {j, j'}} \L\big( D^x_{i,i'},D^y_{j, j'}  \big) \trace( \bGamma_{i,j} \bGamma_{i',j'}),
\end{array}
\end{equation}
% where $\bD^x, \bD^y$ are computed from the ground distance on $\gX, \gY$, respectively.
% Notice in \eqref{scalar_gw_ot}, the cost can be extended to be matrix-valued, i.e., $\bC_{i,i',j,j'} \in \sS_{+}^d$ between pair $i,i'$ and $j,j'$, which gives a transport cost $\sum_{i,i',j',j'}\trace(\bC_{i,i',j,j'} \bGamma_{i,j} \bC_{i,i',j,j'} \bGamma_{i',j'})$. 
where we use Riemannian optimization (Algorithm \ref{Riemannian_optimizer}) to solve problem~\eqref{scalar_gw_ot}.

% is non-convex and quadratic in $\bGamma$ and it can be solved via Riemannian optimization (Algorithm \ref{Riemannian_optimizer}).

% We employ the proposed Algorithm~\ref{Riemannian_optimizer} to solve~\eqref{scalar_gw_ot}. 


%\alertPJ{It should be noted that the proposed GW setting assumes both the metric spaces $\gX$ and $\gY$ to be $d$-dimensional. However, if the spaces are not aligned (alvares-reference), the elements cannot be directly compared across spaces. Question - can we work with different dimensional SPDs? Why are we using Psi and Phi instead of P and Q?}
%\alertAH{Please note that $\gX, \gY$ is not the space of SPD. It is any metric-measured space. Only the marginals are SPD-valued. So the $d$ dimension has nothing to do with $\gX, \gY$.}

% Similarly, we can consider a generalized matrix-valued GW OT problem. Suppose the cost between the distances $D_{i,i'}^x, D^y_{j,j'}$ is matrix-valued, i.e., $\bC_{i,i',j,j'} \in \sS_{+}^d$, $\forall i,i' \in [m], j,j' \in [n]$ and we are given some block SPD-valued marginals, $\bP, \bQ$ on two domains. Then the generalized GW discrepancy is thus given by 
% \begin{equation}
%     \min_{\bGamma \in \M^d_{m \times m}(\bP, \bQ)} \sum_{i,i',j,j'} \trace(\bC_{i,i',j,j'} \bGamma_{i,j}  \bC_{i,i',j,j'} \bGamma_{i',j'}). \label{tensor_GW_problem}
% \end{equation}
% 






\begin{figure*}[!t]
\captionsetup{justification=centering}
    \centering
    \subfloat[MNIST \label{mnist_fig}]{\includegraphics[width = 0.28\textwidth, height = 0.2\textwidth]{Figures/domain_adaptation/mnist_da_result.pdf}} 
    \subfloat[Fashion MNIST \label{fmnist_fig}]{\includegraphics[width = 0.28\textwidth, height = 0.2\textwidth]{Figures/domain_adaptation/fashionmnist_da_result.pdf}} 
    \subfloat[Letters \label{letters_fig}]{\includegraphics[width = 0.28\textwidth, height = 0.2\textwidth]{Figures/domain_adaptation/letters_da_result.pdf}}
    \caption{Domain adaptation and classification results for three datasets: MNIST \eqref{mnist_fig}, Fashion MNIST \eqref{fmnist_fig} and Letters~\eqref{letters_fig}. The skew ratio increases from uniform (uf) to $r=0.5$. For MNIST and Fashion MNIST, uf=$0.1$ and for Letters, uf=$1/26$. We observe that the proposed RMOT performs significantly better than the baselines. 
    %The proposed RMOT outperforms sOT and SPDOT, especially in more challenging domain adaptation settings, i.e., higher skew ratios, implying the usefulness of the non-trivial correlations learned by the SPD matrix valued couplings of {\algname}.
    % Thus, the SPD matrix valued couplings of RMOT seem to better understand the non-trivial correlations. 
    % shows a good performance in harder settings (with higher skew ratios) implying the SPD matrix-valued couplings understand non-trivial correlations.
    } 
    \label{domain_adaptation_figure}
\end{figure*}






\paragraph{Gromov-Wasserstein averaging of distance matrices.} 

The GW formulation with scalar-valued probability measures has been used for averaging distance matrices~\citep{peyre2016gromov}. Building on \eqref{scalar_gw_ot}, we consider the problem of averaging distance matrices where the marginals are SPD-valued.  
% corresponding GW formulation to tensor-valued marginals for quantum distance averaging. 
Let $\{(\bD^\ell, \bP^\ell)\}_{\ell = 1}^K$ with $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$, be a set of distance-marginal pairs on $K$ incomparable domains.
%Given a set of distance-marginal pair $\{(\bD^\ell, \bP^\ell)\}_{\ell = 1}^K$ where $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$ on $K$ incomparable domains.
Suppose the barycenter marginals $\bar{\bP} \in \Delta_{n}(\sS_{++}^d)$ are given, the goal is to find the average distance matrix $\bar{\bD}$ by solving 
\begin{equation}\label{gw_barycenter_problem}
\begin{array}{ll}
    \bar{\bD} = \argmin\limits_{\bD \in \sS^n : D_{i,j} \geq 0} \sum_{\ell=1}^K \omega_\ell \, {\rm MGW} \big( (\bD, \bar{\bP}), ( \bD^\ell, \bP^\ell ) \big),
\end{array}    
\end{equation}
where the given weights satisfy $\sum_\ell \omega_\ell = 1$.  Problem \eqref{gw_barycenter_problem} can be solved via a block coordinate descent method, that iteratively updates the couplings $\{ \bGamma^\ell \}_{\ell=1}^K$ and the distance matrix $\bar{\bD}$. The update of the coupling is performed via Algorithm \ref{Riemannian_optimizer}. For the update of the distance matrix, we show when the loss $\L$ is decomposable, including the case of $L_2$ distance or the KL divergence, the optimal $\bar{\bD}$ admits a closed-form solution. This is a generalization of the result \citep[Proposition 3]{peyre2016gromov} to SPD-valued marginals.
% The update of barycenter concerns the optimization problem 
% \begin{equation}
%     \min_{ \bD \in \sS^n : \bD_{i,j} \geq 0} \sum_{\ell =1}^K \omega_\ell \, \Big( \sum_{i,i',j,j'} \L(\bar{D}_{i,i'}, D^\ell_{j,j'}) \trace(\bGamma^{\ell}_{i,j} \bGamma^{\ell}_{i',j'}) \Big) \label{gw_barycenter_problem}
% \end{equation}
% which can be solved by gradient descent for reparameterized $\bD$. 
\begin{proposition}
\label{average_distance_update}
Suppose the loss $\L$ can be decomposed as $\L(a, b) = f_1(a) + f_2(b) - h_1(a) h_2(b)$ with $f_1'/h_1'$ invertible, then \eqref{gw_barycenter_problem} has a closed form solution given by $\bar{D}_{i,i'} = \big(\frac{f_1'}{h_1'} \big)^{-1} \big(h_{i,i'} \big)$ with
\begin{equation*}
   h_{i,i'} = \Big( \frac{\sum_{\ell=1}^K \omega_\ell \trace \big(\sum_j \bGamma_{i,j}^\ell \sum_{j'} h_2( D^\ell_{j,j'}) \bGamma^\ell_{i', j'} \big) }{\trace(\bar{\bP}_i \bar{\bP}_{i'})} \Big).
\end{equation*}
\end{proposition}
% \alertPJ{It should be noted that Proposition~\ref{average_distance_update} generalized the results in~\citep{peyre2016gromov} for block SPD measure setting.}















\section{Experiments}
\label{Experiment_sect}
In this section, we show the utility of the proposed framework in a number of applications. For empirical comparisons, we refer to our approaches, block SPD OT~\eqref{reformulated_mw}, the corresponding Wasserstein barycenter~\eqref{w_barycenter}, and block SPD Gromov-Wasserstein OT~\eqref{scalar_gw_ot}~\&~\eqref{gw_barycenter_problem}, collectively as RMOT (Riemannian optimized Matrix Optimal Transport). 
For all the experiments, we use the Riemannian steepest descent method using the Manopt toolbox \cite{boumal2014manopt} in Algorithm~\ref{Riemannian_optimizer}. 



\subsection{Domain adaptation}
We apply our OT framework to the application of unsupervised domain adaptation where the goal is to align the distribution of the source with the target for subsequent tasks. 
% We first discuss below the \textit{barycentric projection} for the proposed block SPD OT formulation (\ref{reformulated_mw}). 
%Here we extend this formulation to matrix-valued samples.

Suppose we are given the source $\bp \in \Sigma_m$ and target marginals $\bq \in \Sigma_n$, along with samples $\{ \bX_i\}_{i=1}^m, \{ \bY_j\}_{j = 1}^n$ from the source and target distributions. The samples are matrix-valued, i.e., $\bX_i ,\bY_j \in \sR^{d \times s}$. We define the cost as $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i -\bY_j)^\top$. It should be noted that $\trace{(\bC_{i,j})}=\|\bX_i - \bY_j\|_{\rm F}^2$, which is the cost function under the $2$-Wasserstein OT setting~(\ref{W22}). 
%which can be viewed as a generalized matrix $L_2$ distance. 
For domain adaptation, we first learn an optimal coupling between the source and target samples by solving the proposed OT problem \eqref{reformulated_mw} with marginals $\bP, \bQ$ constructed as $\bP \coloneqq \{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$ (as discussed in Section \ref{matrix_generalized_ot_sect}). Finally, the source samples are projected to the target domain via barycentric projection. 
%to match the target distribution, a process known as the \textit{barycentric projection}.


With the optimal coupling $\bGamma_{i,j}^*$, the barycentric projection of a source sample $\bX_i$ is computed as
\begin{equation*}
\begin{array}{rl}
    \hat{\bX}_i = & \argmin\limits_{\bX_i \in \sR^{d\times s}} \sum_{i,j} \trace ( (\bX_i - \bY_j)(\bX_i - \bY_j)^\top \bGamma_{i,j}^* ) \\
    = & \bP_i^{-1}(\sum_j \bGamma_{i,j}^* \bY_j).
\end{array}
\end{equation*}
% From the first order condition, we have 
% \begin{equation}
%     \hat{\bX}_i = \bP_i^{-1}(\sum_j \bGamma_{i,j}^* \bY_j), \quad \forall i. \label{barycentric_proj}
% \end{equation}
%The projected samples $\{ \hat{\bX}_i\}$ follow the same distribution as the target samples $\{ \bY_j\}$. 

The above formulation also works for structured samples. For instance, when the samples are SPD, i.e., $\bX_i, \bY_j \in \sS_{++}^d$, the projected source sample $\hat{\bX}_i$ is now the solution to the matrix Lyapunov equation: $\{ \bP_i \hat{\bX}_i \}_{\rm S} = \{\sum_j \bGamma^*_{i,j} \bY_j\}_{\rm S}$. Here, $\{ \bA\}_{\rm S} = (\bA + \bA^\top)/2$.



























%\paragraph{Image set classification.} 
\paragraph{Experimental setup.}
We employ domain adaptation to classify the test sets (target) of multiclass image  datasets, where the training sets (source) have a different class distribution than the test sets. 
% Supervision is available only for training set.  
%We test the above formulation for image set classification . 
Suppose we are given a training set $\{ \bX_i\}_{i=1}^m$ and a test set $\{  \bY_j\}_{j=1}^n$ where $\bX_i, \bY_j \in \sR^{d \times s}$ are $s$ (normalized) image samples of the same class in $d$ dimension for each image set $i,j$. Instead of constructing the cost directly on the input space, which are not permutation-invariant, we first compute the sample covariances $\bS_{x_i} = \bX_i \bX_i^\top/s$ and $\bS_{y_j} = \bY_j \bY_j^\top/s$, $\forall i,j$. Now the cost between $i, j$ is given by $\bC_{i,j} = (\bS_{x_i} - \bS_{y_j})(\bS_{x_i} - \bS_{y_j})^\top$. Once the block SPD matrix coupling is learnt, the $\bS_{x_i}$ covarinaces are projected using the barycerntric projection to obtain $\hat{\bS}_{x_i}, i \in [m]$. This is followed by nearest neighbour classification of $j$ based on the Frobenius distance $\| \hat{\bS}_{x_i} - \bS_{y_j} \|_{\rm F} \forall i,j$. 


% We thus solve the symmetric Lyapunov equation for the projected covariance matrices $\hat{\bS}_{x_i}, i \in [m]$. This is followed by nearest neighbour classification based on the Frobenius distance $d_{i,j} = \| \hat{\bS}_{x_i} - \bS_{y_j} \|_{\rm F}$. 

We compare the proposed {\algname} (\ref{reformulated_mw}) with the following baselines: (i) sOT: the $2$-Wasserstein OT~(\ref{W22}) with the cost $c_{i,j} = \trace(\bC_{i,j})=\|\bS_{x_i} - \bS_{y_j} \|_{\rm F}^2$ \cite{courty2016optimal}, and (ii) SPDOT: the $2$-Wasserstein OT (\ref{W22}) with the cost as the squared Riemannian geodesic distance between the SPD matrices $\bS_{x_i}$ and $\bS_{y_j}$ \cite{yair2019parallel}. 
% \begin{itemize}
%     \item sOT: the $2$-Wasserstein OT~(\ref{W22}) with the cost $c_{i,j} = \trace(\bC_{i,j})=\|\bS_{x_i} - \bS_{y_j} \|_{\rm F}^2$ \cite{courty2016optimal}. 
%     \item SPDOT: the $2$-Wasserstein OT (\ref{W22}) with the cost as the squared Riemannian geodesic distance between the SPD matrices $\bS_{x_i}$ and $\bS_{y_j}$ \cite{yair2019parallel}.
% \end{itemize}
%1) the $2$-Wasserstein OT~(\ref{W22}) with the cost $c_{i,j} = \trace(\bC_{i,j})=\| \hat{\bS}_{x_i} - \bS_{y_j} \|_{\rm F}^2$ \cite{courty2016optimal}, and 2) scalar-valued  OT (\ref{W22}) with the cost as Riemannian geodesic distance between the covariance matrices \cite{yair2019parallel}. We label them sOT and SPDOT respectively.

%The results from our proposed Riemannian optimized matrix-valued OT ({\algname}) are compared against two baselines: 1) the scalar-valued OT in (\ref{W22}) with the cost $c_{i,j} = \trace(\bC_{i,j})$ \cite{courty2016optimal} and 2) scalar-valued  OT (\ref{W22}) with the cost as Riemannian geodesic distance between the covariance matrices \cite{yair2019parallel}. We label them sOT and SPDOT respectively.


% \alertAH{In addition, we also compare our balanced OT formulation with a quantum KL regularized variant.}

\textbf{Datasets.} We experiment on three multiclass image datasets -  handwritten letters \cite{frey1991letter}, MNIST \cite{lecun1998gradient} and Fashion MNIST \cite{xiao2017fashion} - with various skewed distributions for the training set. MNIST and Fashion MNIST have $10$ classes, while Letters has $26$ classes. 
Specifically, we fix the distribution of the test set to be uniform (with the same number of image sets per class). We increase the proportion of the a randomly chosen class in the training set to the ratio $r$, where $r=\{{\rm uf},0.1,0.2,0.3,0.4,0.5\}$ and ${\rm uf}$ is the ratio corresponding to the uniform distribution of all classes. We reduce the dimension of MNIST, fashion MNIST, and Letters by PCA to $d=5$ features. We set $s=d$, $m=250$, and $n=100$ for each dataset. 
%The sample size $s = d$ for each dataset is chosen uniformly. 
%This results in $m = 250, n = 100$ for training and test set, respectively. 

\textbf{Results.} Figure~\ref{domain_adaptation_figure} shows the classification accuracy on the three datasets. 
We observe that the proposed RMOT outperforms sOT and SPDOT, especially in more challenging domain adaptation settings, i.e., higher skew ratios. This implies the usefulness of the non-trivial correlations learned by the SPD matrix valued couplings of {\algname}. 
%We observe that the proposed SPD-valued OT compared to scalar-valued OT as the skew $r$ increases (harder settings). 

%  which gives $d = 34$ for MNIST and $d = 14$ for fashion MNIST













\subsection{Tensor Gromov-Wasserstein distance averaging for shape interpolation}
% \alertBM{We should refer to the papers}
We consider an application of the proposed block SPD Gromov-Wasserstein OT formulation (Section~\ref{sec:proposedGW}) for interpolating tensor-valued shapes. We are given two distance-marginal pairs $(\bD^0, \bP^0), (\bD^1, \bP^1)$ where $\bD^0, \bD^1 \in \sR^{n \times n}$ are distance matrices computed from the shapes and $\bP^0, \bP^1$ are given tensor fields. The aim is to interpolate between the distance matrices with weights $\bomega = (t, 1-t), t \in [0,1]$. The interpolated distance matrix $\bD^t$ is computed by solving \eqref{gw_barycenter_problem} via Riemannian optimization and Proposition \ref{average_distance_update}, with the barycenter tensor fields ${\bP}^t$ given. Finally, the shape is recovered by performing multi-dimensional scaling to the distance matrix. 



\begin{figure}[ht]
% \settoheight{\tempdima}{\includegraphics[width=.06\textwidth]{example-image-a}}%
\centering
\begin{tabular}{@{}c@{ \hspace*{1.5pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }}
\raisebox{.025\textwidth}{\footnotesize (a)}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/bary-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/bary-2.pdf}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/bary-3.pdf}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/bary-4.pdf}&
\includegraphics[width=.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-2.pdf}\\[5pt]
% \raisebox{.025\textwidth}{\footnotesize (b)}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-1.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-1.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-2.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-3.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-4.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-2.pdf}\\[5pt]

\raisebox{.025\textwidth}{\footnotesize (b)}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/input-r-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/bary-r-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/bary-r-2.pdf}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/bary-r-3.pdf}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/bary-r-4.pdf}&
\includegraphics[width=.06\textwidth]{Figures/annulus-star4-gw/input-r-2.pdf}\\[5pt]

\raisebox{.025\textwidth}{\footnotesize (c)}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/bary-r-1.pdf}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/bary-r-2.pdf}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/bary-r-3.pdf}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/bary-r-4.pdf}&
\includegraphics[width=.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-2.pdf}\\[3pt]
&{\footnotesize $t=0$} & {\footnotesize $t=0.2$} & {\footnotesize $t=0.4$} & {\footnotesize $t=0.6$} & {\footnotesize $t=0.8$} & {\footnotesize $t=1$} \\
\end{tabular}
\caption{Tensor-valued shape interpolation obtained using the proposed RMOT~(Section~\ref{sec:proposedGW}). }%
\label{GW_distance_averaging}
\end{figure}






Figure \ref{GW_distance_averaging} presents the interpolated shapes with $n = 100$ sample points for the input shapes. The matrices $\bD^0, \bD^1$ are given by the Euclidean distance and we consider $L_2$ loss for $\L$. The input tensor fields $\bP^0, \bP^1$ are generated as uniformly random in (a), cross-oriented in (b) and smoothly varying in (c). The barycenter tensor fields are given by the linear interpolation of the inputs, i.e., $\bP^t = (1-t) \bP^0 + t \bP^1$. The results show the proposed Riemannian optimization approach (Section~\ref{manifold_geometry_sect}) converges to reasonable stationary solutions for non-convex OT problems. 








\begin{figure*}[!th]
\captionsetup{justification=centering}
    \centering
    \subfloat[Linear interpolation]{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/linear-interp.pdf}} 
    \hspace*{5pt}
    \subfloat[QOT ($\rho = 50$)]{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_50.pdf}}
    \hspace*{5pt}
    \subfloat[QOT ($\rho = 100$)]{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_100.pdf}}
    \hspace*{5pt}
    \subfloat[QOT ($\rho = 500$)]{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_500.pdf}}
    \hspace*{5pt}
    \subfloat[{\algname}]{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/BlockMOT-ellipses.pdf}} \\[5pt]
    
    \subfloat[Input ($t = 0$) \label{input_1}]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/input-ellispses-1.pdf}} 
    \hspace*{3pt}
    \subfloat[Input ($t=1$) \label{input_2}]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/input-ellispses-2.pdf}} 
    \hspace*{3pt}
    \subfloat[QOT ($t=0.25$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat[QOT ($t=0.5$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat[QOT ($t=0.75$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-4.pdf}} 
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.25$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.5$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.75$)]{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-4.pdf}}
    \caption{Tensor field mass interpolation on 1-$d$ (top) and 2-$d$ (bottom) grids. On the top, each row corresponds to an interpolation where we show $7$ evenly-spaced interpolated tensor fields. On the bottom, the inputs are given in (f) and (g). We set $\rho = 100$ for QOT and show $3$ evenly-spaced interpolated tensor fields.} 
    \label{interpolation_figure}
\end{figure*}





\subsection{Tensor field optimal transport mass interpolation}
We consider performing optimal transport and displacement interpolation between two tensor fields supported on regular 1-$d$ (or 2-$d$) grids~\citep{peyre2016quantum}. 
We consider a common domain $\gD = [0,1]$ (or $[0,1]^2$) with the cost defined as $\bC_{i,j} = \| \bx_i - \by_j \|^2 \bI$ for $\bx_i, \by_j \in \gD$. The marginals $\bP, \bQ$ are given tensor fields. We first compute the balanced coupling $\bGamma$ by solving an entropy regularized OT problem~(\ref{eqn:regMWOT}): 
\begin{equation*}
    \min_{\bGamma \in \M_{m \times n}^d(\bP, \bQ)} \sum_{i,j} \Big( \trace(\bC_{i,j}\bGamma_{i,j}) - \epsilon \, H(\bGamma_{i,j}) \Big),
\end{equation*} 
where the quantum entropy is defined as $H(\bGamma_{i,j}) \coloneqq - \trace(\bGamma_{i,j} \log(\bGamma_{i,j}) - \bGamma_{i,j})$. 
Then, the coupling is used to interpolate between the two tensor fields by generalizing the displacement interpolation \cite{mccann1997convexity} to SPD-valued marginals. Please refer to~\citep[Section~2.2]{peyre2016quantum} for more details. It should be noted that due to the balanced nature of our formulation, we do not need to adjust the couplings after matching as required in~\cite{peyre2016quantum}.












We compare interpolation results of the proposed (balanced) {\algname} with both linear interpolation $(1-t)\bP + t \bQ$ for $t \in [0,1]$ and the \textit{unbalanced} quantum OT (QOT) of \citet{peyre2016quantum}. The QOT solves the following problem with quantum KL regularization, i.e.,
\begin{equation*}
\begin{array}{ll}
    \min\limits_{\bGamma} \sum_{i,j} \Big( \trace(\bC_{i,j} \bGamma_{i,j}) - \epsilon \, H(\bGamma_{i,j}) \\
  \qquad \qquad \qquad + \rho \, {\rm KL}(\bGamma \sone | \bP) + \rho \,{\rm KL}(\bGamma^\top \sone | \bQ) \Big),
\end{array}
\end{equation*}
where ${\rm KL}(\bP | \bQ) \coloneqq \sum_i \trace \big(\bP_i \log(\bP_i) - \bP_i \log(\bQ_i) -\bP_i +\bQ_i \big)$ and $\bGamma \sone \coloneqq [\sum_j (\bGamma_{i,j})]_{m \times 1}$ and $\bGamma^\top \sone \coloneqq [\sum_i (\bGamma_{i,j})]_{n \times 1}$. For comparability, we set the same $\epsilon$ for both QOT and {\algname}.
% and Riemannian optimization stops after $30$ iterations using Riemannian steepest descent. 




Figure \ref{interpolation_figure} compares the mass interpolation for both 1-$d$ (top) and 2-$d$ (bottom) grids. 
%For the 1-$d$ case, we observe the interpolated tensor fields obtained by QOT traverse from the linear interpolation to {\algname} as the parameter $\rho$ increases.  
%{\algname} can be considered as the limit of QOT when $\rho \xrightarrow{} \infty$. 
For the 2-$d$ tensor fields, we further renders the tensor fields via a background texture where we perform anisotropic smoothing determined by the tensor direction. 
%Similarly, we see the tensor fields generated from {\algname} more closely respect the marginal constraints.
In both the settings, we observe that the tensor fields generated from {\algname} respect the marginal constraints more closely. 






\subsection{Tensor field Wasserstein barycenter}
We also analyze the Wasserstein barycenters learned by the proposed RMOT approach and qualitatively compare with QOT barycenter \citep[Section 4.1]{peyre2016quantum}. We test on two tensor fields ($n = 4$) supported 2-$d$ grids.  
%to illustrate the difference between {\algname} and QOT barycenter \citep[Section 4.1]{peyre2016quantum}. 

Figure~\eqref{barycenter_fig} compares barycenter from QOT (top) and {\algname} (bottom) initialized from the normalized solution of QOT. We observe that the QOT solution is not optimal when the marginal constraint is enforced and the barycenter obtained does not lie in the simplex of tensors. 
% Such a claim is strengthened by comparing the objective value versus the optimal value, obtained by the CVX toolbox \citep{grant2014cvx}. See Figure \ref{obj_compare_barycenter} in the appendix. 




\begin{figure}[!th]
\captionsetup{justification=centering}
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/input-1.pdf}
	\end{minipage}}
 \hfill 	
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-2-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-2-5.pdf}
	\end{minipage}}
	\hfill
	\subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-3-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-3-5.pdf}
	\end{minipage}}
	\hfill
	\subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-4-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-4-5.pdf}
	\end{minipage}}
 \hfill	
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/input-2.pdf}
	\end{minipage}}
\caption{Barycenter interpolation. From left to right $t = 0$ (input), $t= 0.25, 0.5, 0.75$ (barycenters), $t=1$ (input). The top row is QOT and the bottom is {\algname}.}
\label{barycenter_fig}
\end{figure}



% \begin{figure}[!th]
% \captionsetup{justification=centering}
%     \centering
%     \subfloat[Input ($t=0$)]{\includegraphics[width = 0.05\textwidth, height = 0.05\textwidth]{}} 
%     \hspace*{5pt}
%     \subfloat[Input ($t=0$)]{\includegraphics[width = 0.05\textwidth, height = 0.05\textwidth]{Figures/2d-bary-n2/input-2.pdf}} 
%     \caption{Barycenter} 
%     \label{barycenter_fig}
% \end{figure}








% \begin{figure}[!th]
% \captionsetup{justification=centering}
%     \centering
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-2.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-3.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-4.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-2.pdf}} \\[5pt]
    
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-2.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-3.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-4.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-2.pdf}} \\[5pt]
    
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-1.pdf}}{\footnotesize $t=0$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-1.pdf}}{\footnotesize $t=0.2$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-2.pdf}}{\footnotesize $t=0.4$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-3.pdf}}{\footnotesize $t=0.6$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-4.pdf}}{\footnotesize $t=0.8$}
%     \hspace*{0.7pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-2.pdf}}{\footnotesize $t=1$} 
    
%     \caption{Tensor-valued shape interpolation.} 
%     \label{GW_distance_averaging}
% \end{figure}















\section{Conclusion}
In this paper, we have discussed the balanced optimal transport (OT) problem involving SPD matrix-valued measures that is shown to be a natural generalization of ${\rm W}_2$ formulation. It also preserves the metric property. For the SPD matrix-valued OT problem, the coupling matrix is a block matrix where each block is a symmetric positive definite matrix. The set of such coupling matrices can be endowed with Riemannian geometry, which enables optimization both linear and non-linear objective functions. We have also shown how the SPD-valued OT setup extend many optimal transport problems to general SPD-valued marginals, including the Wasserstein barycenter and the Gromov-Wasserstein (GW) discrepancy. Experiments in a number of applications confirm the benefit of our approach.

In the appendix Section \ref{sec:appendix_projection}, we discuss the projected version of the SPD-valued OT problem. The robust version is shown to be a metric. As a future research direction, it would be interesting to explore such other properties. Another direction could be on learning of block coupling matrices with different constraints. In Section \ref{trace_mfd_appendix}, we discuss a constraint involving the matrix trace.






% We have shown how SPD-valued OT problem is a metric and allows to extend many optimal transport problems to general SPD-valued marginals, including the Wasserstein barycenter and the Gromov-Wasserstein (GW) discrepancy.

% We have also developed a new manifold geometry for learning the block SPD matrix couplings and demonstrated its utility in various OT problems.  Potential future research directions include developing faster optimization algorithms in the stochastic settings for sub-sampled marginals.





%trace_mfd_appendix

% to a general SPD-valued GW discrepency.


% The primary advantage of such manifold structure is that we can exploit well-established Riemannian optimization toolbox for any optimization problem with block coupling constraints.


% \alertPJ{Thus, we do not rely on any regularization as in standard OT solvers. - We should not write this anywhere in the main paper.} \alertPJ{We could discuss/summarize more novel contributions if needed - e.g., metric property, shape interpolation of tensor fields }



% One potential future research direction is to reduce the computational cost in high-dimensional and large-sample settings. For example, one can utilize stochastic Riemannian optimizers for sub-sampled marginals, as similarly considered in \cite{aude2016stochastic}. 
% \alertPJ{we should write the future work without highlighting computational cost issue. }


\bibliography{references}
\bibliographystyle{icml2022}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newpage
\appendix
\onecolumn


\section{Convergence of block matrix balancing algorithm and validity of retraction}
\label{convergence_bmb_retr_appendix}
In Section \ref{manifold_geometry_sect}, we generalize the matrix scaling algorithm to block matrix cases, which is essential to derive the retraction for the manifold $\M_{m,n}^d$. Here, we empirically show that the algorithm quickly converges and the proposed retraction is valid and satisfies the two conditions: 1) $R_x(0) = x$ and 2) $\D R_x(0)[u] = u$, where $\D f(x)[u]$ is the derivative of a function at $x$ along direction $u$. 



\paragraph{Convergence.} We show in Figure \ref{algorithm_retr_fig} the convergence of the proposed block matrix balancing procedure in Algorithm \ref{bmb_algorithm}. We generate the marginals as random SPD matrices for different dimensions $d$ and size $m,n$. The convergence is measured as the relative gap to satisfy the constraints. We observe that the number of iterations for convergence are similar with different parameters while the runtime increases by increasing the dimension and size. 

\paragraph{Validity of retraction.} The first condition of retraction is easily satisfied as $R_\bGamma(\bzero) = {\rm MBalance}(\bGamma) = \bGamma$. For the second one, we have for any $\bGamma \in \M_{m,n}^d$ and $\bU \in T_\bGamma \M_{m,n}^d$,
\begin{align*}
    \D R_\bGamma(\bzero)[\bU] = \lim_{h \xrightarrow{} 0} \frac{R_\bGamma(h\bU) -R_\bGamma(\bzero)}{h} .
    % = \lim_{t \xrightarrow{} 0} \frac{{\rm MBalance}([\bGamma_{i,j} + t \bU_{i,j} + O(t^2)]_{m \times n}) - \bGamma}{t},
\end{align*}
% where the second equality is from the expansion of the exponential map. 
Hence, we need to numerically verify $R_\bGamma(h\bU) - \bGamma = O(h) \bU$ for any $\bGamma, \bU$. To this end, we compute an approximation error in terms of the inner product on the tangent space $T_\bGamma \M_{m,n}^d$ as
\begin{equation*}
    \varepsilon = \left| \langle {\rm P}_\bGamma( R_\bGamma(h(\bU) - \bGamma )  , \bV \rangle_\bGamma - \langle  h\bU,\bV\rangle_\bGamma \right|,
\end{equation*}
for any $\bV \in T_\bGamma\M_{m,n}^d$ different from $\bU$. In Figure \ref{algorithm_retr_fig}(c), we show that the slope of the approximation error (as a function of $h$) matches the dotted line $h = 0$, which suggests hat the error $\varepsilon = O(1)$, thereby indicating that the retraction is valid.   










\begin{figure*}[!th]
\captionsetup{justification=centering}
    \centering
    \subfloat[]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/retr-algorithm-converge/bmb_convergence_iter.pdf}} 
    \hspace*{5pt}
    \subfloat[]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/retr-algorithm-converge/bmb_convergence.pdf}} 
    \hspace*{5pt}
    \subfloat[]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/retr-algorithm-converge/testretractionfigure.pdf}} 
    \caption{Convergence of Algorithm \ref{bmb_algorithm} in terms of iterations (a), runtime (b), and validity test for retraction (c). For the retraction to be valid, the slope of the continuous line should match the dotted line (which represents the line $h = 0$).}
    \label{algorithm_retr_fig}
\end{figure*}










\section{Discussion on the construction of matrix-valued cost}
\label{cost_choice_appendix}
As highlighted in Proposition \ref{mw_distance_prop}, for ${\rm MW}(\bp, \bq)$ to be a metric, there are some conditions for the cost $[\bC_{i,j}]_{m \times n}$ to satisfy. In the following, we give some examples of how such costs are constructed:
%can be constructed. Suppose the matrix-valued samples are given by $\{ \bX_i \}_{i \in [m]}$, $\{ \bY_j\}_{j\in [n]}$, where $\bX_i, \bY_j \in \sR^{d \times s}$. 
% We first show a specific construction of the cost that satisfies the conditions in Proposition \ref{mw_distance_prop}, and hence, the SPD matrix-valued OT \eqref{reformulated_mw} gives a distance metric ${\rm MW}(\bp, \bq)$.
\begin{enumerate}
    \item Let the samples are given by $\{ \bX_i \}_{i \in [m]}$, $\{ \bY_j\}_{j\in [n]}$, where $\bX_i, \bY_j \in \sR^{d \times s}$.  Define $\bC_{i,j} = d(\bX_i ,\bY_j)^2 \, \bI$, where $d: \sR^{d \times s} \times \sR^{d \times s} \xrightarrow{} \sR_{+}$ is a distance function. 
    \item Let the samples are given by $\{ \bX_i \}_{i \in [m]}$, $\{ \bY_j\}_{j\in [n]}$, where $\bX_i, \bY_j \in \sR^{d \times s}$, where $s\geq d$. Assume the matrix $\bX_i-\bY_j$ has column full rank. Define $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$. 
\end{enumerate}
% \begin{proposition}
% \label{cost_mw_prop}
% The following assumptions and constructions of $\bC_{i,j}$ lead to a valid metric ${\rm MW}(\bp, \bq)$:
% \begin{enumerate}[label=(\arabic*)]
%     \item Given a scalar-valued distance function $d: \sR^{d \times s} \times \sR^{d \times s} \xrightarrow{} \sR_{+}$. Define $\bC_{i,j} = d(\bX_i ,\bY_j) \, \bI$.
%     \item Let the samples are given by $\{ \bX_i \}_{i \in [m]}$, $\{ \bY_j\}_{j\in [n]}$, where $\bX_i, \bY_j \in \sR^{d \times s}$. Assume the matrix $\bX_i-\bY_j$ has column full rank and define $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$. 
% \end{enumerate}
% \end{proposition}
\begin{proof}
(1) The first definition of cost trivially satisfies all the conditions due to the metric properties of a well-defined scalar-valued distance.

(2) For the second definition of cost, The first two conditions, i.e., symmetric and positive definite conditions are easily satisfied and we only need to verify the third condition in Proposition \ref{mw_distance_prop}. The third condition is also satisfied due to the triangle inequality of Mahalanobis distance metric in the vectorized form. That is, for any $\bA \succeq \bzero$, we consider three sets of samples $\{\bX_i\}, \{ \bY_k\}, \{ \bZ_j\} \subset \sR^{d \times s}$. Then we have
\begin{align*}
    \sqrt{\trace(\bC_{i,j} \bA)} &= \sqrt{\trace( (\bX_i - \bZ_j)^\top \bA (\bX_i -\bZ_j) )} \\
    &= \sqrt{(\Vec(\bX_i) -\Vec(\bZ_j))^\top (\bI \otimes \bA) (\Vec(\bX_i) - \Vec(\bZ_j))} \\
    %  \sum_i (\bx_i - \bz_i)^\top \bD (\bx_i - \bz_i) \leq \sum_i\Big( \sqrt{(\bx_i - \by_i)^\top \bD (\bx_i - \by_i)} + \sqrt{ (\by_i -\bz_i)^\top \bD (\by_i - \bz_i) } \Big)^2 \\
    &\leq  \sqrt{(\Vec(\bX_i) - \Vec(\bY_k))^\top (\bI \otimes \bA) (\Vec(\bX_i) - \Vec(\bY_k))} \\
    &\quad + \sqrt{(\Vec(\bY_k) - \Vec(\bZ_j))^\top (\bI \otimes \bA) (\Vec(Y_k) - \Vec(\bZ_j))}\\
    &=  \sqrt{ \trace((\bX_i -\bY_k)^\top \bA (\bX_i - \bY_k)) } + \sqrt{ \trace((\bY_k -\bZ_j)^\top \bA (\bY_k -\bZ_j)) } \\
    &= \sqrt{\trace(\bC_{i,k} \bA)} + \sqrt{\trace(\bC_{k,j} \bA)},
\end{align*}
where $\Vec(\bC)$ denotes the vectorization of matrix $\bC$ by stacking the columns.
\end{proof}

% The requirement that $s \geq d$ is to ensure $\bC_{i,j} \succ \bzero$. Proposition \ref{cost_mw_prop} assumes no structure for the matrix space $\sR^{d \times s}$, and therefore, remains valid for symmetric matrices or positive semi-definite matrices. 




\section{Additional experiments}
In this section, we give additional experiments to further subsantiate the claims made in the main text. 


\subsection{Tensor field optimal transport mass interpolation}
In addition to the experiments presented in the main texts, we also show several other examples of tensor fields here.



\begin{figure*}[!th]
\captionsetup{justification=centering}

    \centering
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/cross-orient/linear-interp.pdf}} 
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/cross-orient/QOT-ellipses_50.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/cross-orient/QOT-ellipses_100.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/cross-orient/QOT-ellipses_500.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/cross-orient/BlockMOT-ellipses.pdf}} \\[5pt]
    
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/multi-orient/linear-interp.pdf}} 
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/multi-orient/QOT-ellipses_50.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/multi-orient/QOT-ellipses_100.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/multi-orient/QOT-ellipses_500.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/multi-orient/BlockMOT-ellipses.pdf}} \\[5pt]
    
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/split/linear-interp.pdf}} 
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/split/QOT-ellipses_50.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/split/QOT-ellipses_100.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/split/QOT-ellipses_500.pdf}}
    \hspace*{5pt}
    \subfloat{\includegraphics[width = 0.18\textwidth, height = 0.1\textwidth]{Figures/split/BlockMOT-ellipses.pdf}} \\[5pt]
    
    \stackunder[5pt]{\includegraphics[width=0.18\textwidth, height = 0.1\textwidth]{Figures/iso-orient/linear-interp.pdf}}{\footnotesize Linear interpolation}
    \hspace*{2.8pt}
    \stackunder[5pt]{\includegraphics[width=0.18\textwidth, height = 0.1\textwidth]{Figures/iso-orient/QOT-ellipses_50.pdf}}{\footnotesize QOT ($\rho = 50$)}
    \hspace*{2.8pt}
    \stackunder[5pt]{\includegraphics[width=0.18\textwidth, height = 0.1\textwidth]{Figures/iso-orient/QOT-ellipses_100.pdf}}{\footnotesize QOT ($\rho = 100$)}
    \hspace*{2.8pt}
    \stackunder[5pt]{\includegraphics[width=0.18\textwidth, height = 0.1\textwidth]{Figures/iso-orient/QOT-ellipses_500.pdf}}{\footnotesize QOT ($\rho = 500$)}
    \hspace*{2.8pt}
    \stackunder[5pt]{\includegraphics[width=0.18\textwidth, height = 0.1\textwidth]{Figures/iso-orient/BlockMOT-ellipses.pdf}}{\footnotesize {\algname}}
    \caption{1-$d$ tensor fields mass interpolation.}
    \label{tensor_field_mass_1d_appendix}
\end{figure*}




\begin{figure*}[!th]
\captionsetup{justification=centering}
    \centering
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/input-ellispses-1.pdf}} 
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/input-ellispses-2.pdf}} 
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/interpol-ellispses-4.pdf}} 
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/BlockMOT-interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/BlockMOT-interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat{\includegraphics[width = 0.11\textwidth, height = 0.11\textwidth]{Figures/2d-bump-donut/BlockMOT-interpol-ellispses-4.pdf}} \\[5pt]
    
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/input-ellispses-1.pdf}}{\footnotesize Input-1}
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/input-ellispses-2.pdf}}{\footnotesize Input-5}
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/interpol-ellispses-2.pdf}}{\footnotesize QOT-2}
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/interpol-ellispses-3.pdf}}{\footnotesize QOT-3}
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/interpol-ellispses-4.pdf}}{\footnotesize QOT-4}
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/BlockMOT-interpol-ellispses-2}}{\footnotesize {\algname}-2} 
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/BlockMOT-interpol-ellispses-3}}{\footnotesize {\algname}-3} 
    \hspace*{0.7pt}
    \stackunder[5pt]{\includegraphics[width=0.11\textwidth, height = 0.11\textwidth]{Figures/2d-smooth-rand/BlockMOT-interpol-ellispses-3}}{\footnotesize {\algname}-4} 
    \caption{2-$d$ tensor fields mass interpolation.} 
    \label{tensor_field_mass_2d_appendix}
\end{figure*}




\subsection{Tensor field Wasserstein barycenter}

We first show how both linear interpolation and QOT solutions are not optimal by comparing the objective value of $\sum_\ell \omega_\ell {\rm MW}_\epsilon(\bar{\bP}, \bP^\ell)$ against the optimal objective, obtained from CVX \citep{grant2014cvx}. This is achieved by initializing our Riemannian optimizers for $\bar{\bP}$ from the linear interpolation and (normalized) QOT. We also include uniform initialization as a benchmark. In Figure \ref{obj_compare_barycenter}, we see that the objective value keeps decreasing even after properly normalizing the barycenter. 

Additionally, we show the barycenter results for $n = 16$ along with convergence with initialization from the QOT solution in Figure \ref{2d_barycenter_n4}. Compared to the convergence where $n = 4$, the QOT solution is much closer to the optimal when $n = 16$.



\begin{figure*}[!th]
\captionsetup{justification=centering}
    \centering
    \subfloat[$t =0.25$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n2/optgap-2-5.pdf}} 
    \hspace*{5pt}
    \subfloat[$t=0.5$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n2/optgap-3-5.pdf}}
    \hspace*{5pt}
    \subfloat[$t = 0.75$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n2/optgap-4-5.pdf}}
    \caption{Convergence of ($n=4$) barycenter update initialized from linear interpolation (li), QOT (qot), and uniform identity (uf).} 
    \label{obj_compare_barycenter}
\end{figure*}



\begin{figure*}[ht]
\captionsetup{justification=centering}
    \centering
    \subfloat[$t =0$]{\includegraphics[width = 0.1\textwidth, height = 0.1\textwidth]{Figures/2d-bary-n4/input-1.pdf}} 
    \hspace*{5pt}
    \subfloat[$t=0.25$]{\includegraphics[width = 0.1\textwidth, height = 0.1\textwidth]{Figures/2d-bary-n4/MOTbarycenter-qot-2-5.pdf}}
    \hspace*{5pt}
    \subfloat[$t=0.5$]{\includegraphics[width = 0.1\textwidth, height = 0.1\textwidth]{Figures/2d-bary-n4/MOTbarycenter-qot-3-5.pdf}}
    \hspace*{5pt}
    \subfloat[$t=0.75$]{\includegraphics[width = 0.1\textwidth, height = 0.1\textwidth]{Figures/2d-bary-n4/MOTbarycenter-qot-4-5.pdf}}
    \hspace*{5pt}
    \subfloat[$t = 1$]{\includegraphics[width = 0.1\textwidth, height = 0.1\textwidth]{Figures/2d-bary-n4/input-2.pdf}} \\[5pt]
    \subfloat[Convergence $t=0.25$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n4/optgap-qot-2-5.pdf}}
    \hspace*{5pt}
    \subfloat[Convergence $t=0.5$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n4/optgap-qot-3-5.pdf}}
    \hspace*{5pt}
    \subfloat[Convergence $t = 0.75$]{\includegraphics[width = 0.24\textwidth, height = 0.2\textwidth]{Figures/2d-bary-n4/optgap-qot-4-5.pdf}}
    \caption{Tensor field Wasserstein barycenter ($n=16$). The convergence for different barycenter is given in (f) to (h).} 
    \label{2d_barycenter_n4}
\end{figure*}





% \section{Additional propositions}

% \begin{proposition}
% \label{smooth_set_prop}
% The set $\M^d_{m,n}(\bP, \bQ)$ is smooth provided there exists at least one feasible element.
% \end{proposition}
% \begin{proof}
% For a given feasible element $\bGamma \in \M^d_{m,n}(\bP ,\bQ)$, we can construct a family of feasible elements. For example, choose $0 < \zeta < \min_{i,j}\{ \lambda_{\min} (\bGamma_{i,j}) \}$. Then we can add/subtract the equal number of $\zeta \bI$ and the result is still feasible. In other words, the set is smooth in an ball around the element $\bGamma$ of radius $\zeta$.
% \end{proof}






\section{Proofs}
\label{proof_sect}

\begin{proof}[Proof of Proposition \ref{smooth_set_prop}]
For a given feasible element $\bGamma \in \M^d_{m,n}(\bP ,\bQ)$, we can construct a family of feasible elements. For example, choose $0 < \zeta < \min_{i,j}\{ \lambda_{\min} (\bGamma_{i,j}) \}$. Then we can add/subtract the equal number of $\zeta \bI$ and the result is still feasible. In other words, the set is smooth in an ball around the element $\bGamma$ of radius $\zeta$.
\end{proof}



\begin{proof}[Proof of Proposition \ref{mw_distance_prop}]
For simplicity, we assume $\bp, \bq > 0$. Otherwise, we can follow \citep{peyre2019computational} to define $\tilde{p}_j = p_j$ if $p_j > 0$ and $1$ otherwise. Then the proof proceeds. 

First, it is easy to verify the symmetry property, i.e., ${\rm MW}(\bp, \bq) = {\rm MW}(\bq, \bp)$. For the definiteness, when $\bp = \bq$, we have $\bC_{i,i} = \bzero$ and $\bC_{i,j} \succ \bzero$ for $i \neq j$. Hence the optimal coupling would be a block diagonal matrix with $\bGamma_{i,i} = p_i \bI$. Hence ${\rm MW}(\bp, \bp) = 0$. For the opposite direction, if ${\rm MW}(\bp, \bq) = 0$, we always need to have $\bGamma_{i,j} = \bzero$, for $i \neq j$ because $\trace(\bC_{i,j} \bGamma_{i,j}) > 0$ for any $\bC_{i,j} \succ \bzero$ and $i \neq j$. Thus we have $\bGamma_{i,i} \neq \bzero$, which gives $\bC_{i,i} = \bzero$ and $\bp = \bq$. 

Finally, for triangle inequality, given $\ba, \bb, \bc \in \Sigma_n$, and optimal matrix coupling $\bGamma, \bDelta$ between $(\ba, \bb)$ and $(\bb, \bc)$, respectively. That is, $\sum_j \bGamma_{i,j} = a_i \bI, \sum_i \bGamma_{i,j} = b_j \bI$ and similarly $\sum_j \bDelta_{i,j} = b_i \bI, \sum_i \bDelta_{i,j} = c_j \bI$. We now follow the same strategy by gluing the coupling $\bGamma, \bDelta$ in \citep{peyre2019computational,villani2021topics}. That is, we define a coupling $\bT$ as
\begin{equation*}
    \bT_{i,j} = \sum_k \frac{1}{2b_k} (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k}), \quad  \forall i,j.
\end{equation*}
We can verify $\bT_{i,j} \in \sS_{+}^d$, given $\bGamma_{i,j}, \bDelta_{i,j} \in \sS_{+}^d$. Furthermore, we have $\forall i,j$,
\begin{align*}
    \sum_{j} \bT_{i,j} &= \sum_k \frac{1}{2b_k} (\bGamma_{i,k} \sum_j \bDelta_{k,j} + \sum_j \bDelta_{k,j} \bGamma_{i,k}) = \sum_k \bGamma_{i,k} = a_i \bI, \\
    \sum_i \bT_{i,j} &= \sum_k \frac{1}{2b_k} (\sum_i\bGamma_{i,k} \bDelta_{k,j} +  \bDelta_{k,j} \sum_i \bGamma_{i,k}) = \sum_k \bDelta_{k,j} = c_j \bI.
\end{align*}
Hence, $[\bT_{i,j}]_{m \times n}$ is a valid coupling between $(\ba, \bc)$. Let $\bP_i = a_i \bI, \bQ_j = c_j \bI$ and the corresponding samples as $\bX, \bY, \bZ$ for measures $\ba, \bb, \bc$ respectively. Then,
\begin{align*}
    {\rm MW}(\ba, \bc) &= \left( \min_{\bA \in \bPi(n,n,d,\bP, \bQ) } \sum_{i,j} \trace \big( \bC_{i,j} \bA_{i,j} \big)   \right)^{1/2} \leq \left( \sum_{i,j} \trace \big( \bC_{i,j} \bT_{i,j} \big) \right)^{1/2} \\
    % &= \left( \sum_{i,j, k} \frac{1}{2 b_k} \trace\Big( (\bX_i - \bZ_j)^\top  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  (\bX_i - \bZ_j) \Big) \right)^{1/2} \\
    &= \left( \sum_{i,j, k} \frac{1}{2 b_k} \trace\Big( \bC_{i,j}  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k}) \Big) \right)^{1/2} \\
    % &\leq \Big( \sum_{i,j, k} \frac{1}{2 b_k} \Big(\sqrt{ \trace \big((\bX_i - \bY_k)^\top  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  (\bX_i - \bY_k) \big)} \\
    &\leq \Big( \sum_{i,j, k} \frac{1}{2 b_k} \Big(\sqrt{ \trace \big( \bC_{i,k}  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  \big)} + \sqrt{ \trace\big( \bC_{k,j}  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k}) \big) } \Big)^2 \Big)^{1/2} \\
    % &+ \sqrt{ \trace\big((\bY_k - \bZ_j)^\top  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  (\bY_k - \bZ_j) \big) } \Big)^2 \Big)^{1/2} \\
    % &\leq \Big( \sum_{i,j,k} \frac{1}{2b_k} \trace \big( (\bX_i - \bY_k)^\top  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  (\bX_i - \bY_k) \big) \Big)^{1/2} \\
    % &+ \Big( \sum_{i,j,k} \frac{1}{2b_k} \trace \big( (\bY_k - \bZ_j)^\top  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  (\bY_k - \bZ_j) \big) \Big)^{1/2} \\
    &\leq \Big( \sum_{i,j,k} \frac{1}{2b_k} \trace \big( \bC_{i,k} (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k})  \big) \Big)^{1/2} + \Big( \sum_{i,j,k} \frac{1}{2b_k} \trace \big( \bC_{k,j}  (\bGamma_{i,k} \bDelta_{k,j} + \bDelta_{k,j} \bGamma_{i,k}) \big) \Big)^{1/2}  \\
    &= \Big( \sum_{i,k} \trace\Big( \bC_{i,k} \bGamma_{i,k} \Big) \Big)^{1/2}+ \Big( \sum_{k,j} \trace\Big( \bC_{k,j} \bDelta_{k,j} \Big) \Big)^{1/2}\\
    &= {\rm MW}(\ba, \bb) + {\rm MW}(\bb, \bc),
\end{align*}
% where the \alertPJ{second inequality is by triangle inequality for a generalized Mahalanobis distance}, i.e.,
% \begin{align*}
%     \trace( (\bX - \bZ)^\top \bD (\bX -\bZ) ) = \sum_i (\bx_i - \bz_i)^\top \bD (\bx_i - \bz_i) &\leq \sum_i\Big( (\bx_i - \by_i)^\top \bD (\bx_i - \by_i) + (\by_i -\bz_i)^\top \bD (\by_i - \bz_i) \Big) \\
%     &= \trace((\bX -\bY)^\top \bD (\bX - \bY)) + \trace((\bY -\bZ)^\top \bD (\bY -\bZ)),
% \end{align*}
where the second inequality is by assumption (iii) of the proposition and the third inequality is due to the Minkowski inequality. This completes the proof. 
\end{proof}




\begin{proof}[Proof of Proposition \ref{orthogonal_proj}]
Following \citep{mishra2016riemannian}, the projection is derived orthogonal to the Riemannian metric \eqref{Riem_metric} as 
\begin{equation}
    {\rm P}_{\bGamma}(\bS) = \argmin_{\bU \in T_\bGamma \M_{m,n}^d} f(\bU) = - g_\bGamma(\bU, \bS) + \frac{1}{2}g_{\bGamma}(\bU, \bU). \label{argmin_projection}  
\end{equation}
The Lagrangian of problem \eqref{argmin_projection} is 
\begin{equation}
    f(\bU) - \trace(\bLambda_i \sum_j \bU_{i,j}) - \trace( \bTheta_j \sum_i \bU_{i,j}), \label{lagrangian}
\end{equation}
where $\bLambda_i$, $\bTheta_j$ are dual variables for $i \in [m], j \in [n]$. The orthogonal projection follows from the stationary conditions of \eqref{lagrangian}.
\end{proof}



\begin{proof}[Proof of Proposition \ref{Riem_grad_hess}]
Given the manifold $\M_{m,n}^d$ is a submanifold of $\bigtimes_{m, n} \sS_{++}^d$ with affine-invariant (AI) Riemannian metric, the Riemannian gradient is given by
\begin{equation*}
    \grad F(\bGamma) = {\rm P}_{\bGamma}([\grad_{\rm ai} F(\bGamma_{i,j})]_{m \times n}) = {\rm P}_{\bGamma}([ \bGamma_{i,j} \{ \nabla F(\bGamma_{i,j}) \}_{\rm S} \bGamma_{i,j}]_{m \times n}),
\end{equation*}
where $\grad_{\rm ai} F(\bX)$ is the Riemannian gradient of $\bX \in \sS_{++}^d$ with AI metric. Similarly,  the Riemannian Hessian $\hess F(\bGamma)[\bU] = \nabla_{\bU} \grad F(\bGamma)$ where here $\nabla$ denotes the covariant derivative (i.e. Riemannian connection). For submanifold, the connection $\nabla_\bU \grad F(\bGamma) = {\rm P}_{\bGamma}([\tilde{\nabla}_{\bU_{i,j}}(\grad F(\bGamma_{i,j}))]_{m \times n})$ where $\tilde{\nabla}$ represents the connection of $\sS_{++}^d$. According to \citep{bhatia2009positive}, $\tilde{\nabla}_{\bU_{i,j}} \grad F(\bGamma_{i,j}) = \D \grad F(\bGamma_{i,j})[\bU_{i,j}] - \{ \bU_{i,j} \bGamma_{i,j}^{-1} \grad F(\bGamma_{i,j}) \}_{\rm S}$. Hence, the proof is complete.
\end{proof}





% \begin{proof}[Proof of Proposition \ref{retraction_prop}]
% To prove this is indeed a retraction, we need to verify the two conditions, i.e., 1) $R_x(0) = x$ and 2) $\D R_x(0)[u] =u$ for any $\xi \in T_x\M$. 

% The first condition is satisfied trivially, as $R_\bGamma(\bzero) = {\rm MBalance}(\bGamma) = \bGamma$ for $\bGamma \in \M_{m,n}^d$. For the second condition, given $\bGamma \in \M_{m,n}^d$, we have $\tilde{\bL}_i = \tilde{\bR}_j = \bI$ from the uniqueness assumption. Recall the constraints are
% \begin{align*}
%     \sum_i  \tilde{\bL}_i \tilde{\bR}_j \bGamma_{i,j} \tilde{\bR}_j \tilde{\bL}_i &= \bQ_j,\\
%     \sum_j \tilde{\bL}_i \tilde{\bR}_j \bGamma_{i,j} \tilde{\bR}_j \tilde{\bL}_i &= \bP_i.
% \end{align*}
% Taking differential on both sides and ignoring higher order terms yields
% \begin{equation}
%     \sum_i ( \{\partial \tilde{\bL}_i \bGamma_{i,j} \}_{\rm S} + \{\partial \tilde{\bR}_j \bGamma_{i,j} \}_{\rm S}) = \sum_{j} (\{\partial \tilde{\bL}_i \bGamma_{i,j} \}_{\rm S} + \{\partial \tilde{\bR}_j \bGamma_{i,j}\}_{\rm S}) = \bzero, \label{inter_result1}
% \end{equation}
% where $\{ \bA\}_{\rm S} := (\bA + \bA^\top)/2$ and we also uses the fact that $\tilde{\bL}_i = \tilde{\bR}_j = \bI$, following from the assumption of unique form.\footnote{Although the factors are unique up to scaling, we can assume $\tilde{\bL}_i = \tilde{\bR}_j = \bI$ without loss of generality because the scaling has been accounted for in $\partial \tilde{\bL}_i, \partial \tilde{\bR}_j$.} One can verify that the choice of $\partial \tilde{\bL}_i = -\partial \tilde{\bR}_j = \alpha \bI$ for any $\alpha$ satisfies the equation. Further, the two equations in \eqref{inter_result1} concerns $m + n$ block equations with respect to $m+n$ block variable $\tilde{\bL}_i, \tilde{\bR}_j$, $i \in [m], j \in [n]$. This suggests the choice is unique up to a scaling factor. Hence $2\{ \partial \tilde{\bL}_i \bGamma_{i,j}\}_{\rm S} + 2\{ \partial \tilde{\bR}_j \bGamma_{i,j}\}_{\rm S} = \bzero$ $\forall i, j$. From the first order expansion of MBalance,
% \begin{align*}
%     {\rm MBalance}(\bGamma + \partial \bGamma) &\approx [(\tilde{\bL}_i + \partial \tilde{\bL}_i)(\tilde{\bR}_j + \partial \tilde{\bR}_j)(\bGamma_{i,j} + \partial \bGamma_{i,j})(\tilde{\bR}_j + \partial \tilde{\bR}_j)(\tilde{\bL}_i + \partial \tilde{\bL}_i)]_{m \times n} \\
%     &\approx \bGamma + \partial \bGamma + [2\{ \partial \tilde{\bL}_i \bGamma_{i,j}\}_{\rm S} + 2\{ \partial \tilde{\bR}_j \bGamma_{i,j}\}_{\rm S}]_{m\times n} \\
%     &= \bGamma + \partial \bGamma,
% \end{align*}
% which in turn finally leads to
% \begin{align*}
%     \D R_\bGamma(\bzero)[\bU] &= \lim_{t\xrightarrow{} 0} \frac{R_\bGamma(t\bU) - R_{\bGamma}(\bzero)}{t} \\
%     &= \lim_{t\xrightarrow{} 0} \frac{{\rm MBalance}([\bGamma_{i,j} + t\bU_{i,j}  + O(t^2)]_{m \times n}) - \bGamma}{t}  \qquad  (\text{expansion of } {\rm exp}) \\
%     &= \lim_{t\xrightarrow{} 0} \frac{[\bGamma_{i,j} + t\bU_{i,j}  ]_{m \times n} - \bGamma}{t} \\
%     &= \bU,
% \end{align*}
% where the second equality uses the expansion of the expenential map.  
% \end{proof}











\begin{proof}[Proof of Theorem \ref{Prop_Riem_opt_optimal}]
We first write the Lagrange dual function as
\begin{align*}
    g(\bLambda, \bTheta, \bPsi)
    = &\min_{\bGamma = [\bGamma_{i,j}]_{m \times n} } F(\bGamma) + \sum_i \trace \Big( \bLambda_i \big( \sum_j \bGamma_{i,j} - \bP_i \big) \Big)
    + \sum_j \trace\Big(  \bTheta_j \big( \sum_{i} \bGamma_{i,j} - \bQ_j \big) \Big)  - \sum_{i,j} \trace \Big( \bPsi_{i,j} \bGamma_{i,j} \Big),
\end{align*}
where we relax the SPD constraint on $\bGamma_{i,j}$ to the semidefinite constraint, i.e. $\bGamma_{i,j} \succeq \bzero$, for some dual variable $\bLambda_i, \bTheta_j \in \sS^d$ and $\bPsi_{i,j} \succeq \bzero$. Given the function $F$ is convex with non-empty constraint set, by Slater's condition, strong duality holds and the primal and dual variables should jointly satisfy the KKT conditions. 

First, we notice by complementary slackness, $\trace (\bPsi_{i,j}^* \bGamma_{i,j}^*) = 0$ for $\bGamma_{i,j}^* \succ \bzero$. This implies that $\bPsi_{i,j}^* =\bzero$ since $\bPsi_{i,j}^* \succeq \bzero$. Note that in some cases $\bGamma_{i,j}^*$ may be rank-deficient (i.e., some eigenvalues are close to zero), which gives rise to non-zero $\bPsi_{i,j}^*$. Regardless, from the optimality condition, it always satisfies for optimal $\bGamma_{i,j}^*$, $\bLambda_i^*$, $\bTheta_j^*$,
\begin{equation}
    \bGamma_{i,j}^* (\nabla F(\bGamma_{i,j}^*) + \bLambda_i^* + \bTheta_j^*) \bGamma_{i,j}^* = \bzero, \label{main_kkt_cond}
\end{equation}
due to that $\bGamma_{i,j}^*$ is orthogonal to $\bPsi_{i,j}^*$. $\nabla F(\bGamma_{i,j}^*)$ denotes the block partial derivative of $F$ with respect to $\bGamma_{i,j}$ at optimality. 

On the other hand, to perform Riemannian optimization, the Riemannian gradient is first computed for the primal objective $F$ as  
\begin{align*}
    {\rm grad} F(\bGamma) = {\rm P}_\bGamma( [\bGamma_{i,j} \{ \nabla F(\bGamma_{i,j}) \}_{\rm S} \bGamma_{i,j} ]_{m\times n}), 
\end{align*}
which from the definition of orthogonal projection, gives 
\begin{equation*}
    {\rm grad} F(\bGamma_{i,j}) = \bGamma_{i,j} \Big( \nabla F(\bGamma_{i,j}) + \tilde{\bLambda}_i + \tilde{\bTheta}_j  \Big) \bGamma_{i,j},
\end{equation*}
where ${\rm grad} F(\bGamma_{i,j})$ represents the Riemannian partial derivative and $\tilde{\bLambda}_i, \tilde{\bTheta}_j \in \sS^d$ are computed such that 
\begin{align}
\begin{cases}
    \sum_{i} \bGamma_{i,j} ( \bC_{i,j} + \epsilon \nabla \Omega(\bGamma_{i,j}^*) + \tilde{\bLambda}_i + \tilde{\bTheta}_j) \bGamma_{i,j} = \bzero, & \forall j \\
    \sum_{j} \bGamma_{i,j} (\bC_{i,j} + \epsilon \nabla \Omega(\bGamma_{i,j}^*) + \tilde{\bLambda}_i + \tilde{\bTheta}_j) \bGamma_{i,j} = \bzero, & \forall i.
\end{cases}
\label{gradient_proj_cond}
\end{align}
Comparing \eqref{gradient_proj_cond} to \eqref{main_kkt_cond}, we see that at optimality, there exists $\bLambda_i^*, \bTheta_j^*$ such that for all $i, j$, the conditions \eqref{gradient_proj_cond} are satisfied, with $\tilde{\bLambda}_i =  \bLambda_i^* + \Delta, \tilde{\bTheta}_j = \bTheta_j^* - \Delta$, for any symmetric matrix $\Delta$. Hence, the Riemannian gradient at optimality ${\rm grad} F(\bGamma_{i,j}^*) = \bzero$, thus completing the proof. 
\end{proof}









\begin{proof}[Proof of Proposition \ref{dual_var_solution_prop}]
For each regularized OT problem, we consider the Lagrange dual problem of $\min_{\bGamma \in \M_{m,n}^d} {\rm MW}_\epsilon(\bar{\bP}, \bP^\ell)$, which is given as 
\begin{align}
    \L_{{\rm MW}_\epsilon} = \max_{\substack{\bLambda_i^\ell, \, \bTheta_j^\ell \in \sS^d \\ \bPsi_{i,j}^\ell \succeq \bzero}} \Big( \min_{\bGamma_{i,j}^\ell} \sum_{i,j} \big( \trace(\bC_{i,j}^\ell \bGamma_{i,j}^\ell) + \epsilon \, \Omega(\bGamma_{i,j}^\ell) \big)  & + \sum_i \trace\big( \bLambda_i^\ell \big(\sum_j \bGamma_{i,j}^\ell - \bar{\bP}_i \big) \big) \nonumber\\
    &\, + \sum_j \trace \big( \bTheta_j^\ell \big( \sum_{i} \bGamma_{i,j}^\ell - \bP^\ell_j \big) \big) - \sum_{i,j} \trace \big( \bPsi_{i,j}^\ell \bGamma_{i,j}^\ell \big)  \Big). \label{dual_problem_dual_var}
\end{align}
From the Lagrangian (\ref{dual_problem_dual_var}), it is easy to see the Euclidean gradient of the barycenter problem with respect to $\bar{\bP}_i$ is $-\sum_\ell \bLambda_i^\ell$ with the dual optimal $\bLambda_i^\ell$ for problem \eqref{dual_problem_dual_var}. Next, the proof is complete by substituting the objective $F(\bGamma) = \sum_{i,j} \big( \trace(\bC_{i,j} \bGamma_{i,j} + \epsilon \Omega(\bGamma_{i,j})) \big)$ as in Theorem \ref{Prop_Riem_opt_optimal}.
\end{proof}






\begin{proof}[Proof of Proposition \ref{average_distance_update}]
First we rewrite SPD matrix-valued GW discrepancy as 
\begin{align*}
    {\rm MGW}\big((\bar{\bD}, \bar{\bP}), (\bD^\ell, \bP^\ell) \big) &= \sum_{i,i',j,j'} \Big(  f_1(\bar{D}_{i,i'}) + f_2(D^\ell_{j,j'}) -h_1(\bar{D}_{i,i'}) h_2({D}^\ell_{j,j'}) \Big) \trace(\bGamma^\ell_{i,j} \bGamma^\ell_{i',j'}) \\
    &= \sum_{i,j} \trace \Big( \bGamma_{i,j} \Big( \sum_{i'} f_1(\bar{D}_{i,i'}) \bar{\bP}_{i'}  + \sum_{j'} f_2(D^\ell_{j,j'}) \bP^\ell_{j'} - \sum_{i'} h_1(\bar{D}_{i,i'}) \sum_{j'} h_2(D^\ell_{j,j'}) \bGamma^\ell_{i',j'} \Big)  \Big),
\end{align*}
where we use the fact that $\bGamma^\ell_{i,j}$ are optimal and satisfy the constraints $\sum_j \bGamma^\ell_{i,j} = \bar{\bP}_i$ and $\sum_i \bGamma^\ell_{i,j} = \bP^\ell_j$. By the first order condition, we have 
\begin{equation*}
    \trace \Big( \bar{\bP}_i  f_1'(\bar{D}_{i,i'}) \bar{\bP}_{i'} - h_1'(\bar{D}_{i,i'}) \sum_j \bGamma_{i,j}  \big( \sum_{j'} h_2(D^\ell_{j,j'}) \bGamma^\ell_{i',j'} \big) \Big) = 0, \quad \forall i,i' \in [m],
\end{equation*}
which gives the desired result.
\end{proof}









% \section{Efficient optimization via projection}
% \label{proj_appendix}
% Although problem \eqref{eq:manifold_problem} can be solved in a unified framework for any block-wise objective function $F$, the computational cost can greatly increase when the dimension $d$ increases, as discussed in the Section \ref{convergence_complexity_sect}. Here we consider a projected variant of the problem in the form of
% \begin{equation*}
%     \min_{\bGamma \in \M_{m,n}^r} \min_{\bW \in {\rm St}(d,r)} \sum_{i,j} f_{i,j}( \bW^\top \bGamma_{i,j} \bW),
% \end{equation*}
% where we use $f_{i,j}$ as the block-wise component function of $F$. The projection matrix $\bW \in \sR^{d\times r}$ ($r < d$) and satisfies $\bW^\top \bW = \bI$. The set of such column orthonormal matrices can be endowed with a manifold structure, known as the Stiefel manifold ${\rm St}(d,r)$. This problem is nontrivial even for entropy regularized objective. Nevertheless, it can be solved easily by Riemannian optimization with respect to a product of manifold $\M_{m,n}^d \times {\rm St}(d,r)$. See \cite{absil2009optimization,boumal2020intromanifolds} for more details.

% In this case, optimization of coupling is on the space of $\M_{m,n}^r$, thus reducing the per-iteration complexity to $O(mnr^3)$. Optimization over the projection matrix is relatively cheap with many efficient retraction, all taking at most a complexity of $O(d^2r)$. Thus the total per-iteration complexity is given by $O(mnr^3 + d^2r)$. 


% \paragraph{Application in domain adaptation.}
% The above framework can be easily applied in domain adaptation applications where the objective is 
% \begin{equation*}
%     \min_{\bGamma \in \M_{m,n}^r} \min_{\bW \in {\rm St}(d,r)} \sum_{i,j} \Big( \trace(\bC_{i,j} \bW\bGamma_{i,j} \bW^\top ) \Big),
% \end{equation*}
% for the same cost $\bC_{i,j} \in \sS_{++}^d$ on high-dimensional space. The barycentric projection can be similarly derived by replacing the $\bY_j$ with its projection $(\bW^*)^\top \bY_j$ in \eqref{barycentric_proj}. 





















\section{Projection and ${\rm MW}$ (\ref{reformulated_mw}) for probability measures}\label{sec:appendix_projection}

For given marginals $\bp\in\Sigma_m$ and $\bq\in\Sigma_n$, i.e., $\sum_i p_i = \sum_j q_j = 1$, for $p_i, q_j \geq 0$, we consider the corresponding block SPD marginals $\bP$ and $\bQ$ be defined as $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$ in the $d \times d$ space and so are the cost matrices $[\bC_{i,j}]_{m \times n}$.


For this case, we introduce a projected variant of the SPD matrix-valued optimal transport problem by parameterizing the coupling block-matrix $[\bGamma_{i,j}]_{m\times n}$ as $\bGamma_{i,j} = \bW \bGamma^{r}_{i,j} \bW^\top$, where $\bGamma^{r}_{i,j} \succeq \bzero$ is of size $r\times r$ and $\bW \in \mathbb{R}^{d \times r}$. Imposing the projection constraint that $\bW^\top \bW = \bI^r$ ($r \times r$ identity matrix), we observe the new block-SPD marginals $[\bGamma^r_{i,j}]_{m\times n}$ become consistent for the probability measures $\bp$ and $\bq$. Equivalently, $\bP^r\coloneqq\{[\bP^r_i]_{m\times 1}:\bP^r_i = p_i \bI^r\}$ and $\bQ^r\coloneqq\{[\bQ^r_j]_{n\times 1}:\bQ^r_j = q_i \bI^r\}$. In other words, both $\bP$ and $\bP^r$ can be considered as the lifting of $\bp$ but onto different spaces. Similarly for $\bQ$ and $\bQ^r$. In particular, the cost $\bC^r_{i.j}$ is related to $\bC_{i,j}$ as $\bC^r_{i,j} = \bW^\top\bC_{i,j} \bW$. This motivates to consider the formulation
\begin{equation}\label{eq:projection_MW}
    \underset{\bW^\top \bW = \bI^r}{\min {\text / }\max} \sum_{i,j} \min_{\bGamma^r \in \bPi(m,n,r, \bP^r, \bQ^r) } {\rm MW}^2(\bp, \bq; \bW) \coloneqq  \trace(\bC_{i,j} \bW\bGamma^r_{i,j} \bW^\top )  = \trace(\bW^\top\bC_{i,j} \bW\bGamma^r_{i,j}  ),
\end{equation}
which aims to simultaneously optimize the coupling as well as a projection $\bW \in \sR^{d\times r}$. For learning the optimal projection $\bW$ in (\ref{eq:projection_MW}), both minization and maximization make sense depending on applications. 

Let us define the projection robust ${\rm MW}$ OT problem as
\begin{equation}\label{eq:robust_projection_MW}
    {\rm PRMW}^2_r(\bp, \bq)  = \max\limits_{\bW^\top \bW = \bI^r} \sum_{i,j} \min_{\bGamma^r \in \bPi(m,n,r, \bP^r, \bQ^r) } {\rm MW}^2(\bp, \bq; \bW).
\end{equation}

\begin{proposition}\label{prop:PRMW}
Suppose the marginals $\bp, \bq \in \Sigma_n$ have the same support, the cost matrices $[\bC_{i,j}]_{m \times n}$ satisfy the properties in Proposition \ref{mw_distance_prop}, and ${\rm MW}(\bp,\bq)$ is a metric between the marginals $\bp$ and $\bq$. Then, ${\rm PRMW}(\bp, \bq)$ is also a metric between the marginals $\bp$ and $\bq$.
\end{proposition}
\begin{proof}
As the cost matrices $[\bC_{i,j}]_{m \times n}$ satisfy the properties in Proposition \ref{mw_distance_prop}, it is easy to see that the cost matrices $[\bC^r_{i,j}]_{m \times n}$ satisfy the properties as well. Consequently, ${\rm MW}(\bp, \bq ; \bW)$ is a metric for a given projection matrix $\bW$.

It is straightforward to see that ${\rm PRMW}_r(\bp, \bq) = {\rm PRMW}_r(\bq, \bp)$ and ${\rm PRMW}_r(\bp, \bq) = 0$ if and only if  $\bp = \bq$. The remaining property of triangle inequality for ${\rm PRMW}_r(\bp, \bq)$ follows as shown below. Let 
\begin{equation}\label{eq:argmaPRMW}
    \bW^* = \argmax\limits_{\bW^\top \bW = \bI^r} \sum_{i,j} \min_{\bGamma^r \in \bPi(m,n,r, \bP^r, \bQ^r) } {\rm MW}^2(\bp, \bq; \bW).
\end{equation}
Therefore, from (\ref{eq:argmaPRMW}), we have
\begin{equation*}
    \begin{array}{lll}
    {\rm PRMW}_r(\bp, \bq) & = & {\rm MW}(\bp, \bq; \bW*) \\
    & \leq & {\rm MW}(\bp, \tilde{\bq}; \bW^*) + {\rm MW}(\tilde{\bq}, \bq; \bW^*) \text{ as } {\rm MW} \text{ is a metric} \\
    & \leq & {\rm PRMW}_r(\bp, \tilde{\bq}) + {\rm PRMW}_r(\tilde{\bq}, \bq).
    \end{array}
\end{equation*}
This completes the proof.
\end{proof}




% Although problem \eqref{MW_mot_restate} can be solved in a unified framework for any well-defined cost matrix $\bC_{i,j}$ as well as the marginals, the computational cost can greatly increase when the dimension $d$ increases. To mitigate this issue, we introduce a projected variant of matrix-valued optimal transport. This is achieved by simultaneously optimizing the coupling as well as a projection $\bW \in \sR^{d\times r}$ ($r < d$) and $\bW^\top \bW = \bI$. That is
% \begin{equation*}
%     \min_{\bGamma \in \M_{m,n}^r} \min_{\bW \in {\rm St}(d,r)} \sum_{i,j} \Big( \trace(\bC_{i,j} \bW\bGamma_{i,j} \bW^\top ) \Big),
% \end{equation*}
% where ${\rm St}(d,r)$ is the Stiefel manifold, the set of $d \times r$ column orthonormal matrices. This problem is nontrivial even for entropy regularized objective. Nevertheless, it can be solved easily by Riemannian optimization with respect to a product of manifold $\M_{m,n}^d \times {\rm St}(d,r)$. 

% % \alertAH{Show this is a distance metric.}\alertBM{the distance metric is only possible to projection robust matrix-valued ot, i.e., we have maximization with W.}

% % \paragraph{Barycentric projection.} 
% For the application of domain adaptation, the barycentric projection can be similarly derived by replacing the $\bY_j$ with its projection $(\bW^*)^\top \bY_j$ in \eqref{barycentric_proj}. 

% % \alertBM{this is not correct. We can only estimate W'Xhat and not Xhat. and W'Xhat is equal to (8) where Gamma is replaced by Gamma*W'.We write that explicitly here.}






































\section{Trace-constrained \manname}
\label{trace_mfd_appendix}
 
Given the set $\M^d_{m,n}$ might be empty for general block-SPD marginals, here we consider a relaxation of the coupling constraint, where only the sum of traces of the row and columns blocks need to be matched with the trace of block-SPD marginals  \citep{peyre2016quantum,ning2014matrix}.
% \alertBM{cite more papers}. 
That is,
\begin{equation*}
\begin{array}{ll}
    \widetilde{\M}^d_{m,n}(\bp, \bq) 
    \coloneqq \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \sum_{j} \trace(\bGamma_{i,j}) = p_i, \sum_i \trace(\bGamma_{i,j}) = q_j  \},
\end{array}
\end{equation*}
where $\sum_{i} p_i = \sum_j q_j = 1$. We show such set can also be endowed with a manifold structure, thus facilitating optimization with such constraint.

% The trace-constrained extension has also been considered in \citep{peyre2016quantum} while we here discuss the manifold approach that is more flexible and it allows optimization of any nonlinear objective function.

% \alertBM{How to properly contrast with earlier works.}



% Here, we provide a complete characterization of the optimization-related ingredients on the trace-constrained \manname $\widetilde{\M}^d_{m,n}$.

The tangent space characterization of $\widetilde{\M}^d_{m,n}$ at $\bGamma$ is given by 
\begin{align*}
    T_\bGamma \widetilde{\M}^d_{m,n} = \{ &[\bU_{i,j}]_{m \times n} : \bU_{i,j} \in \sS^d, \\
    &\sum_{i} \trace(\bU_{i,j}) = 0, \sum_j \trace(\bU_{i,j}) = 0  \}.
\end{align*}
With the same Riemannian metric in \eqref{Riem_metric}, the orthogonal projection (Proposition \ref{orthogonal_proj}) can be simplified as
\begin{equation}
    \widetilde{{\rm P}}_{\bGamma}(\bS) = \bU, \text{ with } \bU_{i,j} = \bS_{i,j} + (\lambda_i + \theta_j) \bGamma_{i,j}^2, \label{proj_tilde}
\end{equation}
where $\lambda_i, \theta_j$ can be computed from 
\begin{equation*}
\begin{cases}
    -\sum_i \trace(\bS_{i,j}) = \sum_{i} (\lambda_i + \theta_j) \trace(\bGamma_{i,j}^2), & \forall j, \\
    -\sum_j \trace(\bS_{i,j}) = \sum_{j} (\lambda_i + \theta_j) \trace(\bGamma_{i,j}^2) , & \forall i.
\end{cases}
\end{equation*}
The Riemannian gradient and Hessian exactly follows from Proposition \ref{Riem_grad_hess} with projection replaced by \eqref{proj_tilde}. 


\paragraph{Retraction and trace-constrained block matrix balancing algorithm.} 

Although we can follow the same iterative strategy of normalizing the rows and columns as in Algorithm~\ref{bmb_algorithm}, one na\"ive and efficient alternative is to simply solve a classic scalar OT problem for the trace of each block. 

Denote $\tilde{a}_{i,j} = \trace(\bA_{i,j})$ and consider a matrix $\tilde{\bA} = [\tilde{a}_{i,j}]_{m\times n}$, with $\tilde{a}_{i,j} > 0$. We can perform the scalar Sinkhorn algorithm with marginals $\bp$ and $\bq$, which gives a balanced matrix $\tilde{\bB}$ that satisfies $\tilde{\bB}\bone = \bp$ and $\tilde{\bB}^\top \bone = \bq$. Denote its entries as $\tilde{b}_{i,j}$. Then the block matrix that satisfies the trace coupling constraints is given by $[\bB_{i,j}]_{m \times n}$ with $\bB_{i,j} = \frac{\tilde{b}_{i,j}}{\tilde{a}_{i,j}} \bA_{i,j}$ because we see $\sum_i \trace(\bB_{i,j}) = \sum_i \tilde{b}_{i,j} = \nu_j, \forall j$ and $\sum_j \trace(\bB_{i,j}) = \mu_i$. We notice that there are many other approaches to perform diagonal scaling such that the trace coupling constraints are satisfied. See Section \ref{other_approach_trace_appendix} for more details.



Similar to \eqref{retr_define}, the retraction is given by 
\begin{equation*}
    R_\bGamma(\bU)  = {\rm trBalance}([\bGamma_{i,j} \exp(\bGamma_{i,j}^{-1} \bU_{i,j}) ]_{m \times n}), 
\end{equation*}
where ${\rm trBalance}$ denotes the process of balancing the trace of matrix to satisfy the coupling constraints. To verify this is indeed a retraction, we follow the same strategy as in \citep{douik2019manifold,shi2021coupling}. This is formalized in Proposition \ref{trace_retraction_prop}.

\begin{proposition}
\label{trace_retraction_prop}
The operation $R_\bGamma(\bU)  = {\rm trBalance}([\bGamma_{i,j} \exp(\bGamma_{i,j}^{-1} \bU_{i,j}) ]_{m \times n})$ is a valid retraction for the manifold $\widetilde{\M}^d_{m,n}$.
\end{proposition}
\begin{proof}


The first condition of retraction is clearly satisfied. For the second condition, Sinkhorn's Theorem shows that for any positive matrix $\tilde{\bA}$, it can be scaled to a unique coupling matrix of the form $\tilde{\bB} = \bD_1 \tilde{\bA} \bD_2$, where the diagonal matrices $\bD_1, \bD_2$ are unique up to scaling \citep{sinkhorn1964relationship}. 
Suppose the scaling is given by $\alpha_i \beta_j \bA_{i,j}$ with $\alpha_i, \beta_j > 0, \forall i,j$. Then we can easily verify that $\alpha_i \beta_j = \tilde{b}_{i,j}/\tilde{a}_{i,j}$ are unique. This simply follows from the uniqueness of the scaling factors for $\tilde{\bA}$. 

Given $[\bGamma_{i,j}] \in \widetilde{\M}^d_{m, n}$ and also $[\alpha_i \beta_j \bGamma_{i,j}] \in \widetilde{\M}^d_{m, n}$, we see $\alpha_i = \beta_j = 1$ by uniqueness. From the constraint $\sum_i \trace(\alpha_i \beta_j \bGamma_{i,j}) = \nu_j$, $ \sum_j \trace(\alpha_i \beta_j \bGamma_{i,j}) = \mu_i$, we take differential of both sides, which gives
\begin{equation*}
    \sum_i \trace(\partial \alpha_i  \bGamma_{i,j} + \partial \beta_j \bGamma_{i,j}) =  \sum_j \trace(\partial \alpha_i \bGamma_{i,j} + \partial \beta_j \bGamma_{i,j}) = 0.
\end{equation*}
Using similar argument, we can verify $\partial \alpha_i = - \gamma \partial \beta_j$ and thus it gives ${\rm trBalance}(\bGamma + \partial\bGamma) \approx \bGamma + \partial \bGamma$. This further leads to $\D R_\bGamma(\bzero)[\bU] = \bU$.
\end{proof}



\subsection{Alternative balancing approaches for trace coupling constraint}
\label{other_approach_trace_appendix}

Alternatively, we may consider a matrix log-barrier formulation as follows. Let $\bc_j \in \sR^d_{++}$, $j \in [m]$ and $\br_i \in \sR^d_{++}$, $i \in [n]$ be two sets of positive scaling factors. We consider the following optimization problem:
\begin{align}
    \min \,\, g(\bc_{1:m}, \br_{1:n}) &\coloneqq \sum_{i,j} \trace( {\rm diag}(\bc_j) {\rm diag}(\br_i) \bA_{i,j} {\rm diag}(\br_i) {\rm diag}(\bc_j) ) \nonumber \\
    - & \frac{2}{d}\sum_i \mu_i \log\det({\rm diag}(\br_i)) - \frac{2}{d} \sum_j \nu_j \log\det({\rm diag}(\bc_j)) \label{log_barrier_opt}
\end{align}
This problem is clearly convex for each argument given the other fixed. Hence, one strategy is block coordinate descent. The first order conditions are given by
\begin{align}
    \frac{\partial g}{\partial \bc_j} &= 2 \sum_i  (\br_i)^2 \odot {\rm diag}(\bA_{i,j}) \odot \bc_j - \frac{2 \nu_j}{d}  \bc_j^{-1}  = \bzero, \quad \forall j \label{cj_foc}\\
    \frac{\partial g}{\partial \br_i} &= 2 \sum_j  (\bc_j)^2 \odot {\rm diag}(\bA_{i,j}) \odot \br_i - \frac{2 \mu_i}{d}  \br_i^{-1} = \bzero, \quad \forall i \label{ri_foc},
\end{align}
where the $\odot$ and the square stand for elementwise product and elementwise square. ${\rm diag}$ represents the diagonal operation as either extracting the diagonal elements or forming a diagonal matrix depending on the input. $\bone$ denotes the vector of all ones. 

This gives an alternating strategy to update the variables similar to the classic Sinkhorn-Knopp algorithm
\begin{align}
\begin{array}{cc}
     \bc_j &\xleftarrow{} \Big( \nu_j \bone \big{/} \big(d \sum_i (\br_i)^2 \odot {\rm diag}(\bA_{i,j}) \big) \Big)^{1/2}, \quad \forall j \\
    \br_i &\xleftarrow{} \Big( \mu_i \bone \big{/} \big( d \sum_j (\bc_j)^2 \odot {\rm diag}(\bA_{i,j}) \big) \Big)^{1/2}, \quad \forall i. \label{mat_trace_update}
\end{array}
\end{align}

We notice that any stationary points $\br_i^*, \bc_j^*, \forall i,j$ satisfying \eqref{cj_foc}, \eqref{ri_foc} scale the block SPD matrices to satisfy the row and column trace constrained. This is because
\begin{align*}
    \sum_i \trace( {\rm diag}(\bc_j^*) {\rm diag}(\br_i^*) \bA_{i,j} {\rm diag}(\br_i^*) {\rm diag}(\bc_j^*)) &= \sum_i \big( (\bc_j^*)^2 \odot  (\br_i^*)^2 \odot {\rm diag}(\bA_{i,j}) \big)^\top \bone \\
    &= \sum_i \big( \nu_j/d \bone \big)^\top \bone = \nu_j.
\end{align*}
The similar result holds for row sum. Hence, for any block SPD matrix $\bA$, it can be scaled to satisfy the row and column trace sum constrained if and only if the optimization \eqref{log_barrier_opt} has a stationary point. From here, many existing results concerning existence and uniqueness as well as convergence are readily applied because the iterative update in \eqref{mat_trace_update} is a multivariate version of classic Sinkhorn-Knopp update applied elementwise. See for example \citep{knight2008sinkhorn}.









\section{Riemannian geometry for block SPD Wasserstein barycenter}
\label{geometry_spd_simplex_appendix}

\paragraph{Riemannian geometry of $\Delta_n (\sS_{++}^d)$.}

In \cite{mishra2019riemannian}, the authors endow a Riemannian manifold structure for the set $\Delta_n (\sS_{++}^d) \coloneqq \{ \bP = [\bP_i]_{n \times 1} : \sum_i \bP_i = \bI \}$. The manifold is defined as 
\begin{equation*}
    \Delta_n (\sS_{++}^d) \coloneqq \{ (\bP_1,  \bP_2, ..., \bP_n) : \bP_i \in \sS_{++}^d, \sum_i \bP_i = \bI \}.
\end{equation*}
Its tangent space is given by 
\begin{equation*}
    T_\bP \Delta_n (\sS_{++}^d) = \{ (\bU_1, ..., \bU_n) : \bU_i \in \sS^d, \sum_i \bU_i = \bzero \}.
\end{equation*}
By introducing a similar affine-invariant metric $\langle \bU, \bV \rangle_\bP = \sum_i \trace(\bP_i^{-1} \bU_i \bP_i^{-1} \bV_i)$. The retraction from the tangent space to manifold is derived as 
\begin{equation*}
    R_\bP(\bU) = (\hat{\bP}^{-1/2}_{\rm sum} \hat{\bP}_1 \hat{\bP}^{-1/2}_{\rm sum}, ..., \hat{\bP}^{-1/2}_{\rm sum} \hat{\bP}_n \hat{\bP}^{-1/2}_{\rm sum}),
\end{equation*}
where $\hat{\bP}_i = \bP_i (\exp(\bP_i^{-1} \bU_i) )$ and $\hat{\bP}_{\rm sum} = \sum_i \hat{\bP}_i$. 

The Riemannian gradient of a function $F:\Delta_n (\sS_{++}^d) \to \mathbb{R}$ is computed as 
\begin{equation*}
    \grad F(\bP) = {\rm P}_{\bP} \Big( \big(\bP_1 \{ \nabla F(\bP_1) \}_{\rm S} \bP_1, ..., \bP_n \{ \nabla F(\bP_n) \}_{\rm S} \bP_n \big) \Big),
\end{equation*}
where the orthogonal projection $\rm{P}_{\bP}$ of a of $\bS = (\bS_1,  \bS_2, ..., \bS_n)$ such that $\bS_i \in \sS^d$ is
\begin{equation*}
    {\rm P}_\bX(\bS) = (\bS_1 + \bP_1 \bLambda \bP_1, ..., \bS_n + \bP_n \bLambda \bP_n),
\end{equation*}
where $\bLambda \in \sS^d$ is the solution to the linear equation $\sum_i \bP_i \bLambda \bP_i = - \sum_i \bS_i$.



\paragraph{Optimization for Wasserstein barycenter.}

With the Riemannian geometry defined for the simplex of SPD matrices, we can update the barycenter by Riemannian optimization as shown in Algorithm \ref{wb_algorithm}.


\begin{algorithm}[H]
 \caption{Block-SPD Wasserstein barycenter}
 \label{wb_algorithm}
 \begin{algorithmic}[1]
  \STATE \textbf{Input:} block-SPD marginals $\{\bP^\ell\}_{\ell = 1}^K$, cost matrices $\{ \bC^\ell\}_{\ell=1}^K$.
  \STATE Initialize $\bar{\bP}^{0}$ as uniform distribution.
  \FOR{$t = 1,...,T$}
  \FOR{$\ell = 1,...,K$}
  \STATE Compute $(\bLambda^\ell)^*$ as in Proposition \ref{dual_var_solution_prop}.
  \ENDFOR
  \STATE Compute the Riemannian gradient of \eqref{w_barycenter} by orthogonally projecting $\sum_\ell \omega_\ell (\bLambda^\ell)^*$ onto the tangent space of $\Delta_n(\sS_{++}^d)$.
  \STATE Update $\bar{\bP}^t$ by retracting on $\Delta_n(\sS_{++}^d)$ with a step size.
%   \alertBM{We should write the concrete updates in appendix and point to those}
  \ENDFOR
  \STATE \textbf{Output:} Barycenter $\bar{\bP}^T$.
 \end{algorithmic} 
\end{algorithm}

==> manuscript.tex <==







% \begin{abstract}
% % Optimal transport (OT) has seen its popularity in various fields of applications. We start by observing that the discrete OT problem can be equivalently solved with respect to a block matrix-valued coupling with uniform diagonal marginals. This leads us to consider a generalized matrix-valued OT problem setup, where the cost and/or the marginals are symmetric positive definite (SPD) matrix-valued. 

% % We propose a novel Riemannian manifold for the matrix version of general doubly stochastic constraint set, which we call the block SPD coupling manifold. Specifically, we consider blocks of SPD matrices, where summation of row blocks and column blocks are constrained. Developing a manifold structure on the constraint allows to make Riemannian optimization framework to be exploited to solve such problems. The framework is generic to solve any linear and non-linear OT problem without specific regularization. This includes projected matrix-valued OT, matrix-valued domain adaptation and barycentric projection, matrix-valued Wasserstein barycenter, Gromov-Wasserstein OT, and distance averaging.
 
% Optimal transport (OT) has seen its popularity in various fields of applications. We start by observing that the OT problem can be viewed as an instance of a general symmetric positive definite (SPD) matrix-valued OT problem, where the cost, the marginals, and the coupling are represented as block matrices and each component block is a SPD matrix. The summation of row blocks and column blocks in the coupling matrix are constrained by the given block-SPD marginals. We endow the set of such block-coupling matrices with a novel Riemannian manifold structure. This allows to exploit the versatile Riemannian optimization framework to solve generic SPD matrix-valued OT problems. We illustrate the usefulness of the proposed approach in several applications.

% % tensor field mass interpolation, Wasserstein-barycenter learning, 
% % %Gromov-Wasserstein distance averaging, 
% % and domain adaptation tasks.  
% \end{abstract}

\section{Introduction}

Optimal transport (OT) offers a systematic approach to compare probability distributions by finding a transport plan (coupling) that minimizes the cost of transporting mass from one distribution to another. It has been successfully applied in a wide range of fields, such as computer graphics \citep{solomon2015convolutional,solomon2014earth}, graph representation learning \citep{chen2020graph,petric2019got}, text classification \citep{yurochkin2019hierarchical}, and domain adaptation \citep{courty2016optimal,courty2014domain}, to name a few.

%\alertPJ{Main comments: 1) we should only talk about vector/matrix/SPD-valued measures in introduction. We should talk about how they are used in different applications. We should talk about doing OT for such class of measures (perhaps even explain why OT is useful for such measures). Then we should also discuss different works that do OT for such measures and what are the main ideas. Then we should talk about our contribution.}

% There exists a number of efficient solvers for classic optimal transport problem \citep{cuturi2013sinkhorn,ferradans2014regularized,genevay2016stochastic,peyre2019computational}. Particularly, by adding an entropy regularization, the OT problem can be solved efficiently via Sinkhorn algorithm \citep{sinkhorn1964relationship} and is known to achieve faster convergence \citep{cuturi2013sinkhorn} and improved sample complexity \cite{genevay2019sample}. 

Despite the popularity of OT, existing OT formulations are mostly limited to scalar-valued distributions. 
%scalar-valued costs and marginals. 
% which we find it to be an instance of a general OT problem with matrix-valued cost. 
% while sometimes a vector-valued and (positive semidefinite) matrix-valued costs are able to capture more information \citep{lopez2021vector}. 
% such as diffusion tensor imaging \citep{le2001diffusion}, image set classification~\citep{huang2015log,harandi2014manifold}, 
% anisotropic diffusion \citep{weickert1998anisotropic}, involve symmetric positive definite (SPD) matrix-valued distributions. 
\revision{
On the other hand, many applications involve symmetric positive definite (SPD) matrix-valued distributions. In diffusion tensor imaging \citep{le2001diffusion}, the local diffusion of water molecules in human brain are encoded in fields of SPD matrices \citep{assaf2008diffusion}. In image processing, region information of an image can be effectively captured through several SPD covariance descriptors \citep{tuzel2006region}. For the application of image set/video classification, each set of images/frames can be represented by its covariance matrix, which has shown great promise in modelling the intra-set variations \citep{huang2015log,harandi2014manifold}. In addition, fields of SPD matrices are also important in computer graphics for anisotropic diffusion \citep{weickert1998anisotropic}, remeshing \citep{alliez2003anisotropic} and texture synthesis \citep{galerne2010random}, just to name a few. In all such cases, being able to compare fields represented by SPD matrices is crucial.
}
This, however, requires a nontrivial generalization of existing (scalar-valued) optimal transport framework with careful construction of cost and transport plan. 

% Hence a generalization to matrix-valued OT is needed. \alertPJ{I think we need to change/improve this as SPD/matrix valued data points is not our focus. Our focus is SPD-valued marginals. SPD/matrix valued data can have scalar-valued marginals. Maybe we can take inspiration from the motivation from existing works. } 

In the quantum mechanics setting, existing works~\citep{jiang2012distances,carlen2014analog,chen2017matrix,chen2018vector} have explored geodesic formulation of the Wasserstein distance between vector and matrix-valued densities. In \citep{ning2013thesis,ning2014matrix}, the Monge-Kantorovich optimal mass transport problem has been studied for comparing matrix-valued power spectra measures. Recently, \citep{peyre2016quantum} proposed to solve an unbalanced optimal transport problem for SPD-valued distributions of unequal masses. 

%In \cite{jiang2012distances,carlen2014analog,chen2017matrix,chen2018vector}, a geodesic formulation of the Wasserstein distance between vector and matrix-valued densities is given, inspired by quantum mechanics. 
%General Matrix-valued OT formulations are developed in \cite{ning2014matrix, ning2013thesis}. 
%\citet{peyre2016quantum} for SPD-valued OT problems and show the usefulness in various applications. It should be emphasized all of the above works rely on \emph{unbalanced} OT formulations.

% where one considers a trace-constrained relaxation for balancing the trace of the marginals \cite{ning2014matrix} and the other \cite{peyre2016quantum} applies a quantum relative entropy regularization to solve an {unbalanced} OT problem (i.e., the transport plan only approximately satisfy the coupling constraint).  


% \alertPJ{This paragaph should be expanded. No need to give dynamic vs static classification}
% \alertAH{The dynamic vs static are discussed in many papers we are referencing. This helps better compare our work to the others because our formulation is static and balanced.}


% \alertAH{When $F(\bGamma)$ is linear, such as in \eqref{reformulated_mw}, one can solve an unbalanced relaxation of the problem with quantum Sinkhorn algorithm \cite{peyre2016quantum}. However, optimization of \eqref{mot_define} in its generic form is challenging, particularly in the balanced setting. }

% \alertBM{The manifold motivation is missing. Why not cvx and why Riemannian.}

In this paper, we propose a general framework for solving the balanced OT problem between SPD-valued distributions, where the cost and the coupling are represented as block SPD matrices. We discuss a Riemannian manifold structure for the set of such block coupling matrices, and we are able to use the Riemannian optimization framework \citep{absil2009optimization, boumal2020intromanifolds} to solve various generalized OT problems. Specifically, our {contributions} \revision{are} as follows. 
% This generalizes the matrix coupling manifold for scalar-valued densities \cite{shi2021coupling,mishra2021manifold}. 
% which proves its versatility in various non-classic scalar-valued optimal transport problems, such as Gromov-Wasserstein OT \cite{memoli2011gromov,peyre2016gromov}, Co-OT \cite{redko2020co}, regularized OT \cite{ferradans2014regularized}.   
\begin{enumerate}
    \item We introduce the general SPD matrix-valued balanced OT problem for SPD matrix-valued marginals and study its metric properties for a specific setting. 
    %We study the metric properties of the proposed formulation and discuss its relationship with the $2$-Wasserstein distance.
    %In the particular case when the SPD marginals are lifted versions of probability measures, the proposed formulation leads to a well-defined distance metric and that it generalizes the classic $2$-Wasserstein distance.
    
    \item We propose a novel manifold structure for the set of block matrix coupling matrices, which generalizes the manifold structures studied in \citep{douik2019manifold,shi2021coupling,mishra2021manifold,mishra2019riemannian}. We discuss optimization-related ingredients like Riemannian metric, Riemannian gradient, Hessian, and retraction.
    
    \item We extend our SPD-valued balanced OT formulation to block SPD Wasserstein barycenter and Gromov-Wasserstein OT.
    
    \item We empirically illustrate the benefit of the proposed framework in domain adaptation, tensor-valued shape interpolation, and displacement interpolation between tensor fields.
\end{enumerate}




{\bf Organizations.} We start with a brief review of Riemannian optimization and SPD matrix-valued optimal transport problem in Section \ref{preliminary_sect}. In Section \ref{matrix_generalized_ot_sect}, we introduce the generalized SPD matrix-valued OT problem and define the proposed {\manname}. Section \ref{manifold_geometry_sect} discusses the Riemannian structure of the proposed manifold and derives the necessary optimization-related ingredients. Section \ref{sec:applications} presents two additional OT related applications of the proposed {\Manname}. In Section \ref{Experiment_sect}, we empirically evaluate the proposed approach in various applications. Section~\ref{sec:conclusion} concludes the paper. In the appendix sections, we provide the proofs and present additional experiments. 
%In Section \ref{Experiment_sect}, we discuss the empirical results of the proposed framework in various applications. 
%In the appendix sections, we provide the proofs and show additional experiments. 



%\alertAH{preliminary as part of introduction?}

\section{Preliminaries}
\label{preliminary_sect}

\subsection{Riemannian optimization}%geometry and optimization}
A matrix manifold $\M$ is a smooth subset of the ambient vector space $\gV$ with local bijectivity to the Euclidean space. A Riemannian manifold is a manifold endowed with a Riemannian metric (a smooth, symmetric positive definite inner product structure $\langle \cdot, \cdot\rangle_x$) on every tangent space $T_x\M$. The induced norm on the tangent space is thus $\| u\|_x = \sqrt{\langle u,u \rangle_x}$. 
% {\color{red} Optimization of an objective function over a smooth Riemannian manifold $\M$ has gained attraction lately \citep{absil2009optimization, boumal2020intromanifolds}. Conceptually, the Riemannian optimization framework treats a constrained optimization problem as an unconstrained optimization problem over the constraint manifold. Consequently, all the standard unconstrained optimization methods such as steepest descent, conjugate gradient, and trust-region have their Riemannian variants \citep{boumal2020intromanifolds}. } \alertAH{Can this be removed or merged somehow?}

The orthogonal projection operation for an embedded matrix manifold ${\rm P}_{x}: \gV \xrightarrow{} T_x\M$ is a projection that is orthogonal with respect to the Riemannian metric $\langle \cdot, \cdot \rangle_x$. Retraction is a smooth map from tangent space to the manifold
% , which allows iterates to move on the manifold along some direction on the tangent space.
That is, for any $x \in \M$, retraction $R_x: T_x\M \xrightarrow{} \M$ such that 1) $R_x(0) = x$ and 2) $\D R_x(0)[u] = u$, where $\D f(x)[u]$ is the derivative of a function at $x$ along direction $u$. 

The Riemannian gradient of a function $F:\M \xrightarrow{} \sR$ at $x$, denoted as $\grad F(x)$, generalizes the notion of the Euclidean gradient $\nabla F(x)$. It is defined as the unique tangent vector satisfying $\langle \grad F(x) , u \rangle_x = \D F(x)[u] = \langle \nabla F(x) ,u\rangle_2$ for any $u \in T_x\M$, where $\langle \cdot, \cdot\rangle_2$ denotes the Euclidean inner product. To minimize the function, Riemannian gradient descent \citep{absil2009optimization} and other first-order solvers apply retraction to update the iterates along the direction of negative Riemannian gradient while staying on the manifold, i.e., $x_{t+1} = R_{x_t}(-\eta \, \grad F(x_t))$, where $\eta$ is the step size. 
Similarly, the Riemannian Hessian $\hess F(x) : T_x\M \xrightarrow{} T_x\M$ is defined as the covariant derivative of Riemannian gradient. Popular second-order methods, such as trust regions and cubic regularized Newton's methods have been adapted to Riemannian optimization \citep{absil2007trust,agarwal2018adaptive}. 
% \alertPJ{This can be shortened to save space if required.}







% \subsection{Optimal transport and Riemannian geometry}
% Many work has constructed manifold geometry for either the coupling or the marginals. The set of (strictly positive) histograms form the so-called multinomial manifold with the Fisher information Riemannian metric \cite{sun2015heterogeneous}. This has later been generalized to simplex of SPD matrices where each simplex element is a SPD matrix \cite{mishra2019riemannian}. In \cite{douik2019manifold,shi2021coupling}, they construct a coupling manifold for the set of positive doubly stochastic couplings, further generalizing the multinomial manifold. All these works can be regarded as special cases of our proposed block SPD coupling manifold.



\subsection{Scalar-valued optimal transport}
\label{ot_preliminary_sect}

Consider two discrete measures supported on $\sR^d$, $\mu = \sum_{i = 1}^m p_i \delta_{\bx_i}$, $\nu = \sum_{j = 1}^n q_j \delta_{\by_j}$, where $\bx_i, \by_j \in \sR^d$ and $\delta_\bx$ is the Dirac at $\bx$. The weights $\bp \in \Sigma_m, \bq \in \Sigma_n$ are in probability simplex \revision{where $\Sigma_k \coloneqq \{ \bp \in \sR^k : p_i \geq 0, \sum_i p_i = 1 \}$}.
% i.e., $\sum_i p_i = \sum_j q_j = 1$, for $p_i, q_j \geq 0$. 
The $2$-Wasserstein distance between $\mu, \nu$ is given by solving the Monge-Kantorovich optimal transport problem: 
% \alertPJ{Here source/target terminology and symbols $\bx_i$ and $\by_i$ are not defined.}
\begin{equation}
\label{W22}
    {\mathrm W}_2^2(\bp,\bq) = \min_{\bgamma \in \Pi(\bp,\bq)} \sum_{i,j} \|\bx_i-\by_j\|^2 \gamma_{i,j},
\end{equation}
where $\Pi(\bp,\bq) \coloneqq \{\bgamma \in \sR^{m \times n} : \bgamma \geq 0, \bgamma \bone = \bp, \bgamma^\top \bone = \bq  \}$ is the space of joint distribution between the source and
the target marginals. An optimal solution of (\ref{W22}) is referred to as an optimal transport plan (or coupling).  %the set of couplings with marginals $\bp$ and $\bq$. 
Recently, \citet{cuturi2013sinkhorn} proposed the Sinkhorn-Knopp  algorithm~\citep{sinkhorn1964relationship,knight2008sinkhorn} for entropy-regularized OT formulation. In case $\mu$ and $\nu$ are measures (i.e., the setting is not restricted to probability measures), it may happen that they are of unequal masses. OT in this case is termed as unbalanced optimal transport \citep{chizat18a,Liero2018}. 
For a recent survey of OT literature and related machine learning applications, please refer to~\citep{peyre2019computational}. 

%Although \eqref{W22} can be solved via linear programming, the computational cost scales poorly with dimension $d$. In \citep{cuturi2013sinkhorn}, an entropy regularization is added to largely reduce the computational cost while pushing the solution away from the boundary. 
% Define the entropy of the coupling as $h(\bgamma) = - \sum_{i,j} \gamma_{i,j} \log(\gamma_{i,j}) + \gamma_{i,j}$. The entropy-regularized problem is 
% \begin{equation}
% \label{W22_reg}
%         _{\bgamma \in \Pi(\bp,\bq)} \sum_{i,j} \|\bx_i-\by_j\|^2 \gamma_{i,j} - \epsilon \, h(\bgamma).
% \end{equation}
%The solution to the regularized problem is unique and can be efficiently solved via the Sinkhorn-Knopp algorithm, originally designed for matrix balancing \citep{sinkhorn1964relationship}. 
% \alertPJ{This can be shortened to save space if required.}


% \paragraph{Matrix OT} brief literature review

% \alertAH{Already give a review in intro. No need to do it again because we do not rely on their formulation.}

\subsection{SPD matrix-valued optimal transport}\label{sec:preliminaries_spdOT}
A SPD matrix-valued measure is a generalization of the (scalar-valued) probability measure (discussed in Section~\ref{ot_preliminary_sect}). Let us consider a SPD matrix-valued measure $M$ and a scalar-valued measure $\mu$  defined on a space $\mathcal{X}$. Let $A$ be a measurable subset of $\mathcal{X}$. Then, while $\mu(A)$ is a non-negative scalar, the ``mass'' $M(A)\in\sS_{+}^d$, where $\sS_{+}^d$ denotes the set of $d\times d$ positive semi-definite matrices. SPD matrix-valued measures have been employed in applications such as diffusion tensor imaging \citep{le2001diffusion}, image set classification~\citep{huang2015log,harandi2014manifold}, 
anisotropic diffusion \citep{weickert1998anisotropic}, and brain imaging~\citep{assaf2008diffusion}, to name a few. 

Recent works~\citep{carlen2014analog,chen2017matrix,ryu18a,peyre2016quantum} have explored optimal transport formulations for SPD matrix-valued measures. While the works \citep{carlen2014analog,chen2017matrix,ryu18a} discuss dynamical (geodesic) OT framework, \citep{peyre2016quantum} studies the ``static'' OT formulation that learns a suitable joint coupling between the input SPD matrix-valued measures. However, \citet{peyre2016quantum} explore an unbalanced OT setup for SPD matrix-valued measures and term it as quantum optimal transport (QOT). Thus, the marginals of the (learned) joint coupling in QOT is not equal to the input SPD matrix-valued measures. As in case of unbalanced (scalar-valued) OT \citep{chizat18a,Liero2018}, the discrepancy between marginals of the joint and the input measures in QOT is penalized via the Kulback-Leibler divergence (for SPD matrix-valued measures). 
%and propose a generalized Sinkhorn algorithm for their problem. 


%In the quantum mechanics setting, existing works~\citep{jiang2012distances,carlen2014analog,chen2017matrix,chen2018vector} have explored geodesic formulation of the Wasserstein distance between vector and matrix-valued densities. In \citep{ning2013thesis,ning2014matrix}, the Monge-Kantorovich optimal mass transport problem has been studied for comparing matrix-valued power spectra measures. Recently, \citep{peyre2016quantum} proposed to solve an unbalanced optimal transport problem for SPD-valued distributions of unequal masses. 




%\section{{\Manname}}
\section{Block SPD optimal transport} 
\label{matrix_generalized_ot_sect}
%\alertPJ{Consider the same setting as in Section \ref{ot_preliminary_sect}.} 
%Let $\bp \in \Sigma_m$ and $\bq \in \Sigma_n$ be the given marginal distributions with supports given by the sets $\{\bx_i\}_{i=1}^m \in \sR^d$ and $\{\by_j\}_{j=1}^n \sR^d$, respectively. 
In this section, we study a balanced OT formulation for SPD matrix-valued measures. Consider $\bP$ and $\bQ$ to be ($d$-dimensional) SPD matrix-valued input measures. Let $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i \in \sS_{++}^d\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}: \revision{\bQ_j} \in \sS_{++}^d\}$ and $\bP$ and $\bQ$ have the same total mass. Without loss of generality, we assume $\sum_i \bP_i = \sum_j \bQ_j = \bI$. Here, $[\cdot]_{m \times n}$ denotes a collection of $mn$ matrices organized as a block matrix and $\bI$ represents the identity matrix. 
The cost of transporting a positive definite matrix-valued mass $\bA$ from position $\bx_i$ (in source space) to $\by_j$ (in target space) is parameterized by a (given) positive semi-definite matrix $\bC_{i,j}$ and is computed as $\trace(\bC_{i,j}\bA)$. Under this setting, we propose the block SPD matrix-valued balanced OT problem as 
\begin{equation}\label{reformulated_mw}
    {\rm MW}^2(\bP, \bQ) \coloneqq \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}), 
\end{equation}
where $\bGamma = [\bGamma_{i,j}]_{m \times n}$ is a block-matrix coupling of size $m \times n$ and the set of such couplings are defined as $\bPi(m,n,d,\bP, \bQ) \coloneqq \{ [\bGamma_{i,j}]_{m \times n} : \bGamma_{i,j} \in \sS_{+}^d, \sum_j \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} = \bQ_j, \forall i \in [m], j \in [n] \}$. Here $\sS_{+}^d$ is used to denote the set of $d\times d$ positive semi-definite matrices and $\trace(\cdot)$ is the matrix trace. The problem is well-defined provided that the corresponding coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ is non-empty. For arbitrary SPD marginals $\bP, \bQ$, there is no guarantee that the set $\bPi(m,n,d,\bP, \bQ)$ defined in (\ref{reformulated_mw}) is not empty \citep{ning2014matrix}. Hence, in this work, we assume that the given marginals $\bP$ and $\bQ$ are such that $\bPi(m,n,d,\bP, \bQ)$ is not empty. In Section \ref{retraction_sinkhorn} later, we discuss a block matrix balancing algorithm which can be used to check whether $\bPi(m,n,d,\bP, \bQ)$ is empty or not for given marginals $\bP$ and $\bQ$. 



\subsection{Metric properties of ${\rm MW}(\bP, \bQ)$} 
%\paragraph{Metric properties of ${\rm MW}(\bP, \bQ)$.} 
In the following result, we show that ${\rm MW}(\bP, \bQ)$ is a valid distance metric for a special case of block SPD marginals.
\begin{proposition}
\label{mw_distance_prop}
Suppose the input SPD matrix-valued marginals have the same support size $n$ and the costs $\{\bC_{i,j}\}_{i,j=1}^n$ satisfy
\begin{enumerate}
    \item $\bC_{i,j}=\bC_{j,i}$ and
    \item $\bC_{i,j}\succ\bzero$ for $i\neq j$ and $\bC_{i,j}=\bzero$ for $i=j$,
%    \item $\bC_{i,j}=\bzero$ if and only if $i=j$
    \item $\forall (i,j,k)\in [n]^3,$ and $ \bA\succeq \bzero,$ $\sqrt{\trace( \bC_{i,j} \bA)} \leq \sqrt{\trace( \bC_{i,k} \bA)} + \sqrt{\trace(  \bC_{j,k}  \bA)}$.
\end{enumerate}
Then, ${\rm MW}(\bP, \bQ)$ is a metric between the SPD matrix-valued marginals $\bP$ and $\bQ$ defined as $\bP\coloneqq\{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$, where $\bp, \bq \in \Sigma_n$ and $\bI$ is the $d\times d$ identity matrix. 
\end{proposition}

We remark that the conditions on $\bC_{i,j}$ in Proposition \ref{mw_distance_prop} generalize the conditions required for ${\rm W}_2(\bp, \bq)$ in \eqref{W22} to be a metric. See for example \citep[Proposition 2.2]{peyre2019computational}. In Appendix \ref{cost_choice_appendix}, we discuss some particular constructions of the cost that satisfy the conditions.



\subsection{Manifold structure for the coupling set $\bPi(m,n,d,\bP,\bQ)$}

We next analyze the coupling constraint set $\bPi(m,n,d,\bP, \bQ)$ and show that it can be endowed with a manifold structure. This allows to exploit the versatile Riemannian optimization framework to solve (\ref{reformulated_mw}) and any more general problem \citep{absil2009optimization}. 

We propose the following manifold structure,
termed as the {\manname}, 
\begin{equation}\label{eq:manifold_proposed}
    \M_{m,n}^d(\bP, \bQ) 
    \coloneqq \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \sum_{j} \bGamma_{i,j} = \bP_i, 
     \sum_i \bGamma_{i,j} =\bQ_j \},
\end{equation}
where $\sum_i \bP_i = \sum_j \bQ_j = \bI$. Particularly, we restrict $\bP_i, \bQ_j,\bGamma_{i,j} \in \sS_{++}^d$, the set of SPD matrices. This ensures that the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ in (\ref{eq:manifold_proposed}) is the interior of the set $\bPi(m,n,d,\bP, \bQ)$. 


As discussed earlier $\bPi(m,n,d,\bP,\bQ)$ is not guaranteed to be non-empty for arbitrary choices of block SPD marginals $\bP$ and $\bQ$~\citep{ning2013thesis}. To this end, we assume that the marginals $\bP$ and $\bQ$ that are given ensure feasibility of the set $\bPi(m,n,d,\bP,\bQ)$. In particular, the manifold $ \M_{m,n}^d(\bP, \bQ)$ inherits the following assumption.
\begin{assumption}\label{assumption:existence}
In this work, we consider block-SPD marginals $\bP$ and $\bQ$ such that the set $\M_{m,n}^d(\bP, \bQ)$ is not empty. 
\end{assumption}
It should be noted that Assumption \ref{assumption:existence} is trivially satisfied for diagonal SPD marginals, i.e., when $\bP_i$ and $\bQ_j$ are diagonal. However, non-diagonal SPD marginals may also satisfy Assumption \ref{assumption:existence} for many problem instances. In Section~\ref{Experiment_sect}, we discuss empirical settings where non-diagonal SPD marginals satisfying Assumption~\ref{assumption:existence} are considered. The following proposition implies that we can endow $\M^d_{m,n}(\bP, \bQ)$ with a differentiable structure.  
\begin{proposition}
\label{smooth_set_prop}
Under Assumption \ref{assumption:existence}, the set $\M^d_{m,n}(\bP, \bQ)$ is smooth, i.e., differentiable.
\end{proposition}


%\paragraph{Relationship with existing manifolds.} 
It should be emphasized that the proposed manifold $\M_{m,n}^d(\bP, \bQ)$ can be regarded as a generalization to existing manifold structures. For example, when $d =1$ and either $m=1$ or $n=1$, $\M_{m,n}^d(\bP, \bQ)$ reduces to the multinomial manifold of probability simplex  \citep{sun2015heterogeneous}. When $d=1$ and $m, n \neq 1$, it reduces the so-called doubly stochastic manifold \citep{douik2019manifold} with uniform marginals or the more general matrix coupling manifold \citep{shi2021coupling}. When $d > 1$ and either $m =1$ or $n =1$, our proposed manifold simplifies to the simplex manifold of SPD matrices \citep{mishra2019riemannian}.



In the next section, we derive various optimization-related ingredients on $\M_{m,n}^d(\bP, \bQ)$ that allow optimization of an arbitrary differentiable objective function on the manifold. In particular, we propose a Riemannian optimization approach following the general treatment by \citep{absil2009optimization, boumal2020intromanifolds}. It allows employing the proposed approach not only for (\ref{reformulated_mw}) but also for other OT problems as discussed in Section~\ref{sec:applications}. 






\begin{algorithm}[t]
 \caption{Riemannian optimization for solving (\ref{eq:manifold_problem}).}
 \label{Riemannian_optimizer}
 \begin{algorithmic}[1]
 \STATE Initialize a feasible $\bGamma_0 \in \M_{m,n}^d$.
 \STATE $\bGamma = \bGamma_0$.
  \WHILE{not converging}
  \STATE Compute Riemannian gradient (and Hessian) at $\bGamma$.
  \STATE Compute the update step $\bxi \in T_{\bGamma} \M_{m,n}^d$.
   \STATE Update $\bGamma \leftarrow R_{\bGamma}(\bxi)$.
  \ENDWHILE
\STATE \textbf{Output:} $\bGamma$.
 \end{algorithmic} 
\end{algorithm}





% We define the \manname \, as 
% \begin{align*}
%     &\M_{m,n}^d(\bP, \bQ) \\
%     &:= \{ \bGamma : \bGamma_{i,j} \in \sS_{++}^d, \sum_{j} \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} =\bQ_j \},
% \end{align*}
% where we restrict $\bGamma_{i,j} \in \sS_{++}^d$, the set of symmetric positive definite (SPD) matrices. This ensures that $\M_{m,n}^d(\bP, \bQ)$ is the interior of the set $\bPi(m,n,d,\bP, \bQ)$. Without loss of generality, we assume $\sum_i \bP_i = \sum_j \bQ_j = \bI$.

\section{Riemannian geometry and optimization over $\M_{m,n}^d(\bP, \bQ)$}
\label{Riem_opt_sec} \label{manifold_geometry_sect}

% \alertPJ{(this subsection should focus on optimization only)}
We consider the general optimization problem
\begin{equation}
    \min_{\bGamma \in \M_{m,n}^d(\bP, \bQ)} F(\bGamma), \label{eq:manifold_problem}
\end{equation}
where $F:{\M_{m,n}^d(\bP, \bQ)} \rightarrow \mathbb{R}$ is a differentiable objective function. The proposed manifold ${\M_{m,n}^d(\bP, \bQ)}$ can be endowed with a smooth Riemannian manifold structure \citep{absil2009optimization, boumal2020intromanifolds}. Consequently, (\ref{eq:manifold_problem}) is an optimization problem on a Riemannian manifold. We solve the problem via the Riemannian optimization framework. It provides a principled class of optimization methods and computational tools for manifolds, both first order and second order, as long as the ingredients such as Riemannian metric, orthogonal projection, retraction, and Riemannian gradient (and Hessian) of a function are defined \citep{absil2009optimization, boumal2014manopt, boumal2020intromanifolds}. Conceptually, the Riemannian optimization framework treats (\ref{eq:manifold_problem}) as an ``unconstrained'' optimization problem over the constraint manifold $\M_{m,n}^d$ (omitted marginals $\bP$, $\bQ$ for clarity).

In Algorithm \ref{Riemannian_optimizer}, we outline the skeletal steps involved in optimization over $\M_{m,n}^d$, where the step $\bxi$ can be computed from different Riemannian methods. In Riemannian steepest descent, $\bxi = -\eta \, \grad F(\bGamma)$, where $\grad F(\bGamma)$ is the Riemannian gradient at $\bGamma$. Also, $\bxi$ is given by the ``conjugate'' direction of $\grad F(\bGamma)$ in the Riemannian conjugate gradient method. And, for the Riemannian trust-region method, $\bxi$ computation involves minimizing a second-order approximation of the objective function in a trust-region ball
\citep{absil2009optimization}. Below, we show the computations of these ingredients.












\subsection{Riemannian metric}
% \paragraph{Riemannian metric.} 
% \alertPJ{Can this be moved up to before Section 4.1?} 
The manifold $\M^d_{m,n}$ is a submanifold of the Cartesian product of $m \times n$ SPD manifold of size $d \times d$, which we denote as $\bigtimes_{m, n} \sS_{++}^d$. The dimension of the manifold $\M^d_{m,n}$ is $(m-1)(n-1)d(d+1)/2$. The {tangent space} characterization of $\M_{m,n}^d$ at $\bGamma$ is obtained as
\begin{equation*}
    T_\bGamma \M_{m,n}^d = \{ [\bU_{i,j}]_{m \times n}: \bU_{i,j} \in \sS^d, \sum_{j} \bU_{i,j} = \bzero, \sum_{i} \bU_{i,j} = \bzero\},
\end{equation*}
where $\sS^d$ is the set of $d \times d$ symmetric matrices. The expression for the tangent space is obtained by linearizing the constraints. We endow each SPD manifold with the affine-invariant Riemannian metric \citep{bhatia2009positive}, which induces a {Riemannian metric} for the product manifold $\M_{m,n}^d$ as
\begin{equation}
    \langle \bU, \bV \rangle_\bGamma = \sum_{i,j} \trace(\bGamma_{i,j}^{-1} \bU_{i,j} \bGamma^{-1}_{i,j} \bV_{i,j}), \label{Riem_metric}
\end{equation}
for any $\bU, \bV \in T_{\bGamma} \M_{m,n}^d$. 

%\GaoC{Better to use $\Gamma_{i,j}$ instead of $\mathbf X_{i,j}$ for notation consistence?}


\subsection{Orthogonal projection, Riemannian gradient, and Riemannian Hessian}
% \paragraph{Orthogonal projection, Riemannian gradient, and Riemannian Hessian.}
As an embedded submanifold, the orthogonal projection plays a crucial role in deriving the Riemannian gradient (as orthogonal projection of the Euclidean gradient in the ambient space). 

\begin{proposition}
\label{orthogonal_proj}
The orthogonal projection of any $\bS \in \bigtimes_{m, n} \sS^d$ to $T_\bGamma\M_{m,n}^d$ with respect to the Riemannian metric \eqref{Riem_metric} is given by 
\begin{equation*}
     {\rm P}_{\bGamma}(\bS) = \bU, \text{ with } \bU_{i,j} = \bS_{i,j} + \bGamma_{i,j} (\bLambda_i+ \bTheta_j) \bGamma_{i,j},
\end{equation*}
where auxiliary variables $\bLambda_i, \bTheta_j$ are solved from the system of matrix linear equations:
\begin{equation*}
\begin{cases}
    -\sum_i \bS_{i,j} = \sum_{i} \bGamma_{i,j} (\bLambda_i + \bTheta_j) \bGamma_{i,j}, & \forall j \\
    -\sum_j \bS_{i,j} = \sum_{j} \bGamma_{i,j} (\bLambda_i + \bTheta_j) \bGamma_{i,j}, & \forall i.
\end{cases}
\end{equation*}
\end{proposition}


Subsequently, the Riemannian gradient and Hessian are derived as the orthogonal projection of the gradient and Hessian from the ambient space. 

\begin{proposition}
\label{Riem_grad_hess}
The Riemannian gradient and Hessian of $F: \M_{m\times n}^d \xrightarrow{} \sR$ are derived as 
\begin{align*}
    \grad F(\bGamma) &= {\rm P}_\bGamma([\bGamma_{i,j} \{ \nabla F(\bGamma_{i,j}) \}_{\rm S} \bGamma_{i,j}]_{m\times n}),\\
    \hess F(\bGamma)[\bU] &= {\rm P}_\bGamma([\D \grad F(\bGamma_{i,j})[\bU_{i,j}] - \{ \bU_{i,j} \bGamma_{i,j}^{-1} \grad F(\bGamma_{i,j}) \}_{\rm S}]_{m\times n}),
\end{align*}
where $\bU \in T_\bGamma\M_{m,n}^d$ and $\nabla F(\bGamma_{i,j})$ is the block partial derivative of $F$ with respect to $\bGamma_{i,j}$. Here, $\D \grad F(\bGamma_{i,j})[\bU_{i,j}]$ denotes the directional derivative of the Riemannian gradient $\grad F$ along $\bU$ and $\{ \bA\}_{\rm S} \coloneqq (\bA + \bA^\top)/2$.
\end{proposition}


\subsection{Retraction and block matrix balancing algorithm}
\label{retraction_sinkhorn}

% \paragraph{Retraction and block matrix balancing algorithm.}
The retraction operation on $\M_{m, n}^d$ is given by a composition of two operations. The first operation is to ensure positive definiteness of the blocks in the coupling matrix. In particular, we use the exponential map associated with the affine-invariant metric on the SPD manifold $\sS_{++}^d$ \citep{bhatia2009positive}. The second operation is to ensure that the summation of the row blocks and column blocks respect the block-SPD marginals. Given an initialized block SPD matrix $[\bA_{i,j}]_{m \times n}$, where $\bA_{i,j} \in \sS_{++}^d$, the goal is to find a `closest' block SPD coupling matrix $\bB \in \M_{m,n}^d$. This is achieved by alternatively normalizing the row and column blocks to the corresponding marginals. The procedure is outlined in Algorithm~\ref{bmb_algorithm}. The solution for the row and column normalization factors $\bR_j, \bL_i$, which are SPD matrices, are computed by solving the Riccati equation $\bT \bX \bT = \bY$ for given $\bX, \bY \in \sS_{++}^d$. Here, $\bT$ admits a unique solution \citep{bhatia2009positive,malago2018wasserstein}. Different from the scalar marginals case where the scaling can be expressed as a diagonal matrix, we need to symmetrically normalize each SPD block matrix. Algorithm~\ref{bmb_algorithm} is a generalization of the RAS algorithm for balancing non-negative matrices \citep{sinkhorn1967diagonal}, which is related to the popular Sinkhorn-Knopp algorithm \citep{sinkhorn1964relationship,knight2008sinkhorn}. We also use Algorithm \ref{bmb_algorithm} to test feasibility of the set $\M_{m, n}^d$ by checking whether Algorithm \ref{bmb_algorithm} outputs a balanced block SPD matrix for a random block SPD matrix $\bA$.

It should be noted that a similar matrix balancing algorithm has been introduced for positive operators \citep{gurvits2004classical,georgiou2015positive}, where the convergence is only established in limited cases. Algorithm~\ref{bmb_algorithm} is different from the quantum Sinkhorn algorithm proposed in \citep{peyre2016quantum} that applies to the {unbalanced} setting. Although we do not provide a theoretical convergence analysis for Algorithm \ref{bmb_algorithm}, we empirically observe quick convergence of this algorithm in various settings (see Appendix \ref{convergence_bmb_retr_appendix}).

% \alertAH{It can be seen that Algorithm~\ref{bmb_algorithm} is a generalization of the popular Sinkhorn-Knopp algorithm \citep{knight2008sinkhorn} which deals with non-negative scalar entries (instead of SPD blocks).}

% \alertAH{RAS algorithm}


% {Here we overload the notation $\sS_{++}^d$ to mean both the set of SPD matrices and SPD manifold with the AI metric.} 
% which is $\bX \exp(\bX^{-1} \bU)$ for any $\bX \in \sS_{++}^d, \bU \in T_\bX\sS_{++}^d$. The $\exp(\cdot)$ denotes matrix exponential.




% \begin{algorithm}[H]
%  \caption{Block matrix balancing algorithm}
%  \label{bmb_algorithm}
%  \begin{algorithmic}[1]
%   \STATE Initialize $\bA_{i,j}^0 = \bA_{i,j}$.
%   \FOR{$t = 1, \ldots, T$}
%   \STATE Find $\bR_j^{t-1}$ such that $\sum_i \bR_j^{t-1} \bA_{i,j}^{t-1} \bR_j^{t-1} = \bQ_j$, $\forall j$.
%   \STATE Update $\bA_{i,j}^{t-1} \xleftarrow{} \bR_j^{t-1} \bA_{i,j}^{t-1} \bR_j^{t-1}$, $\forall j$. 
%   \STATE Find $\bL_i^{t-1}$ such that $\sum_j \bL_i^{t-1} \bA_{i,j}^{t-1} \bL_i^{t-1} = \bP_i$, $\forall i$.
%   \STATE Update $\bA_{i,j}^t \xleftarrow{} \bL_i^{t-1} \bA_{i,j}^{t-1} \bL_i^{t-1}, \forall i$. 
%   \ENDFOR
%  \end{algorithmic} 
% \end{algorithm}


\begin{algorithm}[t]
 \caption{Block matrix balancing algorithm}
 \label{bmb_algorithm}
 \begin{algorithmic}[1]
  \STATE \textbf{Input:} $[\bA_{i,j}]_{m \times n}$, where $\bA_{i,j} \in \sS_{++}^d$ and block SPD marginals $\bP$ and $\bQ$.
  \STATE Initialize $\bB = [\bA_{i,j}]_{m \times n}$. 
  \WHILE{not converging}
  \STATE Find $\bR_j \in \sS_{++}^d$ such that $\sum_i \bR_j \bB_{i,j} \bR_j = \bQ_j$, $\forall j$.
  \STATE Update $\bB_{i,j} \xleftarrow{} \bR_j \bB_{i,j} \bR_j$, $\forall j$. 
  \STATE Find $\bL_i \in \sS_{++}^d$ such that $\sum_j \bL_i \bB_{i,j} \bL_i = \bP_i$, $\forall i$.
  \STATE Update $\bB_{i,j} \xleftarrow{} \bL_i \bB_{i,j} \bL_i, \forall i$. 
  \ENDWHILE
  \STATE \textbf{Output:} The balanced matrix $\bB$.
 \end{algorithmic} 
\end{algorithm}






Based on Algorithm \ref{bmb_algorithm}, we define a retraction $R_\bGamma(\bU)$ at $\bGamma \in  \M_{m, n}^d$ for any $\bU \in T_\bGamma \M_{m,n}^d$ as
\begin{equation}
    R_\bGamma(\bU) = {\rm MBalance} \big([\bGamma_{i,j} {\rm exp}(\bGamma_{i,j}^{-1} \bU_{i,j})]_{m \times n} \big), \label{retr_define}
\end{equation}
where {\rm MBalance} calls the matrix balancing procedure in Algorithm~\ref{bmb_algorithm} and $\exp(\cdot)$ denotes the matrix exponential. The retraction proposed in \eqref{retr_define} is valid (i.e., satisfy the two conditions) for diagonal marginals and empirically we also see the retraction is well-defined for arbitrary block-SPD marginals. See Appendix \ref{convergence_bmb_retr_appendix} for more details. 

% \alertPJ{Is our matrix balancing algorithm similar-to/different-from quantum Sinkhorn algorithm?}



% When each block $\bA_{i,j} \in \sR$ is a positive scalar, i.e. $d = 1$, Sinkhorn's Theorem \cite{sinkhorn1964relationship} proves that the balanced matrix $\bB$ has a standard form $\bB = \bD_1 \bA \bD_2$ for diagonal matrices $\bD_1, \bD_2$. The convergence of the balancing algorithm can be easily established. 

% However, when $d > 1$, proving convergence of Algorithm \ref{bmb_algorithm} is challenging given we need to symmetrically normalize each block. Further, finding the standard form of the balanced block matrix is nontrivial. Nevertheless, we assume a standard form of the resulting block matrix as $\bB_{i,j} = \tilde{\bL}_i \tilde{\bR}_j \bA_{i,j} \tilde{\bR}_j \tilde{\bL}_i$ (or $\tilde{\bR}_j \tilde{\bL}_i \bA_{i,j} \tilde{\bL}_i \tilde{\bR}_j$) $\forall i,j$.

% This assumption is needed to establish a valid retraction based on Algorithm \ref{bmb_algorithm}. 
% Although no theoretical analysis is given, we observe quick empirical convergence of the balancing algorithm, which is illustrated in Figure ..., with randomly generated SPD marginals and block identity initialization.








% \alertAH{The convergence analysis is referred to the Riemannian optimization. However, it seems abrupt to directly move from retraction to convergence for Riemannian optimization.}

\subsection{Convergence and computational complexity}
\label{convergence_complexity_sect}


{\bf Convergence of Riemannian optimization.}
Similar to Euclidean optimization, the necessary first-order optimality condition for any differentiable $F$ on $\M_{m,n}^d$ is $\grad F(\bGamma^*) = 0$, i.e., where the Riemannian gradient vanishes. We call such $\bGamma^*$ the stationary point. The Riemannian methods are known to converge to a stationary point \citep{absil2009optimization,boumal2020intromanifolds} under standard assumptions. Additionally, we show the following.



\begin{theorem}
\label{Prop_Riem_opt_optimal}
Suppose the objective function of the problem $\min_{\bGamma \in \bPi(m,n,d,\bP, \bQ)} F(\bGamma)$ is strictly convex and the optimal solution $\bGamma^*$ is positive definite, i.e., it lies in the interior of $\bPi(m,n,d, \bP, \bQ)$. Then, Riemannian optimization (Algorithm~\ref{Riemannian_optimizer}) for (\ref{eq:manifold_problem}) converges to the same global optimal solution $\bGamma^*$. 
% \alertBM{rephrase this properly}
\end{theorem}
% \begin{proof}
% The main idea is to write out the Riemannian gradient at optimality, which we show coincides with the KKT optimality conditions of (\ref{mot_define}). See Appendix \ref{proof_sect} for more details. 
% \end{proof}
Theorem \ref{Prop_Riem_opt_optimal} guarantees the quality of the solution obtained by Riemannian optimization for a class of objective functions which includes the SPD matrix-valued OT problem with convex regularization.


% \subsection{Computational complexity}
{\bf Computational complexity.}
The complexity of each iteration of the Riemannian optimization algorithm is dominated by the computations of retraction, the Riemannian gradient, the Riemannian Hessian. These also make use of the orthogonal projection operation. All these operations cost $O(mnd^3)$. 
Since the number of parameters to be learned \revision{is} $N=mnd^2$ (size of the coupling block SPD matrix $\bGamma$), the above cost is almost linear in $N$. 









%\section{Block SPD coupling matrix and optimal transport}
%\section{Barycenter learning and Gromov-Wasserstein discrepancy}
\section{Applications of {\manname}}
\label{sec:applications}

As discussed earlier, we employ the proposed {\manname} optimization approach to solve the block SPD matrix valued balanced OT problem (\ref{reformulated_mw}). We now present two other OT related applications of the {\manname}: learning Wasserstein barycenters and the Gromov-Wasserstein averaging of distance matrices. 
%In particular, we consider the problems of learning Wasserstein barycenters and the Gromov-Wasserstein averaging of distance matrices. 
%Apart from making use of the {\manname} to solve \ref{reformulated_mw}, we also consider the problems of learning Wasserstein barycenters and the Gromov-Wasserstein averaging of distance matrices. 


%\section{Applications \alertAH{(better title needed)}}

%In this section, we consider the application of 



% \subsection{Matrix generalized Wasserstein distance}

% We first analyze the metric property of the generalized matrix Wasserstein distance introduced in Section \ref{matrix_generalized_ot_sect}:
% \begin{equation}
%     {\rm MW}^2(\bP, \bQ) = \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}). \label{MW_mot_restate}
% \end{equation}
% With a slight abuse of notation, we denote ${\rm MW}(\bp, \bq)$ as the matrix Wasserstein distance between $\bP, \bQ$ where $\bP_i = p_i \bI, \bQ_j = q_j \bI$ for $\bp, \bq$ in probability simplex. 

% We show in the following proposition that ${\rm MW}(\bp, \bq)$ is a valid distance metric between the discrete measures $\bp, \bq$ provided we construct $\bC_{i,j}$ to be strictly positive definite for $i \neq j$.

% \begin{proposition}
% \label{mw_distance_prop}
% Given $\bp, \bq \in \Sigma_n$ and the cost matrix $\bC_{i,j} \succ \bzero$ for $i \neq j$ and $\bC_{i,j} = \bzero$ for $i = j$, ${\rm MW}(\bp, \bq)$ is a metric between histograms $\bp, \bq$.
% \end{proposition}

% For general semidefinite cost matrix $\bC_{i,j} \succeq \bzero$ for $i \neq j$, ${\rm MW}(\bp, \bq)$ is a pseudo metric where it may happen that ${\rm MW}(\bp, \bq) = 0$ for $\bp \neq \bq$. 



% In Section \ref{matrix_generalized_ot_sect}, we show how the matrix Wasserstein distance is generalized from classic Wasserstein distance: 
% \begin{equation*}
%     {\rm MW}^2(\bp, \bq) := \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}), 
% \end{equation*}

% However, because the matrix cost $\bC_{i,j}$ is a rank-1 semi-definite matrix, the generalized matrix Wasserstein distance ${\rm MW}(\bp, \bq)$ fails to be a valid distance as it does not satisfy the definiteness property. Nevertheless, we show that when $\bC_{i,j}$ is strictly positive definite for $i \neq j$, ${\rm MW}(\bp, \bq)$ is a valid distance metric.




% In this section, we develop various applications and extensions that involve optimization with respect to a block doubly stochastic matrix. We show how our proposed unified framework can be applied in all the settings. 







% \subsection{Barycentric projection for Block SPD OT}

% \label{matrix_domain_adaptation}
% \alertPJ{No need of this section, we need to shift the expression to Section 6.4. Note that useful expression for barycentric projection is available only for a few cost functions, e.g., W22 for scalar OT. Hence, we can discuss our  exact expression in Section 6.4 itself. }

% The optimal transport framework has been popularly explored in unsupervised domain adaptation problems \alertPJ{references} as it exploits the geometry of the underlying metric space to provide distances between the source and the target distributions even when the supports of these distributions do not overlap. The barycentric projection expression for the $2$-Wasserstein OT setting (\ref{W22}) is well-known. 
% Here, we discuss the computation of unsupervised mapping (barycenter projection) of source points in the target domain. 

% Given the source samples $\{ \bX_i \}_{i = 1}^m$, and the target $\{ \bY_j \}_{j = 1}^n$, with $\bX_i, \bY_j \in \sR^{d \times s}$. We define a matrix-valued cost as $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$, which can be viewed as a cross-covariance between the samples. 


% \begin{proposition}
% When $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i - \bY_j)^\top$, ${\rm MW}(\bp, \bq)$ is a distance metric. 
% \end{proposition}




% Domain adaptation first searches for an optimal coupling by solving problem \eqref{MW_mot_restate}. From Theorem \ref{Prop_Riem_opt_optimal}, we can use Riemannian framework developed in Section \ref{manifold_geometry_sect} to optimize the coupling. Then the source samples are projected to align with the target, a process known as \textit{barycentric projection}.


% With the optimal coupling $\bGamma_{i,j}^*$, barycentric projection of the source $\{\bX_i\}$ is computed as
% \begin{equation*}
%     \hat{\bX}_i = \argmin_{\bX_i \in \sR^{d\times s}} \sum_{i,j} \trace \big( (\bX_i - \bY_j)(\bX_i - \bY_j)^\top \bGamma_{i,j}^* \big).
% \end{equation*}
% From the first order condition, we have 
% \begin{equation}
%     \hat{\bX}_i = \bP_i^{-1}(\sum_j \bGamma_{i,j}^* \bY_j), \quad \forall i. \label{barycentric_proj}
% \end{equation}
% The projected samples $\{ \hat{\bX}_i\}$ follow the same distribution as the target samples $\{ \bY_j\}$. When the samples are structured, i.e. symmetric and even semidefinite, barycentric projection can be similarly derived. For symmetric $\bX_i, \bY_j \in \sS_{+}^d$, the projected source samples $\hat{\bX}_i$ are now the symmetric solution to the Lyapunov equation: $\{ \bP_i \hat{\bX}_i \}_{\rm S} = \{\sum_j \bGamma^*_{i,j} \bY_j\}_{\rm S}$.  




\subsection{Block SPD Wasserstein barycenter learning}
\label{block_spd_barycenter}
We consider the problem of computing the Wasserstein barycenter of a set of block SPD matrix-valued measures. 
%Let $\Delta_n(\sS_{++}^d)$ denote $n$ SPD matrices of size $d\times d$, i.e., $\Delta_n(\sS_{++}^d) := \{ \bP = [\bP_i]_{n \times 1} : \sum_i \bP_i = \bI \}$. 
Let $\Delta_n(\sS_{++}^d) \coloneqq \{ \bP = [\bP_i]_{n \times 1} : \bP_i\in\sS_{++}^d, \sum_i \bP_i = \bI \}$ denotes the space of $n\times 1$ block SPD marginals. 
%Let $\{\bP^\ell\}_{\ell=1}^K \in \Delta_{n_\ell}(\sS_{++}^d)$ be the given set of measures. 
Then, the Wasserstein barycenter $\bar{\bP}$ of a set $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$ for all $\ell=\{1, \ldots, K \}$ is computed as follows:
%Given a set of SPD matrix-valued measures, $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$ for $\ell = 1,...,K$, the block SPD Wasserstein barycenter learning problem is to identify
\begin{equation}
    % \gW\gB_\epsilon(\{ \bP^\ell \}, \bomega)
    \bar{\bP}= \argmin_{{\bP} \in \Delta_{n}(\sS_{++}^d)} \sum_{\ell =1}^K \omega_\ell {\rm MW}^2_\epsilon({\bP}, \bP^\ell) , \label{w_barycenter}
\end{equation}
where the given non-negative weights satisfy $\sum_\ell \omega_\ell =1$. 
It should be noted that we employ a regularized version of the proposed block SPD OT problem (\ref{reformulated_mw}) to ensure the differentiability of the objective function near boundary in~\eqref{w_barycenter}. The regularized block SPD OT problem is defined as 
%For the purpose of barycenter learning, we consider a regularized matrix-valued OT problem:
\begin{equation}\label{eqn:regMWOT}
    {\rm MW}^2_\epsilon(\bP, \bQ) \coloneqq \min_{\bGamma \in \M_{m,n}^d(\bP, \bQ)} \sum_{i,j} \Big( \trace( \bC_{i,j}\bGamma_{i,j})+ \epsilon \, \Omega(\bGamma_{i,j}) \Big), 
\end{equation}
where $\epsilon>0$ is the regularization parameter and  $\Omega(\cdot)$ is a strictly convex regularization  (e.g., entropic regularization) on the block SPD coupling matrices. 
%As long as the regularization is convex, Theorem \ref{Prop_Riem_opt_optimal} guarantees the optimal solution by Riemannian optimization. 

%\alertBM{$\gW\gB_\epsilon$ is not used anywhere, removing it}

To solve for $\bar{\bP}$ in (\ref{w_barycenter}), we consider Riemannian optimization on $\Delta_n(\sS_{++}^d)$, which has recently been studied in~\citep{mishra2019riemannian}. 
%To solve $\bar{\bP}$ in (\ref{w_barycenter}), we consider Riemannian optimization in the space of $\Delta_n(\sS_{++}^d)$, which has recently been shown to have a Riemannian manifold structure~\citep{mishra2019riemannian}. 
%that allows optimization of a general objective function. 
%To that end, we only need to compute the Euclidean gradient of the barycenter problem \eqref{w_barycenter} with respect to $\bar{\bP}$ (the Riemannian gradient and other optimization-related ingredients for $\Delta_n(\sS_{++}^d)$ follow from the work of \citep{mishra2019riemannian}. 
%The next proposition shows the Euclidean gradient is given by evaluating the projection of Euclidean gradient of ${\rm MW}_\epsilon$ at optimality.
The following result provides an expression for the Euclidean gradient of the objective function in problem~(\ref{w_barycenter}). 
% with the dual variables $\bLambda_i, \bTheta_j, \bPsi_{i,j}$. From the dual problem, we can verify the Euclidean gradient of the barycenter problem \eqref{w_barycenter} with respect to $\bar{\bX}_i$ is $\bLambda_i^*$ (which is unique up to a translation matrix of size $d \times d$), the optimal dual variable. As long as the optimal dual variable $\bLambda_i^*$ can be computed, we can update $\bar{\bX}_i$ via Riemannian gradient descent on the simplex of SPD manifold \cite{mishra2019riemannian}. 
\begin{proposition}
\label{dual_var_solution_prop}
The Euclidean gradient of \eqref{w_barycenter} with respect to ${\bP}_i$, for $i \in [n]$ is
\begin{equation*}
    \sum_{\ell=1}^K \omega_\ell \nabla_{{\bP}_i}{\rm MW}_\epsilon({\bP}, \bP^\ell) = - \sum_{\ell=1}^K \omega_\ell (\bLambda^\ell_i)^*,
\end{equation*}
where $(\bLambda^\ell_i)^*$ is given by evaluating the orthogonal projection ${\rm P}_{(\bGamma^\ell)^*}(\nabla_{(\bGamma^\ell)^*} {\rm MW}_\epsilon)$, where $\nabla_{(\bGamma^\ell_{i,j})^*} {\rm MW}_\epsilon = \bC_{i,j}^\ell + \epsilon \nabla \Omega((\bGamma^\ell_{i,j})^*)$ and $(\bGamma^\ell)^*$ is the optimal coupling for $\bP^\ell$. That is, $(\bLambda^\ell_i)^*$ is the auxiliary variable obtained during the solving of the system of matrix linear equations in Proposition \ref{orthogonal_proj}. %\alertPJ{Some notational issues - will discuss it over call.}
% The optimal dual variables $\bLambda_i^*, \bTheta_j^*$, $\forall i,j$ of the regularized block matrix-valued OT problem $min_{\bGamma \in \M_{m \times n}^d(\bP, \bQ)} \gW_\epsilon(\bP, \bQ)$ is given by evaluating the orthogonal projection ${\rm P}_{\bGamma^*}(\nabla_{\bGamma^*} \gW_\epsilon)$, where $\nabla_{\bGamma^*_{i,j}} \gW_\epsilon = \bC_{i,j} + \epsilon \nabla \Omega(\bGamma_{i,j}^*)$. The $\bLambda_i^*, \bTheta_j^*$ are given by solving the system of matrix linear equations in Proposition \ref{orthogonal_proj}.
\end{proposition}
% This proposition is a direct result from Theorem \ref{Prop_Riem_opt_optimal}, based on which the Euclidean gradient of problem \eqref{w_barycenter} with respect to the barycenter $\bar{\bX}_i$ is given by $\sum_\ell \omega_\ell (\bLambda_i^\ell)^*$.
The complete algorithm for computing the barycenter in \eqref{w_barycenter} is outlined in Algorithm \ref{wb_algorithm} (Appendix \ref{geometry_spd_simplex_appendix}). 

% \alertPJ{Is this algorithm required or can we simply refer to~\citep{mishra2019riemannian}.} 
% \alertAH{Yes it is required. It is for the purpose of general audience.} \alertPJ{If its general audience, we should put it in supplementary unless we need to fill the main paper - as all the steps can be mapped to the general Algorithm 1.}




% \alertBM{Relook at the remark}
% \begin{remark}
% \label{fast_compute_barycenter_rmk}
% When there are only two input marginals $\sum_{i=1}^m \bX_i \delta_{x_i}$ and $\sum_{j=1}^n \bY_j \delta_{y_j}$, and the distance matrix is scalar-valued, i.e., $\bC_{i,j} = d(x_i, y_j) \bI$ for some ground cost metric $d(\cdot, \cdot)$ on $\gX = \gY$, the barycenter computation can be simplified by extending the displacement interpolation \cite{mccann1997convexity} to matrix-valued marginals. See \citep[Section~2.2]{peyre2016quantum} for more information. Note that due to the balanced nature of our proposed formulation, we do not need to adjust the couplings after matching as required in \cite{peyre2016quantum}.
% \end{remark}




%\subsection{Matrix-valued Gromov-Wasserstein optimal transport and distance averaging}
\subsection{Block SPD Gromov-Wasserstein discrepancy}
\label{sec:proposedGW}
The Gromov-Wasserstein (GW) distance~\citep{memoli2011gromov} generalizes the optimal transport to the case where the measures are supported on possibly different metric spaces $\gX$ and $\gY$. 
Let $\bD^x\in\sR^{m\times m}$ and $\bD^y\in\sR^{n\times n}$ represent the similarity (or distance) between elements in metric spaces $\gX$ and $\gY$ respectively. Let $\bp\in \Sigma_m$ and $\bq \in \Sigma_n$ be the marginals corresponding to the elements in $\gX$ and $\gY$, respectively. 
%Let two set of metric-measure pairs be represented by $(\bD^x, \bp)$ and $(\bD^y, \bq)$. Here, $\bp\in \Sigma_m$ and $\bq \in \Sigma_n$ are the measures and  where $\bD^x$ and $\bD^y$ represent distance (or similarity) matrices 
%Suppose we are given two sets of pairs $(\bD^x, \bp), (\bD^y, \bq)$, where $\bD^x, \bD^y$ represent either similarity or distance matrices and $\bp \in \Sigma_m, \bq \in \Sigma_n$ are the given marginals. 
Then, the GW discrepancy between the two distance-marginal pairs $(\bD^x, \bp)$ and $(\bD^y, \bq)$ is defined as 
\begin{equation*}
\label{eqn:GW}
{\rm GW} \big( (\bD^x, \bp), ( \bD^y, \bq ) \big)  \coloneqq \min_{\bgamma \in \Pi(\bp, \bq)} \sum_{i,i',j,j'} \L(D^x_{i,i'}, D^y_{j,j'}) \gamma_{i,j} \gamma_{i',j'},
\end{equation*}
where $D_{k,l}$ denotes the $(k,l)$-th element in the matrix $\bD$ and $\L$ is a loss between the distance pairs. Common choices of $\L$ include the $L_2$ distance and the KL divergence. 


% \paragraph{GW for cross-domain quantum optimal transport.} 
We now generalize the GW framework to our setting where the marginals are SPD matrix-valued measures.  
%(i.e., tensor-valued by the terminology in \cite{peyre2016quantum}). 
% This can be used for matching tensor fields supported on different domains. 
Let $(\bD^x, \bP)$ and $(\bD^y, \bQ)$ be two distance-marginal pairs, where the Dirac measures are given by $\sum_i \bP_i \delta_{x_i}$, $\sum_j \bQ_j \delta_{y_j}$ respectively, for $\{x_i\}_{i \in [m]} \subset \gX, \{y_j\}_{j \in [n]} \subset \gY$. The marginals are tensor-valued with $\bP \in \Delta_m(\sS_{++}^d)$, $\bQ \in \Delta_n(\sS_{++}^d)$. 
%Different to setting in \citep{peyre2016quantum}, we consider the general case where $\gX \neq \gY$ while the SPD-valued marginals are assumed to have the same dimension $d$. 
%
% We now generalize the GW distance to different metric spaces having block SPD measures. 
% $\bPsi\coloneqq\{[\bPsi_i]_{m\times 1}:\bPsi_i \in \sS_{+}^d,\sum_i \bPsi_i=\bI\}$ and $\bPhi\coloneqq\{[\bPhi_j]_{n\times 1}:\bPhi_i \in \sS_{+}^d,\sum_j \bPhi_j=\bI\}$. 
%Consider two dirac measures $\bPsi = \sum_i \bPsi_i \delta_{x_i}$ and $\bPhi = \sum_j \bPhi_j \delta_{y_j}$ where $\{x_i\}_{i \in [m]} \in \gX, \{y_j\}_{j \in [n]} \in \gY$ and the measures are tensor-valued, i.e., $\bPsi_i, \bPhi_j \in \sS_{++}^d$. Different to \citep{peyre2016quantum}, we consider the general case where $\gX \neq \gY$ and thus the classic matrix-valued OT cannot apply. 
% In \citep{peyre2016quantum}, the domains are assumed to be identical, i.e., $\gX = \gY$ and thus the classic matrix-valued OT can be applied. Here we consider the general case where $\gX \neq \gY$, with $D^x_{i,i'} = d_\gX(x_i, x_{i'}), D^y_{j, j'} = d_{\gY}(y_j, y_{j'})$ for $i,i'\in [m], j,j' \in [n]$ computed from the ground distance on $\gX, \gY$. 
We define the SPD generalized GW discrepancy as
\begin{equation}\label{scalar_gw_ot}
    {\rm MGW} \big( (\bD^x, \bP), ( \bD^y, \bQ ) \big)  \coloneqq \min\limits_{\bGamma \in \M^d_{m \times n}} \sum\limits_{{i,i',} {j, j'}} \L\big( D^x_{i,i'},D^y_{j, j'}  \big) \trace( \bGamma_{i,j} \bGamma_{i',j'}),
\end{equation}
% where $\bD^x, \bD^y$ are computed from the ground distance on $\gX, \gY$, respectively.
% Notice in \eqref{scalar_gw_ot}, the cost can be extended to be matrix-valued, i.e., $\bC_{i,i',j,j'} \in \sS_{+}^d$ between pair $i,i'$ and $j,j'$, which gives a transport cost $\sum_{i,i',j',j'}\trace(\bC_{i,i',j,j'} \bGamma_{i,j} \bC_{i,i',j,j'} \bGamma_{i',j'})$. 
where we use Riemannian optimization (Algorithm \ref{Riemannian_optimizer}) to solve problem~\eqref{scalar_gw_ot}.

% is non-convex and quadratic in $\bGamma$ and it can be solved via Riemannian optimization (Algorithm \ref{Riemannian_optimizer}).

% We employ the proposed Algorithm~\ref{Riemannian_optimizer} to solve~\eqref{scalar_gw_ot}. 


%\alertPJ{It should be noted that the proposed GW setting assumes both the metric spaces $\gX$ and $\gY$ to be $d$-dimensional. However, if the spaces are not aligned (alvares-reference), the elements cannot be directly compared across spaces. Question - can we work with different dimensional SPDs? Why are we using Psi and Phi instead of P and Q?}
%\alertAH{Please note that $\gX, \gY$ is not the space of SPD. It is any metric-measured space. Only the marginals are SPD-valued. So the $d$ dimension has nothing to do with $\gX, \gY$.}

% Similarly, we can consider a generalized matrix-valued GW OT problem. Suppose the cost between the distances $D_{i,i'}^x, D^y_{j,j'}$ is matrix-valued, i.e., $\bC_{i,i',j,j'} \in \sS_{+}^d$, $\forall i,i' \in [m], j,j' \in [n]$ and we are given some block SPD-valued marginals, $\bP, \bQ$ on two domains. Then the generalized GW discrepancy is thus given by 
% \begin{equation}
%     \min_{\bGamma \in \M^d_{m \times m}(\bP, \bQ)} \sum_{i,i',j,j'} \trace(\bC_{i,i',j,j'} \bGamma_{i,j}  \bC_{i,i',j,j'} \bGamma_{i',j'}). \label{tensor_GW_problem}
% \end{equation}
% 











{\bf Gromov-Wasserstein averaging of distance matrices.} The GW formulation with scalar-valued probability measures has been used for averaging distance matrices~\citep{peyre2016gromov}. Building on \eqref{scalar_gw_ot}, we consider the problem of averaging distance matrices where the marginals are SPD-valued.  
% corresponding GW formulation to tensor-valued marginals for quantum distance averaging. 
Let $\{(\bD^\ell, \bP^\ell)\}_{\ell = 1}^K$ with $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$, be a set of distance-marginal pairs on $K$ incomparable domains.
%Given a set of distance-marginal pair $\{(\bD^\ell, \bP^\ell)\}_{\ell = 1}^K$ where $\bP^\ell \in \Delta_{n_\ell}(\sS_{++}^d)$ on $K$ incomparable domains.
Suppose the barycenter marginals $\bar{\bP} \in \Delta_{n}(\sS_{++}^d)$ are given, the goal is to find the average distance matrix $\bar{\bD}$ by solving 
\begin{equation}\label{gw_barycenter_problem}
\begin{array}{ll}
    \bar{\bD} = \argmin\limits_{\bD \in \sS^n : D_{i,j} \geq 0} \sum_{\ell=1}^K \omega_\ell \, {\rm MGW} \big( (\bD, \bar{\bP}), ( \bD^\ell, \bP^\ell ) \big),
\end{array}    
\end{equation}
where the given weights satisfy $\sum_\ell \omega_\ell = 1$.  Problem \eqref{gw_barycenter_problem} can be solved via a block coordinate descent method, that iteratively updates the couplings $\{ \bGamma^\ell \}_{\ell=1}^K$ and the distance matrix $\bar{\bD}$. The update of the coupling is performed via Algorithm \ref{Riemannian_optimizer}. For the update of the distance matrix, we show when the loss $\L$ is decomposable, including the case of $L_2$ distance or the KL divergence, the optimal $\bar{\bD}$ admits a closed-form solution. This is a generalization of the result \citep[Proposition 3]{peyre2016gromov} to SPD-valued marginals.
% The update of barycenter concerns the optimization problem 
% \begin{equation}
%     \min_{ \bD \in \sS^n : \bD_{i,j} \geq 0} \sum_{\ell =1}^K \omega_\ell \, \Big( \sum_{i,i',j,j'} \L(\bar{D}_{i,i'}, D^\ell_{j,j'}) \trace(\bGamma^{\ell}_{i,j} \bGamma^{\ell}_{i',j'}) \Big) \label{gw_barycenter_problem}
% \end{equation}
% which can be solved by gradient descent for reparameterized $\bD$. 
\begin{proposition}
\label{average_distance_update}
Suppose the loss $\L$ can be decomposed as $\L(a, b) = f_1(a) + f_2(b) - h_1(a) h_2(b)$ with $f_1'/h_1'$ invertible, then \eqref{gw_barycenter_problem} has a closed form solution given by $\bar{D}_{i,i'} = \big(\frac{f_1'}{h_1'} \big)^{-1} \big(h_{i,i'} \big)$ with
\begin{equation*}
   h_{i,i'} = \Big( \frac{\sum_{\ell=1}^K \omega_\ell \trace \big(\sum_j \bGamma_{i,j}^\ell \sum_{j'} h_2( D^\ell_{j,j'}) \bGamma^\ell_{i', j'} \big) }{\trace(\bar{\bP}_i \bar{\bP}_{i'})} \Big).
\end{equation*}
\end{proposition}
% \alertPJ{It should be noted that Proposition~\ref{average_distance_update} generalized the results in~\citep{peyre2016gromov} for block SPD measure setting.}







% \subsection{Connection with scalar valued OT}
% Consider the same setting as in Section \ref{ot_preliminary_sect}, with two given measures $\mu = \sum_{i = 1}^m p_i \delta_{\bx_i}$, $\nu = \sum_{j = 1}^n q_j \delta_{\by_j}$ and the marginals $\bp \in \Sigma_m$ and $\bq \in \Sigma_n$. 

% We consider \textit{lifting} the given probability measures to a space of matrix-valued measures where an associated \textit{mass} is represented as a positive semi-definite matrix. To this end, we convert the marginals $\bp$ and $\bq$ to block matrices $\bP$ and $\bQ$, where $\bP \coloneqq \{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = q_i \bI\}$. Here, $[\cdot]_{m \times n}$ denotes a collection of $mn$ matrices organized as a block matrix and $\bI$ represents the identity matrix. 
% The cost of transporting a positive semi-definite (matrix) mass $\bA$ from position $\bx_i$ to $\by_j$ is parameterized by a (given) positive semi-definite matrix $\bC_{i,j}$ and is computed as $\trace(\bC_{i,j}\bA)$. Under this setting, we propose a {block SPD matrix valued OT} problem as 
% \begin{equation}
%     {\rm MW}^2(\bP, \bQ) \coloneqq \min_{\bGamma \in \bPi(m,n,d, \bP, \bQ)  } \sum_{i,j} \trace( \bC_{i,j} \bGamma_{i,j}), %\label{reformulated_mw}
% \end{equation}
% where $\bGamma = [\bGamma_{i,j}]_{m \times n}$ is a block-matrix coupling of size $m \times n$ and the set of such couplings are defined as $\bPi(m,n,d,\bP, \bQ) \coloneqq \{ [\bGamma_{i,j}]_{m \times n} : \bGamma_{i,j} \in \sS_{+}^d, \sum_j \bGamma_{i,j} = \bP_i, \sum_i \bGamma_{i,j} = \bQ_j, \forall i \in [m], j \in [n] \}$. Here $\sS_{+}^d$ is used to denote the set of $d\times d$ positive semi-definite matrices and $\trace(\cdot)$ is the matrix trace. 
% With a slight abuse of notation, let ${\rm MW}(\bp, \bq)\coloneqq {\rm MW}(\bP, \bQ)$ with $\bP,\bQ$ defined above. Below we compare the generalized distance ${\rm MW}(\bp, \bq)$ to ${\rm W}_2(\bp, \bq)$ and analyze its metric properties. 


% \paragraph{Relationship with ${\rm W}_2(\bp, \bq)$.} 
% The $2$-Wasserstein distance ${\mathrm W}_2(\bp,\bq)$ considers the transportation cost of a unit mass from $\bx_i$ to $\by_j$ as $\|\bx_i-\by_j\|^2$, which can be rewritten as $\trace{((\bx_i -\by_j)(\bx_i - \by_j)^\top)}$. Hence, if we consider the cost for the proposed OT problem (\ref{reformulated_mw}) as $\bC_{i,j} = (\bx_i -\by_j)(\bx_i - \by_j)^\top$, then ${\rm MW}(\bp, \bq) = {\mathrm W}_2(\bp,\bq)$ where the optimal block-matrix coupling is $\bGamma^* = \bgamma^* \otimes \bI$ where $\bgamma^*$ is the optimal coupling for ${\rm W}_2(\bp, \bq)$ and $\otimes$ is the Kronecker product.














\section{Experiments}
\label{Experiment_sect}
In this section, we show the utility of the proposed framework in a number of applications. For empirical comparisons, we refer to our approaches, block SPD OT~\eqref{reformulated_mw}, the corresponding Wasserstein barycenter~\eqref{w_barycenter}, and block SPD Gromov-Wasserstein OT~\eqref{scalar_gw_ot}~\&~\eqref{gw_barycenter_problem}, collectively as RMOT (Riemannian optimized Matrix Optimal Transport). 
For all the experiments, we use the Riemannian steepest descent method using the Manopt toolbox \citep{boumal2014manopt} for implementing Algorithm~\ref{Riemannian_optimizer}. The codes are available at \url{https://github.com/andyjm3/BlockSPDOT}.


\subsection{Domain adaptation}
\label{domain_adapt_sect}
We apply our OT framework to the application of unsupervised domain adaptation where the goal is to align the distribution of the source with the target for subsequent tasks. 
% We first discuss below the \textit{barycentric projection} for the proposed block SPD OT formulation (\ref{reformulated_mw}). 
%Here we extend this formulation to matrix-valued samples.

Suppose we are given the source $\bp \in \Sigma_m$ and target marginals $\bq \in \Sigma_n$, along with samples $\{ \bX_i\}_{i=1}^m, \{ \bY_j\}_{j = 1}^n$ from the source and target distributions. The samples are matrix-valued, i.e., $\bX_i ,\bY_j \in \sR^{d \times s}$. We define the cost as $\bC_{i,j} = (\bX_i - \bY_j)(\bX_i -\bY_j)^\top$. It should be noted that $\trace{(\bC_{i,j})}=\|\bX_i - \bY_j\|_{\rm F}^2$ is the cost function under the $2$-Wasserstein OT setting~(\ref{W22}). 
%which can be viewed as a generalized matrix $L_2$ distance.


For domain adaptation, we first learn an optimal coupling between the source and target samples by solving the proposed OT problem \eqref{reformulated_mw} with marginals $\bP, \bQ$ constructed as $\bP \coloneqq \{[\bP_i]_{m\times 1}:\bP_i = p_i \bI\}$ and $\bQ\coloneqq\{[\bQ_j]_{n\times 1}:\bQ_j = \revision{q_j} \bI\}$. Finally, the source samples are projected to the target domain via barycentric projection. Once the optimal couplings $[\bGamma_{i,j}^*]_{m\times n}$, the barycentric projection of a source sample $\bX_i$ is computed as
\begin{equation}\label{eq:barycenter_SPDOT}
% \begin{array}{rl}
    \hat{\bX}_i = \argmin\limits_{\bX_i \in \sR^{d\times s}} \sum_{i,j} \trace ( (\bX_i - \bY_j)(\bX_i - \bY_j)^\top \bGamma_{i,j}^* ) = \bP_i^{-1}(\sum_j \bGamma_{i,j}^* \bY_j).
% \end{array}
\end{equation}
The above approach also works for structured samples. For instance, when the samples are SPD, i.e., $\bX_i, \bY_j \in \sS_{++}^d$, the projected source sample $\hat{\bX}_i$ is now the solution to the matrix Lyapunov equation: $\{ \bP_i \hat{\bX}_i \}_{\rm S} = \{\sum_j \bGamma^*_{i,j} \bY_j\}_{\rm S}$. Here, $\{ \bA\}_{\rm S} = (\bA + \bA^\top)/2$.


For the scalar-valued OT case, discussed in Section \ref{ot_preliminary_sect}, the barycentric projection of a source sample $\bX_i$ is computed as
\begin{equation}\label{eq:barycenter_scalar}
% \begin{array}{rl}
    \hat{\bX}_i = \argmin\limits_{\bX_i \in \sR^{d\times s}} \sum_{i,j} \| \bX_i - \bY_j\|_F^2 \bgamma_{i,j}^* = p_i^{-1}(\sum_j \gamma_{i,j}^* \bY_j),
% \end{array}
\end{equation}
where $\bgamma^* = [\gamma^*_{i,j}]$ is the optimal coupling matrix of size $m\times n$ for the scalar-valued OT problem.

Contrasting the barycentric projection operations (\ref{eq:barycenter_SPDOT}) with (\ref{eq:barycenter_scalar}), we observe that (\ref{eq:barycenter_SPDOT}) allows to capture feature-specific correlations more appropriately. The benefit of the matrix-valued OT modeling over the scalar-valued OT modeling is reflected in the experiments below.
























%\paragraph{Image set classification.} 
{\bf Experimental setup.}
We employ domain adaptation to classify the test sets (target) of multiclass image  datasets, where the training sets (source) have a different class distribution than the test sets. 
% Supervision is available only for training set.  
%We test the above formulation for image set classification . 
    Suppose we are given a training set $\{ \bX_i\}_{i=1}^m$ and a test set $\{  \bY_j\}_{j=1}^n$ where $\bX_i, \bY_j \in \sR^{d \times s}$ are $s$ (normalized) image samples of the same class in $d$ dimension for each image set $i,j$. Instead of constructing the cost directly on the input space, which are not permutation-invariant, we first compute the sample covariances $\bS_{x_i} = \bX_i \bX_i^\top/s$ and $\bS_{y_j} = \bY_j \bY_j^\top/s$, $\forall i,j$. Now the cost between $i, j$ is given by $\bC_{i,j} = (\bS_{x_i} - \bS_{y_j})(\bS_{x_i} - \bS_{y_j})^\top$. Once the block SPD matrix coupling is learnt, the $\bS_{x_i}$ covarinaces are projected using the barycerntric projection to obtain $\hat{\bS}_{x_i}, i \in [m]$. This is followed by nearest neighbour classification of $j$ based on the Frobenius distance $\| \hat{\bS}_{x_i} - \bS_{y_j} \|_{\rm F} \forall i,j$. 



We compare the proposed {\algname} (\ref{reformulated_mw}) with the following baselines: (i) sOT: the $2$-Wasserstein OT~(\ref{W22}) with the cost $c_{i,j} = \trace(\bC_{i,j})=\|\bS_{x_i} - \bS_{y_j} \|_{\rm F}^2$ \citep{courty2016optimal}, and (ii) SPDOT: the $2$-Wasserstein OT (\ref{W22}) with the cost as the squared Riemannian geodesic distance between the SPD matrices $\bS_{x_i}$ and $\bS_{y_j}$ \citep{yair2019parallel}. 

\begin{figure}%[!t]
\label{domain_adaptation_figure}
%\captionsetup{justification=raggedright,singlelinecheck=false}
    \centering
    \subfloat[MNIST \label{mnist_fig}]{\includegraphics[width = 0.33\textwidth, height = 0.25\textwidth]{Figures/domain_adaptation/mnist_da_result.pdf}} 
    \subfloat[Fashion MNIST \label{fmnist_fig}]{\includegraphics[width = 0.33\textwidth, height = 0.25\textwidth]{Figures/domain_adaptation/fashionmnist_da_result.pdf}} 
    \subfloat[Letters \label{letters_fig}]{\includegraphics[width = 0.33\textwidth, height = 0.25\textwidth]{Figures/domain_adaptation/letters_da_result.pdf}}
    \caption{Domain adaptation and classification results for three datasets: MNIST \eqref{mnist_fig}, Fashion MNIST \eqref{fmnist_fig} and Letters~\eqref{letters_fig}. The skew ratio increases from uniform (uf) to $r=0.5$. For MNIST and Fashion MNIST, uf=$0.1$ and for Letters, uf=$1/26$. We observe that the proposed RMOT performs significantly better than the baselines. 
    %The proposed RMOT outperforms sOT and SPDOT, especially in more challenging domain adaptation settings, i.e., higher skew ratios, implying the usefulness of the non-trivial correlations learned by the SPD matrix valued couplings of {\algname}.
    % Thus, the SPD matrix valued couplings of RMOT seem to better understand the non-trivial correlations. 
    % shows a good performance in harder settings (with higher skew ratios) implying the SPD matrix-valued couplings understand non-trivial correlations.
    }
\end{figure}



\textbf{Datasets.} We experiment on three multiclass image datasets -  handwritten letters \citep{frey1991letter}, MNIST \citep{lecun1998gradient} and Fashion MNIST \citep{xiao2017fashion} - with various skewed distributions for the training set. MNIST and Fashion MNIST have $10$ classes, while Letters has $26$ classes. 
Specifically, we fix the distribution of the test set to be uniform (with the same number of image sets per class). We increase the proportion of the a randomly chosen class in the training set to the ratio $r$, where $r=\{{\rm uf},0.1,0.2,0.3,0.4,0.5\}$ and ${\rm uf}$ is the ratio corresponding to the uniform distribution of all classes. We reduce the dimension of MNIST, fashion MNIST, and Letters by PCA to $d=5$ features. We set $s=d$, $m=250$, and $n=100$ for each dataset. 
%The sample size $s = d$ for each dataset is chosen uniformly. 
%This results in $m = 250, n = 100$ for training and test set, respectively. 

\textbf{Results.} Figures~\ref{mnist_fig}-\ref{letters_fig} shows the classification accuracy on the three datasets. 
We observe that the proposed RMOT outperforms sOT and SPDOT, especially in more challenging domain adaptation settings, i.e., higher skew ratios. This implies the usefulness of the non-trivial correlations learned by the SPD matrix valued couplings of {\algname}. 
%We observe that the proposed SPD-valued OT compared to scalar-valued OT as the skew $r$ increases (harder settings). 

%  which gives $d = 34$ for MNIST and $d = 14$ for fashion MNIST













\subsection{Tensor Gromov-Wasserstein distance averaging for shape interpolation}
% \alertBM{We should refer to the papers}
We consider an application of the proposed block SPD Gromov-Wasserstein OT formulation (Section~\ref{sec:proposedGW}) for interpolating tensor-valued shapes. We are given two distance-marginal pairs $(\bD^0, \bP^0), (\bD^1, \bP^1)$ where $\bD^0, \bD^1 \in \sR^{n \times n}$ are distance matrices computed from the shapes and $\bP^0, \bP^1$ are given tensor fields. The aim is to interpolate between the distance matrices with weights $\bomega = (t, 1-t), t \in [0,1]$. The interpolated distance matrix $\bD^t$ is computed by solving \eqref{gw_barycenter_problem} via Riemannian optimization and Proposition \ref{average_distance_update}, with the barycenter tensor fields ${\bP}^t$ given. Finally, the shape is recovered by performing multi-dimensional scaling to the distance matrix. 



\begin{figure}%[ht]
% \settoheight{\tempdima}{\includegraphics[width=.06\textwidth]{example-image-a}}%
\centering
\begin{tabular}{@{}c@{ \hspace*{1.5pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }c@{ \hspace*{2pt} }}
\raisebox{.025\textwidth}{\footnotesize (a)}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/cat-dog-input-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/bary-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/bary-2.pdf}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/bary-3.pdf}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/bary-4.pdf}&
\includegraphics[width=.11\textwidth]{Figures/cat-dog-gw/cat-dog-input-2.pdf}\\[5pt]
% \raisebox{.025\textwidth}{\footnotesize (b)}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-1.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-1.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-2.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-3.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/bary-4.pdf}&
% \includegraphics[width=.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-2.pdf}\\[5pt]

\raisebox{.025\textwidth}{\footnotesize (b)}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/input-r-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/bary-r-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/bary-r-2.pdf}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/bary-r-3.pdf}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/bary-r-4.pdf}&
\includegraphics[width=.11\textwidth]{Figures/annulus-star4-gw/input-r-2.pdf}\\[5pt]

\raisebox{.025\textwidth}{\footnotesize (c)}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/disk-star5-input-r-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/bary-r-1.pdf}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/bary-r-2.pdf}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/bary-r-3.pdf}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/bary-r-4.pdf}&
\includegraphics[width=.11\textwidth]{Figures/disk-star5-r/disk-star5-input-r-2.pdf}\\[3pt]
&{\footnotesize $t=0$} & {\footnotesize $t=0.2$} & {\footnotesize $t=0.4$} & {\footnotesize $t=0.6$} & {\footnotesize $t=0.8$} & {\footnotesize $t=1$} \\
\end{tabular}
\caption{Tensor-valued shape interpolation obtained using the proposed Gromov-Wasserstein RMOT formulation~(Section~\ref{sec:proposedGW}). We note that each shape consists of several SPD-matrix/tensor valued fields (displayed using ellipses). \revision{In (a), the tensors follow a uniform distribution. In (b), the tensors are generated with multiple orientation and in (c), tensors vary smoothly in both size and orientation.} The proposed approach takes the anisotropy and orientation of tensor fields into account while interpolating shapes. }%
\label{GW_distance_averaging}
\end{figure}






Figure \ref{GW_distance_averaging} presents the interpolated shapes with $n = 100$ sample points for the input shapes. The matrices $\bD^0, \bD^1$ are given by the Euclidean distance and we consider $L_2$ loss for $\L$. The input tensor fields $\bP^0, \bP^1$ are generated as uniformly random in (a), cross-oriented in (b) and smoothly varying in (c). \revision{For simplicity, we consider the barycenter tensor fields given by the linear interpolation of the inputs, i.e., $\bP^t = (1-t) \bP^0 + t \bP^1$. In \citep{peyre2016gromov}, we highlight that the marginals are scalar-valued and fixed to be uniform. Here, on the other hand, the marginals are tensor-valued and the resulting distance matrix interpolation would be affected by the relative mass of the tensors, as shown by Proposition \ref{average_distance_update}.}
% The barycenter tensor fields are given by the linear interpolation of the inputs, i.e., $\bP^t = (1-t) \bP^0 + t \bP^1$. 
The results show the proposed Riemannian optimization approach (Section~\ref{manifold_geometry_sect}) converges to reasonable stationary solutions for non-convex OT problems. 








\begin{figure*}%[!th]
%\captionsetup{justification=centering}
    \centering
    \subfloat[Linear interpolation]{\includegraphics[width = 0.19\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/linear-interp.pdf}} 
    \hspace*{5pt}
    \subfloat[QOT ($\rho$=50)]{\includegraphics[width = 0.19\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_50.pdf}}
    \hspace*{5pt}
    \subfloat[QOT($\rho$=100)]{\includegraphics[width = 0.19\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_100.pdf}}
    \hspace*{5pt}
    \subfloat[QOT($\rho$=500)]{\includegraphics[width = 0.19\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/QOT-ellipses_500.pdf}}
    \hspace*{5pt}
    \subfloat[{\algname}]{\includegraphics[width = 0.19\textwidth, height = 0.1\textwidth]{Figures/dirac-pairs-smooth/BlockMOT-ellipses.pdf}} \\[5pt]
    
    \subfloat[Input ($t = 0$) \label{input_1}]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/input-ellispses-1.pdf}} 
    \hspace*{3pt}
    \subfloat[Input ($t=1$) \label{input_2}]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/input-ellispses-2.pdf}} 
    \hspace*{3pt}
    \subfloat[QOT ($t=0.25$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat[QOT ($t=0.5$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat[QOT ($t=0.75$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/interpol-ellispses-4.pdf}} 
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.25$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-2.pdf}}
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.5$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-3.pdf}}
    \hspace*{3pt}
    \subfloat[{\algname} ($t=0.75$)]{\includegraphics[width = 0.12\textwidth, height = 0.12\textwidth]{Figures/2d-aniso-fields/BlockMOT-interpol-ellispses-4.pdf}}
    \caption{Tensor field mass interpolation on 1-$d$ (top) and 2-$d$ (bottom) grids. On the top, each row corresponds to an interpolation where we show $7$ evenly-spaced interpolated tensor fields. On the bottom, the inputs are given in (f) and (g). We set $\rho = 100$ for QOT and show $3$ evenly-spaced interpolated tensor fields.} 
    \label{interpolation_figure}
\end{figure*}





\subsection{Tensor field optimal transport mass interpolation}
We consider performing optimal transport and displacement interpolation between two tensor fields supported on regular 1-$d$ (or 2-$d$) grids~\citep{peyre2016quantum}. 
We consider a common domain $\gD = [0,1]$ (or $[0,1]^2$) with the cost defined as $\bC_{i,j} = \| \bx_i - \by_j \|^2 \bI$ for $\bx_i, \by_j \in \gD$. The marginals $\bP, \bQ$ are given tensor fields. We first compute the balanced coupling $\bGamma$ by solving an entropy regularized OT problem~(\ref{eqn:regMWOT}): 
\begin{equation*}
    \min_{\bGamma \in \M_{m \times n}^d(\bP, \bQ)} \sum_{i,j} \Big( \trace(\bC_{i,j}\bGamma_{i,j}) - \epsilon \, H(\bGamma_{i,j}) \Big),
\end{equation*} 
where the quantum entropy is defined as $H(\bGamma_{i,j}) \coloneqq - \trace(\bGamma_{i,j} \log(\bGamma_{i,j}) - \bGamma_{i,j})$. 
Then, the coupling is used to interpolate between the two tensor fields by generalizing the displacement interpolation \citep{mccann1997convexity} to SPD-valued marginals. Please refer to~\citep[Section~2.2]{peyre2016quantum} for more details. It should be noted that due to the balanced nature of our formulation, we do not need to adjust the couplings after matching as required in~\citep{peyre2016quantum}.












We compare interpolation results of the proposed (balanced) {\algname} with both linear interpolation $(1-t)\bP + t \bQ$ for $t \in [0,1]$ and the \textit{unbalanced} quantum OT (QOT) of \citep{peyre2016quantum}. The QOT solves the following problem with quantum KL regularization, i.e.,
\begin{equation*}
    \min\limits_{\bGamma} \sum_{i,j} \Big( \trace(\bC_{i,j} \bGamma_{i,j}) - \epsilon \, H(\bGamma_{i,j}) + \rho \, {\rm KL}(\bGamma \sone \vert \bP) + \rho \,{\rm KL}(\bGamma^\top \sone \vert \bQ) \Big), 
\end{equation*}
where ${\rm KL}(\bP \vert \bQ) \coloneqq \sum_i \trace \big(\bP_i \log(\bP_i) - \bP_i \log(\bQ_i) -\bP_i +\bQ_i \big)$  and $\bGamma \sone \coloneqq [\sum_j (\bGamma_{i,j})]_{m \times 1}$  and  $\bGamma^\top \sone \coloneqq [\sum_i (\bGamma_{i,j})]_{n \times 1}$. For comparability, we set the same $\epsilon$ for both QOT and {\algname}.
% and Riemannian optimization stops after $30$ iterations using Riemannian steepest descent. 




Figure \ref{interpolation_figure} compares the mass interpolation for both 1-$d$ (top) and 2-$d$ (bottom) grids. 
%For the 1-$d$ case, we observe the interpolated tensor fields obtained by QOT traverse from the linear interpolation to {\algname} as the parameter $\rho$ increases.  
%{\algname} can be considered as the limit of QOT when $\rho \xrightarrow{} \infty$. 
For the 2-$d$ tensor fields, we further render the tensor fields via a background texture where we perform anisotropic smoothing determined by the tensor direction. \revision{To be specific, we follow the procedures in \citep{peyre2016quantum} by applying the tensor to the gradient vector of the textures on the grid such that the texture is stretched in the main eigenvector directions of the tensor.}
%Similarly, we see the tensor fields generated from {\algname} more closely respect the marginal constraints.
In both the settings, we observe that the tensor fields generated from {\algname} respect the marginal constraints more closely. 






\subsection{Tensor field Wasserstein barycenter}
We also analyze the Wasserstein barycenters learned by the proposed RMOT approach and qualitatively compare with QOT barycenter \citep[Section 4.1]{peyre2016quantum}. We test on two tensor fields ($n = 4$) supported 2-$d$ grids.  
%to illustrate the difference between {\algname} and QOT barycenter \citep[Section 4.1]{peyre2016quantum}. 

Figure~\ref{barycenter_fig} compares barycenter from QOT (top) and {\algname} (bottom) initialized from the normalized solution of QOT. We observe that the QOT solution is not optimal when the marginal constraint is enforced and the barycenter obtained does not lie in the simplex of tensors. 
\revision{Such a claim is strengthened by comparing the objective value versus the optimal value, obtained by the CVX toolbox \citep{grant2014cvx}. The objective can be further decreased when initialized from the (normalized) QOT solution, see more discussions in Appendix \ref{appendix:additional_experiments}. }




\begin{figure}%[!th]\
\centering
%\captionsetup{justification=centering}
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/input-1.pdf}
	\end{minipage}}
 %\hfill 	
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-2-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-2-5.pdf}
	\end{minipage}}
	%\hfill
	\subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-3-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-3-5.pdf}
	\end{minipage}}
	%\hfill
	\subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/QOTbarycenter-4-5.pdf} \\[8pt]
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/MOTbarycenter-qot-4-5.pdf}
	\end{minipage}}
 %\hfill	
  \subfloat{
	\begin{minipage}[c][0.08\textwidth]{
	   0.08\textwidth}
	   \centering
	   \includegraphics[width=0.5\textwidth]{Figures/2d-bary-n2/input-2.pdf}
	\end{minipage}}
\caption{Barycenter interpolation. From left to right $t = 0$ (input), $t= 0.25, 0.5, 0.75$ (barycenters), $t=1$ (input). The top row is QOT and the bottom is {\algname}.}
\label{barycenter_fig}
\end{figure}



% \begin{figure}[!th]
% \captionsetup{justification=centering}
%     \centering
%     \subfloat[Input ($t=0$)]{\includegraphics[width = 0.05\textwidth, height = 0.05\textwidth]{}} 
%     \hspace*{5pt}
%     \subfloat[Input ($t=0$)]{\includegraphics[width = 0.05\textwidth, height = 0.05\textwidth]{Figures/2d-bary-n2/input-2.pdf}} 
%     \caption{Barycenter} 
%     \label{barycenter_fig}
% \end{figure}








% \begin{figure}[!th]
% \captionsetup{justification=centering}
%     \centering
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-2.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-3.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/bary-4.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cat-dog-gw/cat-dog-input-2.pdf}} \\[5pt]
    
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-1.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-2.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-3.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/bary-4.pdf}}
%     \hspace*{5pt}
%     \subfloat{\includegraphics[width = 0.06\textwidth, height = 0.06\textwidth]{Figures/cross-heart-gw/cross-heart-input-2.pdf}} \\[5pt]
    
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-1.pdf}}{\footnotesize $t=0$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-1.pdf}}{\footnotesize $t=0.2$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-2.pdf}}{\footnotesize $t=0.4$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-3.pdf}}{\footnotesize $t=0.6$}
%     \hspace*{3pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/bary-r-4.pdf}}{\footnotesize $t=0.8$}
%     \hspace*{0.7pt}
%     \stackunder[6pt]{\includegraphics[width=0.06\textwidth, height = 0.06\textwidth]{Figures/disk-star5-r/disk-star5-input-r-2.pdf}}{\footnotesize $t=1$} 
    
%     \caption{Tensor-valued shape interpolation.} 
%     \label{GW_distance_averaging}
% \end{figure}















\section{Conclusion}\label{sec:conclusion}
In this paper, we have discussed the balanced optimal transport (OT) problem involving SPD matrix-valued measures. For the SPD matrix-valued OT problem, the coupling matrix is a block matrix where each block is a symmetric positive definite matrix. The set of such coupling matrices can be endowed with Riemannian geometry, which enables optimization both linear and non-linear objective functions. We have also shown how the SPD-valued OT setup extend many optimal transport problems to general SPD-valued marginals, including the Wasserstein barycenter and the Gromov-Wasserstein (GW) discrepancy. Experiments in a number of applications confirm the benefit of our approach.

% In the appendix Section \ref{sec:appendix_projection}, we discuss the projected version of the SPD-valued OT problem. As a future research direction, it would be interesting to explore such other properties. Another direction could be on learning of block coupling matrices with different constraints. In Section \ref{trace_mfd_appendix}, we discuss a constraint involving the matrix trace.






% We have shown how SPD-valued OT problem is a metric and allows to extend many optimal transport problems to general SPD-valued marginals, including the Wasserstein barycenter and the Gromov-Wasserstein (GW) discrepancy.

% We have also developed a new manifold geometry for learning the block SPD matrix couplings and demonstrated its utility in various OT problems.  Potential future research directions include developing faster optimization algorithms in the stochastic settings for sub-sampled marginals.





%trace_mfd_appendix

% to a general SPD-valued GW discrepency.


% The primary advantage of such manifold structure is that we can exploit well-established Riemannian optimization toolbox for any optimization problem with block coupling constraints.


% \alertPJ{Thus, we do not rely on any regularization as in standard OT solvers. - We should not write this anywhere in the main paper.} \alertPJ{We could discuss/summarize more novel contributions if needed - e.g., metric property, shape interpolation of tensor fields }



% One potential future research direction is to reduce the computational cost in high-dimensional and large-sample settings. For example, one can utilize stochastic Riemannian optimizers for sub-sampled marginals, as similarly considered in \cite{aude2016stochastic}. 
% \alertPJ{we should write the future work without highlighting computational cost issue. }


% \bibliographystyle{plain}
% \bibliography{references}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newpage
% \section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% % The checklist follows the references.  Please
% % read the checklist guidelines carefully for information on how to answer these
% % questions.  For each question, change the default \answerTODO{} to \answerYes{},
% % \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% % justification to your answer}, either by referencing the appropriate section of
% % your paper or providing a brief inline description.  For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% % Please do not modify the questions and only use the provided macros for your
% % answers.  Note that the Checklist section does not count towards the page
% % limit.  In your paper, please delete this instructions block and only keep the
% % Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerTODO{}
%   \item Did you discuss any potential negative societal impacts of your work?
%      \answerNA{We currently do not foresee any negative societal impact given the work is theoretical nature.}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%      \answerYes{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}
%         \item Did you include complete proofs of all theoretical results?
%     \answerYes{In the supplementary material}
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{In supplementary material}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{See experiment sections}
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerYes{}
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{}
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{}
%   \item Did you mention the license of the assets?
%     \answerYes{In the code}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerYes{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerNA{Data are publicly available}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNA{}
% \end{enumerate}


% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}


% \end{enumerate}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







